A New Algorithm for Decremental Single-Source Shortest Paths with Applications to Vertex-Capacitated Flow and Cut Problems

We study the vertex-decremental Single-Source Shortest Paths (SSSP) problem: given an undirected graph $G=(V,E)$ with lengths $\ell(e)\geq 1$ on its edges and a source vertex $s$, we need to support (approximate) shortest-path queries in $G$, as $G$ undergoes vertex deletions. In a shortest-path query, given a vertex $v$, we need to return a path connecting $s$ to $v$, whose length is at most $(1+\epsilon)$ times the length of the shortest such path, where $\epsilon$ is a given accuracy parameter. The problem has many applications, for example to flow and cut problems in vertex-capacitated graphs. Our main result is a randomized algorithm for vertex-decremental SSSP with total expected update time $O(n^{2+o(1)}\log L)$, that responds to each shortest-path query in $O(n\log L)$ time in expectation, returning a $(1+\epsilon)$-approximate shortest path. The algorithm works against an adaptive adversary. The main technical ingredient of our algorithm is an $\tilde O(|E(G)|+ n^{1+o(1)})$-time algorithm to compute a \emph{core decomposition} of a given dense graph $G$, which allows us to compute short paths between pairs of query vertices in $G$ efficiently. We believe that this core decomposition algorithm may be of independent interest. We use our result for vertex-decremental SSSP to obtain $(1+\epsilon)$-approximation algorithms for maximum $s$-$t$ flow and minimum $s$-$t$ cut in vertex-capacitated graphs, in expected time $n^{2+o(1)}$, and an $O(\log^4n)$-approximation algorithm for the vertex version of the sparsest cut problem with expected running time $n^{2+o(1)}$. These results improve upon the previous best known results for these problems in the regime where $m= \omega(n^{1.5 + o(1)})$.

==> applications.tex <==
\section{Application: Maximum $s$--$t$ Flow and Minimum $s$--$t$ Cut}\label{sec: max flow min cut}
%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------
%-------------------------------------------------------------------------------------------





%We modify our graph $G$, as follows. For each vertex $v\in A\cup B$, we create one special copy $v^*$. We let $A'$ denote the set of special copies of the vertices in $A$, and by $B'$ the set of copies of the vertices in $B$. Additionally,
%for every vertex $v\in V(G)$, we create $1/\alpha$ regular copies. For every edge $(u,v)\in E(G)$, we add edges between every copy of $u$ and every copy of $v$. Let $G'$ denote this resulting graph (we note that we never actually compute or store this graph; it is only defined for the sake of the analysis). Let $\pset$ denote the set of all paths connecting vertices of $A'$ to vertices of $B'$.

We assume that we are given an undirected graph $G=(V,E)$ with capacities $c(v)$ on vertices $v\in V$, and two special vertices $s$ and $t$ with infinite capacity. Our goal is to find maximum $s$-$t$ flow that obeys the vertex capacities. We show below an algorithm that finds a $(1-\eps)$-approximate flow in time $\frac{n^{2+o(1)}\log(1/\eps)}{\eps^2}$. Let $\pset$ be the set of all paths connecting $s$ to $t$ in $G$.




\begin{tabular}[t]{|l|l|}\hline &\\
$\begin{array}{lll}
\text{\underline{Primal}}&&\\
\text{Max}&\sum_{P\in \pset} f(P)&\\
\text{s.t.}&&\\
%&\sum_{P\in \pset(a)}f(P)\leq 1&\forall a\in A'\\
%&\sum_{P\in \pset(b)}f(P)\leq 1&\forall b\in B'\\
&\sum_{\stackrel{P\in\pset:}{v\in P}}f(P)\leq
c(v)&\forall v\in V(G')\\
&f(P)\geq 0&\forall P\in \pset\\
\end{array}$
&$
\begin{array}{lll}
\text{\underline{Dual}}&&\\
\text{Min}&\sum_{v\in V(G')}c(v)x_v\\
\text{s.t.}&&\\
&\sum_{v\in P}x_v\geq 1&\forall P\in \pset\\
&x_v\geq 0&\forall v\in V(G')\\
&&\\
\end{array}$\\ &\\ \hline
\end{tabular}

Recall that for any feasible dual solution of cost $C_{\mbox{Dual}}$,

\[\opt\leq \opt_{\mbox{Primal}}\leq \opt_{\mbox{Dual}}\leq C_{\mbox{Dual}}\]

%Therefore, if we find any integral solution (even with congestion $c$), that routes at least $C_{\mbox{Dual}}/4$ pairs, for some feasible dual solution, then this means that our solution routes $\opt/4$ pairs with congestion $c$.

At the beginning of the algorithm, for every vertex $v\in V$, $x_v=0$. The length of a path $P$ is $\sum_{v\in P}x_v$.


Suppose we are given an oracle, that, in every iteration, produces a path $P\in \pset$, whose length is less than $1$ (in fact even an approximate oracle would work). Once such a path arrives, we add it to our solution. Assume that $a\in A'$ and $b\in B'$ are the endpoints of $P$. We set $x_a=x_b=1$. For every inner vertex $v\in V$, we update the value $x_v$ as follows. If $x_v=0$, then we set $x_v=1$; otherwise, we double it. Notice that in every iteration, the number of the paths we route increases by $1$, while the dual solution value increases by at most $4$.  Therefore, if $\pset'$ if the set of the paths that we have routed, then $|\pset'|\geq  C_{\mbox{Dual}}/4$. Notice that all paths in $\pset'$ have distinct endpoints. We now consider two cases.

The first case is when $|\pset'|\geq |A|/100$. In that case, we return the set $\pset'$ of paths. It is easy to see that the paths in $\pset'$ cause vertex-congestion at most $\log n/\alpha$ in $G$.

 Assume now that $|\pset'|<|A|/100$. We show a near-linear algorithm to compute a cut of sparsity at most $O(\alpha)$ in $G$.
Let $A''\subseteq A'$ and $B''\subseteq B;$ be the sets of vertices that are not routed by the paths in $\pset'$. Notice that $|A''|,|B''|>0.99n/2$,  and for all $v\in A''\cup B''$, $x_v=0$. We unify all vertices of $A''$ into a source $s$ and all vertices of $B''$ into a destination $t$. The current values $x_v$ for vertices $v\in H$ now define a valid solution to the minimum $s$-$t$ cut LP in this new graph. Moreover, for every vertex $v$, we can assume that all regular copies of $v$ have the same value $x_v$: otherwise, we can lower all these values to the smallest value of any copy. The value of this LP-solution is at most $4n/100$. By unifying all regular copies of each vertex $v$, we obtain a fractional solution to the $s$-$t$ cut problem of value $O(\alpha n)$. We can then use a random threshold cut to separate $s$ from $t$, obtaining a cut of value $O(\alpha n)$, that separates two subsets of $\Omega(n)$ vertices of $G$ from each other.

\subsection{The Oracle}
From now on, we need to construct an oracle, that in every iteration will return a path of length at most $1$, if such a path exists. We will use existing algorithms for decremental single-source shortest path. In all such algorithms, we are given a graph $G$ with a special source vertex $s$. We maintain the distances of all vertices from $s$ (possibly approximately), under edge deletion. 

Even though we have lengths on vertices and not on edges, we can define the length of every edge $e=(v,u)$ to be the sum of $x_u$ and $x_v$; this will distort the lengths by factor $2$ at most.

Using these algorithms on our modified graph $G'$ is too expensive. Instead, we do the following. We maintain a different graph $H$, defined on the same set of vertices as the original graph $G$. But now we replace each edge $(u,v)\in E(G)$ with $log^2n$ copies. So for edge $e=(u,v)$, for all $1\leq i,j\leq \log n$, we will have a copy $e_{i,j}$, whose cost is $2^i+2^j$. In every iteration, in graph $H$, we find a short $s$-$t$ path $P$. Once we find $P$, we donÕt delete its vertices. Instead, we update the whole graph, using the following rule:

Let $e=(u,v)$ be an edge in the $G$, and let $e_{i,j}$ be its copy. Edge $e_{i,j}$ remains in $H$ as long as $u$ has been used by fewer than $i/\alpha$ paths, and $v$ has been used by fewer than $j/\alpha$ paths. The moment either one of these vertices participates in more than this number of paths, we delete the edge $e_{i,j}$ from $H$. This simulates the exponential weight update of the $\alpha$ copies of $u$ and $v$: we will first use the cheapest copies, then the more expensive ones, and so on, and the length of the edge is the sum of weights of its endpoints.


 \mynote{this should go to one of previous sections}
A quick note on how we decide which edges to delete in the algorithm for vertex sparsest cut. 
Recall that our algorithm executes a number of phases, where in each phase, we choose an approximate shortest $s$-$t$ path $P$. We do not necessarily delete the edges of $P$ from the graph.
Recall that for each edge $e=(u,v)$ in the original graph $G$, we have added $\log^2n$ copies of $e$ to the new graph $G'$. For $1\leq i,j\leq \log^2n$, copy $e_{i,j}$ has weight $2^i+2^j$, and it is present in $G'$, as long as $v$ participates in fewer than $i/\alpha$ paths and $u$ participates in fewer than $j/\alpha$ paths. 
Throughout the algorithm, we maintain, for every vertex $v$ of $G$, a counter $p(v)$ that counts the number of paths in which $v$ participated so far. For each $1\leq i\leq \log n$, let $B_i(v)$ be the set of all edges of the new graph $G'$, that contains, for each edge $e=(u,v)$ of $G$ incident to $v$, the copies $\set{e_{i,j}\mid 1\leq j\leq \log n}$ of $e$. We add bi-directional links between the copies of $e_{i,j}$ in $B_i(v)$ and $B_j(u)$.

Once a path $P$ is chosen for the current phase, we perform procedure that we call \procetd, whose goal is to produce the set $E'$ of edges that need to be deleted from $G'$ in the current phase. Procedure \procetd updates the counters $p(v)$ for every vertex $v\in V(P)$. For every vertex $v\in P$, if $p(v)$ reaches an integral multiple of $1/\alpha$, say $i/\alpha$, all edges that currently belong to $B_i(v)$ are added to $E'$, to be deleted from $G'$. For each such edge $e_{i,j}$, where $e=(v,u)$, we  also delete $e_{i,j}$ from $B_j(u)$.
The running time of \procetd is proportional to the number of edges that are eventually added to the set $E'$, and deleted from $G'$. Therefore, over the course of the algorithm, we will spend at most $O(|E(G')|)=O(|E(G)|\cdot \log^2n)$ time on Procedure \procetd.

\mynote{end of part that needs to move to another section}




%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
\section{Application: Sparsest Cut with Capacities on Vertices}

%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
A vertex cut in a graph $G$ is  a partition $(A,X,B)$ of its vertices, so that there is no edge from $A$ to $B$, and $A,B\neq \emptyset$. The sparsity of the cut is $\frac{|X|}{\min\set{|A|,|B|}}$. The goal in the vertex sparsest cut problem is to compute a vertex cut of minimum sparsity.


Let $\alpha$ be our guess on the sparsity of the sparsest cut in our graph. At a high level, our algorithm will play the cut-matching game of KRV.  In every iteration, the cut player will produce a bi-partition of the vertices of $G$ into two equal-cardinality subsets, $A$ and $B$. Our algorithm will return one of the following:

\begin{itemize}
\item Either a vertex cut in $G$ of sparsity at most $\alpha\poly\log n$; or

\item A set $\pset$ of paths in $G$, connecting every vertex of $A$ to a distinct vertex of $B$, such that the paths cause vertex-congestion at most $\poly\log n/\alpha$ in $G$.
\end{itemize}

If, in any iteration of the algorithm, it returns a cut, then we are done. Otherwise, after $O(\log^2n)$ iterations, we embed a $1/2$-expander into $G$, with vertex-congestion at most $\poly\log n/\alpha$, therefore certifying that the value of the sparsest vertex cut in $G$ is more than $\alpha/\poly\log n$.

It is now enough to prove the following theorem.

\begin{theorem}\label{thm: main}
There is a near-linear time algorithm, that, given a partition $(A,B)$ of $V(G)$ into two equal-cardinality subsets, returns one of the following:

\begin{itemize}
\item Either a vertex cut in $G$ of sparsity at most $\alpha\poly\log n$; or

\item A set $\pset$ of $\Omega(n/\poly\log n)$ paths in $G$, connecting vertices of $A$ to vertices of $B$, such that the endpoints of the paths n $\pset$ are disjoint, and all paths in $\pset$ cause vertex-congestion at most $\poly\log n/\alpha$ in $G$.
\end{itemize}
\end{theorem}

Notice that by running the algorithm in the above theorem $\poly\log n$ times, we will either find a vertex cut in $G$ of sparsity at most $\alpha\poly\log n$, or a set $\pset^*$ of paths in $G$, connecting every vertex of $A$ to a distinct vertex of $B$, such that the paths cause vertex-congestion at most $\poly\log n/\alpha$ in $G$ (after every run we discard from $A$ and from $B$ the vertices that are already routed by the paths in $\pset$).

From now on we focus on proving the theorem.



\iffalse

\section{Getting Running Time $O(m/\alpha)$}
To get a running time of $O(m/\alpha)$, we use the Entropy-based algorithm for sparsest cut.  Again, we are trying to embed the expander $H$ into our graph $G$, using the cut-matching game. The algorithm consists of two phases. In the first phase, as long as $H$ contains sparse balanced cuts, we let $(A,B)$ be any such cut. Notice that if there is a collection of paths in $G$ routing $A$ to $B$ with vertex congestion at most $1/\alpha$, then most of these paths have length less than $1/\alpha$. So in the primal-dual scheme, we can restrict ourselves to only paths that have at most $1/\alpha$ hops, and, instead of starting with weights $1/n$, start with weights $\alpha$. This means that in the oracle, we can set the bound $D$ on the path length to roughly $1/\alpha$, and use the $O(mD)$-time algorithm for directed graphs.

Therefore, in every iteration of phase 1, we will return either a cut of sparsity $\alpha/\poly\log n$, or a routing of a large constant fraction of the vertices in $A,B$, on paths that cause congestion at most $\log n/\alpha$ in $G$. The first phase ends when every balanced cut in $G$ has $\Omega(n)$ edges. We then perform one more iteration, cutting off sparse cuts from $H$, until we get one large cluster with no sparse cuts. All sparse cuts that we cut off become the set $A$ (which can now have small cardinality), and the remaining vertices become $B$. 
In order to compute these sparse cuts, we use the paper of Racke for computing a hierarchical tree decomposition in near-linear time.

We now want to perform one more iteration, connecting the vertices of $A$ to vertices of $B$, with vertex-congestion at most $1/\alpha$.  But every vertex of $B$ should be connected to at most one vertex of $A$. Suppose such a set $\pset$ of paths exist. Then most of the paths in $\pset$ use at most $1/\alpha$ vertices of $A$. Let $\pset'$ be this set of paths. Next, we would like to argue that we can assume that most of these paths use at most $1/\alpha$ vertices of $B$. Let $v$ be any vertex of $B$. At most $1/\alpha$ paths of $\pset$ go through $v$. We will let $v$ randomly choose one of these paths to terminate at $v$, and the rest of them will be allowed to continue going through $v$. Using this procedure, if we take any $P\in \pset$, with high probability one of the first $\log n/\alpha$ of its vertices in $B$ has chosen $P$ to terminate there, so we can shorten $P$ to use at most $\log n/\alpha$ vertices of $B$.
\fi



==> decremental-sssp-backup.tex <==
\newpage
\section{Decremental Single-Source Shortest Paths}

Pointer to Bernstein's paper: "Deterministic Partially Dynamic Single Source Shortest Paths in Weighted Graphs", \url{https://arxiv.org/abs/1705.10097}


The goal of this section is to prove the following theorem that extends the results of Bernstein~\cite{Bernstein}.

\begin{theorem}\label{thm: decremental shortest path main}
There is a deterministic algorithm, that, given an undirected $n$-vertex graph $G=(V,E)$ with integral weights $w(e)\geq 1$ on edges $e\in E$, that is subject to edge deletions, and an error parameter $0<\eps<1$, maintains, for every vertex $v\in V$, a value $\delta(v)$, such that $\dist(s,v)\leq \delta(v)\leq (1+\eps)\dist(s,v)$, in total update time $O(n^2\poly\log n\log W/\eps^2)$, where $W=\max_{e\in E}\set{w(e)}$. Moreover, the algorithm can answer shortest-path queries that are interspersed with updates, in time $O(n\poly\log n)$ per query. In every query, the algorithm is given a vertex $v$ and needs to return a path from $s$ to $v$ in $G$, of length at most $(1+\eps)\dist(s,v)$.
\end{theorem}

%Throughout this section, the graphs we consider are undirected, and all algorithms are deterministic.
%In the decremental single-source shortest paths problem, we are given a graph $G=(V,E)$, a source vertex $s$, and weights $w_e> 0$ on the edges of $G$. In every iteration, some edge is deleted from $G$. We would like to maintain the (approximate) distances of all vertices from the source. We assume that all edge weights are integers between $1$ and $W$. Bernstein showed a deterministic algorithm, that maintains $(1+\eps)$-approximate distances from $s$ to every vertex in total update time $O(m\log^2n\log(nW)+n^2\log n\log(nW)/\eps^2)=\tilde{O}(n^2/\eps^2)$. 
%The drawback of his algorithm is that the data structure he maintains does not allow us to recover the path itself. In this section, we will try to rectify this drawback.
We note that Bernstein~\cite{Bernstein} showed a similar result, except that his algorithm cannot handle shortest-paths queries. Our algorithm follows his approach, and extends it to handle such queries.

%For convenience, we consider a simpler setting, which is sufficient for the vertex sparsest cut problem; it is possible that we can extend it to the general setting. In this restricted setting:

\begin{itemize}
\item For each edge $e$, the weight $w(e)$ is an integral power of $2$, and $1\leq w(e)\leq n$. 

\item In addition to the source vertex $s$, we also have a destination vertex $t$. Our algorithm performs $n$ iterations (that we call stages, to distinguish them from the iterations that happen inside each stage when the data structure gets updated). In every stage, we compute an (approximate) shortest $s$-$t$ path $P$ (with respect to the edge weights in the current graph), and then delete some of the edges incident to the vertices of $P$. For us, it is sufficient to get an $O(\log n)$-approximate shortest path, though the algorithm can probably be extended to a constant or $(1+\eps)$-approximation, by losing polylogarithmic factors in the running time.
\end{itemize}

A quick note on how we decide which edges to delete. 
Recall that in each phase, we choose an approximate shortest $s$-$t$ path $P$. We do not necessarily delete the edges of $P$ from the graph.
Recall that for each edge $e=(u,v)$ in the original graph $G$, we have added $\log^2n$ copies of $e$ to the new graph $G'$. For $1\leq i,j\leq \log^2n$, copy $e_{i,j}$ has weight $2^i+2^j$, and it is present in $G'$, as long as $v$ participates in fewer than $i/\alpha$ paths and $u$ participates in fewer than $j/\alpha$ paths. 
Throughout the algorithm, we maintain, for every vertex $v$ of $G$, a counter $p(v)$ that counts the number of paths in which $v$ participated so far. For each $1\leq i\leq \log n$, let $B_i(v)$ be the set of all edges of the new graph $G'$, that contains, for each edge $e=(u,v)$ of $G$ incident to $v$, the copies $\set{e_{i,j}\mid 1\leq j\leq \log n}$ of $e$. We add bi-directional links between the copies of $e_{i,j}$ in $B_i(v)$ and $B_j(u)$.

Once a path $P$ is chosen for the current phase, we perform procedure that we call \procetd, whose goal is to produce the set $E'$ of edges that need to be deleted from $G'$ in the current phase, and to update the data structure. Procedure \procetd updates the counters $p(v)$ for every vertex $v\in V(P)$. For every vertex $v\in P$, if $p(v)$ reaches an integral multiple of $1/\alpha$, say $i/\alpha$, all edges that currently belong to $B_i(v)$ are added to $E'$, to be deleted from $G'$. For each such edge $e_{i,j}$, where $e=(v,u)$, we may also need to delete $e_{i,j}$ from $B_j(u)$.
The running time of \procetd is proportional to the number of edges that are eventually added to the set $E'$, and deleted from $G'$. Therefore, over the course of the algorithm, we will spend at most $O(|E(G')|)$ time on Procedure \procetd.

Our algorithm follows the high-level framework of Bernstein, but modifies his algorithm and the data structure in a way that allows us to compute the approximate shortest path. The algorithm of Bernstein, as well as our extensions, rely on Even-Shiloach trees (ES-trees). In the next subsection, we describe ES-trees and a modification of these trees that Bernstein uses, and another new modification that we need. We then describe Bernstein's algorithm, followed by our extension.

\subsection{ES-Trees}
Even-Shiloach trees (ES-trees) are a data structure for decremental single-source shortest-path. Given a graph $G=(V,E)$ with weights $w(e)> 0$ on its edges, a source $s$, and a distance bound $D$, the data structure maintains, for every vertex $v$ with $d(s,v)\leq D$, the distance $d(s,v)$, under edge deletions. We denote the corresponding data structure, that we describe below, by $\EST(G,s,D)$.
The total running time, over all deletions, is $\tilde{O}(m\cdot D)$. We assume that all edge weights are integers, with the smallest edge weight at least $1$.



Throughout the algorithm, we maintain a shortest-path tree $T$ from $s$, up to distance $D$. The algorithm is partitioned into phases, where in every phase some edge is deleted from $G$, and the data structure is updated. Throughout the algorithm, every vertex $v$ has a label $\delta(v)$, whose value is exactly $d(s,v)$ (between updates; during an update, we will only guarantee that $\delta(v)\leq d(s,t)$).

For every vertex $v\in V$, we maintain a heap $H(v)$, that stores, for every neighbor $u$ of $v$, the vertex $u$ with the key $w(u,v)+\delta(u)$. Vertex $v$ has pointers to all its copies in the heaps of all its neighbors.

The main idea of the algorithm is: we inspect  or ``touch'' a vertex $v$ in three cases:

\begin{itemize}
\item If an edge incident to $v$ is deleted -- there can be at most $2m$ such inspections overall;

\item If $\delta(v)$ grows -- this can be done at most $D$ times per vertex, and overall the number of such inspections is bounded by $nD$. Each such inspection is charged to the vertex $v$; and

\item If $\delta(u)$ grows for one of the neighbors of $u$. Each vertex $u$, when $\delta(u)$ grows, may cause the inspection of up to $d(u)$ additional vertices. As $\delta(u)$ can grow at most $D$ times, overall, the number of such inspections is bounded by $\sum_{u\in V}D\cdot d(u)=O(mD)$. If we inspect $u$ because $\delta(v)$ increases for one of its neighbors $v$, we charge this inspection to the edge $(u,v)$, so every edge is charged at most $2D$ times.
\end{itemize}

Each inspection takes $\tau=O(\log n)$ time, and consists of a constant number of heap operations (return smallest-key element; delete an element; insert an element).


\paragraph{Initialization}
To initialize, we build a shortest-path tree $T$ from $s$, and compute the labels $\delta(v)$ for all vertices $v\in V$ along the way. We also initialize the heaps $H(v)$ for every vertex $v$. All this can be done in time $\tilde O(m)$.

\paragraph{Phases}
Consider a phase when some edge $e=(u,v)$ is deleted from the graph. If this edge does not belong to the current tree $T$, we don't need to do anything. So we assume that $e$ lies in the tree. Assume that $u$ is the father of $v$ in the tree. Then $\delta(v)$ may change, and this change may propagate to its subtree.
Let $T_v$ be the sub-tree of $T$ rooted at $v$.

Throughout the algorithm, we will maintain a heap $H$, containing vertices of $T_v$ that we need to inspect. The key stored with each vertex $x$ in $H$ is the current value $\delta(x)$. As the algorithm progresses, $\delta(x)$ may grow. We ensure that during the update, $\delta(x)\leq d(s,x)$ always holds. 
If a vertex $x$ does not belong to the heap $H$, then we have not changed $\delta(x)$ in this iteration yet. If it belongs to the heap, then it is possible that we have increased $\delta(x)$.
At the beginning, the heap $H$ is empty.

We start by inspecting the vertex $v$ (recall that an edge $e=(u,v)$ was deleted, and $u$ was the parent of $v$ in the tree). We inspect the first vertex $v'$ in the heap $H_v$, that is, a neighbor of $v$ minimizing $\delta(v')+w(v,v')$. If $\delta(v')+w(v,v')\leq \delta(v)$ (in which case equality must hold), then we know that $v'\in T\setminus T_v$ (all vertices $x\in T_v$ have $\delta(x)\geq\delta(v)$, as all edges have length at least $1$), and so $\delta(v)$ remains the same. We re-attach $v$ to the tree by connecting it to $v'$ and terminate the phase.

Otherwise, we know for sure that $\delta(v)$ increases by at least $1$. We increase $\delta(v)$ by $1$, and declare that $v$ is a \emph{changed} vertex. Notice that the new value of $\delta(v)$ is no more than $d(s,v)$, but it may be smaller than $d(s,v)$ - we do not know this yet. We add $v$ to the heap $H$, and we also add all its children to $H$, which 
are now called \emph{suspicious} vertices. We also update the key of $v$ in the heaps $H_x$ of all its neighbors $x$, to reflect the change in $\delta(v)$.

In general, throughout the algorithm, the vertices $x$ of $T_v$ can be in one of the following four statuses:

\begin{itemize}
\item Untouched: we have never inspected $x$, and it is not currently attached to the tree $T$; we do not know if $\delta(x)$ increased;
\item Settled: we attached $x$ to the tree, and its current value $\delta(x)=d(s,x)$ in the new graph;
\item Suspicious: We have added $x$ to the heap $H$ but we did not inspect it yet, and $\delta(x)$ has not changed yet. However, if $y$ is the parent of $x$, then $\delta(y)$ has increased. A suspicious vertex is not currently attached to the tree; and
\item Changed: we have increased $\delta(x)$ in the current iteration, but we do not yet know the value of $d(s,x)$. All changed vertices belong to $H$, and a changed vertex is not attached to the tree.
\end{itemize}

In every iteration, we inspect a vertex $x$ from the heap $H$, with the smallest key $\delta(x)$. Let $y\in H_x$ be the vertex minimizing $\delta(y)+w(x,y)$. If $\delta(y)+w(x,y)\leq \delta(x)$ (which must hold with equality), then we attach $x$ to the tree through $y$, and declare it a settled vertex.  (We will show later that $y$ must be currently attached to $T$, and so $\delta(y)=d(s,y)$.)  Note that if $x$ was not yet inspected in this iteration, that is, we never changed $\delta(x)$, then all its descendants are untouched, and they get attached to the tree together with $x$. In that case, all descendants of $x$ become settled vertices. Otherwise, $x$ was a changed vertex at the beginning of this iteration, and so all its children lie in the heap $H$. We do not reattach any of its descendants to the tree then.

Otherwise, if $\delta(y)+w(x,y)> \delta(x)$, we know that the current estimate of $\delta(x)$ is too small. We then increase $\delta(x)$ by $1$ and return $x$ to $H$. If this is the first time that $\delta(x)$ is increased in the current iteration, then it becomes a changed vertex, and all its children in the tree $T_v$ become suspicious and are added to the heap $H$. In any case, we update the key of $x$ in the heaps $H_z$ for all neighbors $z$ of $x$.

Notice that, when $x$ is inspected, if $\delta(x)$ increases, then we need to spend $O(\log n)\cdot d(x)$ time to update all the heaps $H_z$ of its neighbors, and $O(\log n)$ time to find the first vertex on $H_x$. Additionally, for every child of $x$ that becomes suspicious but never becomes changed, we charge the processing time of that child to $x$. Whenever a suspicious vertex is inspected, and it becomes settled (so it never becomes changed), the corresponding processing time is $O(\log n)$, and it is charged to the edge connecting it to its (changed) parent in the tree. We do not need to explicitly update the status of its descendants to ``settled''; the algorithm naturally ensures that these vertices are never added to $H$.


Pictorially, if we look at the sub-tree $T_v$ of the original tree $T$ rooted at $v$, then the vertices that were added to $H$ so far (not the vertices currently in $H$; the vertices that have been added throughout this phase) are a connected sub-tree of $v$, including $v$. Let us denote this sub-tree by $T'$. The leaves of $T'$ are the vertices whose distance from $s$ has not yet changed -- these are the suspicious vertices (some of them may be settled); the inner vertices are those whose distances have increased already -- these are the changed vertices (some of them may now be settled). Therefore, if any vertex $x$ is untouched (but not settled), then it has an ancestor that is suspicious, and currently belongs to the heap $H$.

It remains to show that, if $x$ is a vertex of $H$ with minimum $\delta(x)$, and $y\in H_x$ is the vertex minimizing $\delta(y)+w(x,y)$, with $\delta(y)+w(x,y)=\delta(x)$ then $y$ is a settled vertex, or $y\in T\setminus T_v$. Assume otherwise. Then either $y\in H$, or $y$ is untouched. If $y\in H$, then $\delta(y)\geq \delta(x)$, and, since $w(x,y)\geq 1$, it is impossible that $\delta(y)+w(x,y)=\delta(x)$. Therefore, $y$ is untouched. But then $y$ has a suspicious ancestor $y'$ in the heap, with $\delta(y')<\delta(y)$. Since we chose $x$ in the current iteration, $\delta(x)\leq \delta(y')<\delta(y)$, a contradiction.

The update algorithm terminates once one of the following two things happen: either the heap $H$ becomes empty, in which case we have updated the tree successfully and can continue to the next phase; or for the vertex $x$ at the top of the heap $H$, $\delta(x)>D$ holds. In the latter case, 
We know that for every vertex $y$ of $T_v$ that is not settled yet, $d(s,y)>D$. We discard all vertices that are not currently attached to the tree $T$ and continue to the next phase.


In one of our algorithms, we will choose the bound $D$ in such a way that, if $G'$ is connected, then for every vertex $x$, $d(s,x)\leq D$. If the update algorithm terminates with not all vertices attached to $T$, then we know that the graph has become disconnected. But since we have only deleted one edge $(u,v)$ in the current iteration, we know that the connected components are induced by $V(T\setminus T_v)$ and $V(T_v)$. Moreover, $T\setminus T_v$ is the shortest-distance tree from $s$ for the first component, and $T_v$ is the shortest-distance tree from $v$ for the second component. We will use this fact later.


\subsection*{Extension 1: Edge Insertion}
The ES-trees support edge insertion, if the insertion does not shorten any distances. If we would like to insert such an edge $e=(u,v)$, then the tree $T$ does not change. We update the heaps $H_u$ and $H_v$ by inserting $v$ into the first heap and $u$ into the second. All this takes $O(\log n)$ time per insertion. %Overall, if we denote by $m$ the total number of edges that ever appear in $G'$ (that is, both the original edges and the inserted edges), then the total running 

We now analyze the whole running time, with edge insertions.

Let $E_0$ be the set of all edges that were present in the original graph, and let $E_1$ be the set of all edges that were inserted through the edge-insertion procedure. We denote $m=|E_0\cup E_1|$. Note: if an edge is deleted and then inserted back, then we count this as two different edges.

Recall that $\eta=O(\log m)$ is the time that the ES procedure spends on inspecting one vertex $x$ (this involves a constant number of standard operations to the heap $H_x$).
For every vertex $v$ in the current graph, we define its potential of $v$ to be: $\phi(v)=(D+1-\delta(v))\cdot d(v)\cdot \eta$. Let the total current potential in graph $G$ be $\phi=\sum_{v\in V(G)}\phi(v)$.

\paragraph{Edge-Deletion.} After each edge-deletion operation, the amount of time spent on the update is equal to the decrease of the potential: we inspect the first vertex $v$, which takes time $\eta$, but the potential of $v$ decreases by at least $\eta$, since its degree decreases by $1$. For every vertex $x$, if $\delta(x)$ decreases by $\Delta$, then we spend $\Delta\eta d(x)$ time on $x$ (we inspect it up to $\Delta$ times; each time we update the heaps $H_z$ of their neighbors; we also need to pay for inspecting those neighbors whose distance from $s$ did not increase). 
The potential of $x$ decreases by $\Delta\eta d(x)$, so the time spent on the update is bounded by the total decrease in the potential.


\paragraph{Edge-Insertion.} After each edge-insertion operation, the potential increases by at most $2D\eta$, as the endpoints of the inserted edge $e$ may have their potential increase by $D\eta$ each. The amount of time we spend on a single edge insertion is $2\eta$. 


The total running time of the algorithm is bounded by the original potential at the start of the algorithm, plus all increases in the potential due to edge insertions, plus $O(|E_1|\eta)$ -- we may spend up to $\eta$ update time per edge insertion. 

We conclude that the total running time of the algorithm, over the course of all edge deletions, and edge insertions is at most $O(Dm\log m)$. 







\subsection*{Extension 2: Weighted Graphs}
One unfortunate property of the ES algorithm is that its total running time is $O(mD)$.  Bernstein's algorithm uses the ES-trees only in a sub-graph of the original graph $G$, where large-degree vertices are deleted. If the graph were unweighted, we could use a threshold $\tau=n/D$, and ignore all vertices whose degree is greater than $\tau$ -- such vertices are taken care of by an auxiliary structure. The total running time of the ES algorithm then becomes $O(mD)=O(n\tau D)=O(n^2)$. However, when edges have large weights, in order to ensure that the algorithm always returns a good approximation to the distances from the source $s$, we need to set the threshold $\tau$ differently for different weight classes. Because of this, for each $i$, we may have up to $n^2\cdot 2^i/D$ edges of weight $2^i$ in the resulting graph. Bernstein modifies the ES-trees, so that edges of greater weight contribute less to the running time of the algorithm, at the cost of maintaining the shortest paths approximately. The time is the sum of $O(nD)$ and $\sum_{e\in E_0\cup E_1}\frac{D}{\eps w(e)}$. This is perfect for us, because we will have up to $n^22^i/D$ edges of weight $2^i$. His algorithm allows edge deletions and insertion of edges that do not increase distances from $s$. It also allows increase in edge weights, but we do not need this part. The algorithm is called WSES (weight-sensitive Even-Shiloach).

Below is a restatement of Lemma 4.3 from [Bernstein]

\begin{lemma}\label{lem: WSES}
Let $G$ be an undirected graph with positive integer edge weights, a source $s$ and a bound $D\geq 1$. Suppose $G$ is subject to edge deletions and edge insertions, such that the distances in $G$ never decrease as a result of an update. Then there is an algorithm $WSES(G,D,s)$, that maintains approximate distances $d'(s,v)$, such that for every vertex $v$, as long as $v$ is in the tree $T$,

\[d(s,v)\leq d'(s,v)\leq (1+\eps)d(s,v),\]

and the total update time is $O(nD)+O\left (\sum_{e\in E_0\cup E_1}\frac{D}{\eps w(e)}\right )$. (Here, as before, $E_0$ is the original set of edges of $G$, and $E_1$ is the set of edges that were ever inserted). Vertex $v$ is only deleted from the tree $T$ when $d(s,v)>D$.
\end{lemma}

Notice that if all edge weights are unit, then the running time becomes $O(mD)$ as before. But if many edges have large weights, we may save on the running time.

The algorithm WSES actually also allows us to find the approximate shortest $s$-$t$ path, even though the above lemma does not state that.
\mynote{The rest can be skipped; it repeats Bernstein paper; this is mostly to make sure I understand this part well}

The lemma is proved by modifying the ES algorithm. Recall that the original ES algorithm stored, together with every vertex $v$, a value $\delta(v)$, which was the distance from $s$ to $v$. Now we will no longer ensure that $\delta(v)=d(s,v)$. Instead we ensure the following: between updates, the values $\delta(v)$ for $v\in V$ will have the following two properties:

\begin{properties}{I}
\item If $v=s$, then $\delta(v)=0$. Otherwise, if $p$ is the parent of $v$ in the current tree $T$, then $\delta(v)\geq \delta(p)+w(p,v)$; and \label{inv1: father}
\item For every neighbor $u$ of $v$, $\delta(v)\leq \delta(u)+(1+\eps)w(u,v)$. \label{inv1: neighbor}
\end{properties}

We first show that, if the above invariants are maintained, then we indeed maintain approximate shortest paths from $s$.

\begin{claim}\label{claim: approx}
Assume that the values $\delta(v)$ for $v\in T$ obey the above invariants. Then for each $v\in T$, $d(s,v)\leq \delta(v)\leq (1+\eps)d(s,v)$.
\end{claim}
\begin{proof}
To see that $\delta(v)\geq d(s,v)$, we simply follow the path in the tree $T$ from $v$ to $s$. From the first invariant, $\delta(v)$ is at least the sum of weights of edges along this path, which is at least $d(s,v)$. We now turn to prove that $\delta(v)\leq (1+\eps)d(s,v)$.

The proof is by induction on the number of edges in the shortest path from $s$ to $v$. If the shortest path contains just one edge $e$, then 
$\delta(v)\leq \delta(s)+(1+\eps)w(e)$. Assume now that the shortest $s$-$v$ path has $i>1$ edges, and let $u$ be the penultimate vertex on this path. Then $d(s,v)=d(s,u)+w(u,v)$. From the induction hypothesis, $\delta(u)\leq (1+\eps)d(s,u)$. From the second invariant, $\delta(v)\leq \delta(u)+(1+\eps)w(u,v)\leq (1+\eps)d(s,u)+(1+\eps)w(u,v)=(1+\eps)d(s,v)$.
\end{proof}



\begin{definition}
Let $e$ be an edge and let $x$ be an integer. $\round_e(x)$ is the smallest integer $y>x$ that is an integral multiple of $\eps w(e)$.
\end{definition}


Recall that in the ES-procedure, whenever $\delta(v)$ increases, we immediately update the copies of $v$ in the heaps $H_u$ of its neighbors to reflect this change. In the modified algorithm, every neighbor $u$ of $v$ will keep a copy $\delta_u(v)$ of the value $\delta(v)$, that is not necessarily up to date. We replace the invariants~\ref{inv1: father} and \ref{inv1: neighbor} with the following two approximation invariants, that hold for every vertex $v$:

\begin{properties}{A}
\item If $v=s$, then $\delta(v)=0$. Otherwise, let $u$ be the parent of $v$ in the tree. Then $\delta(v)=\delta_v(u)+w(u,v)$. (that is, we use the approximate local estimate on $\delta(u)$ in order to establish $\delta(v)$). Moreover, $u$ is the neighbor of $v$ with minimum $\delta_v(u)+w(u,v)$.
\label{inv2: approx father}


\item If $u$ is a neighbor of $v$, then $\delta(u)\leq \delta_v(u)\leq \round_{e=(u,v)}(\delta(u))$.\label{inv2: approx neighbor}
\end{properties}


Observe that, if Invariants~\ref{inv2: approx father} and \ref{inv2: approx neighbor} hold, then so do Invariants~\ref{inv1: father} and \ref{inv1: neighbor}. Indeed, Invariant~\ref{inv1: neighbor} follows immediately from Invariant~\ref{inv2: approx father}, and from the fact that $\delta_v(u)\geq \delta(u)$. For Invariant~\ref{inv1: neighbor}, denote $e=(u,v)$, and observe that:

\[\delta(v)\leq \delta_v(u)+w(e)\leq \round_e(\delta(u))+w(e)\leq \delta(u)+(1+\eps)w(e).\]

Therefore, it is now enough to maintain Invariants~\ref{inv2: approx father} and \ref{inv2: approx neighbor}.


In order to obtain the improved running time, we implement the following changes:

\begin{itemize}
\item Whenever $\delta(v)$ increases, we can inspect it, and charge the vertex for the inspection. However, we do not immediately inspect its neighbors. The number of such inspections is bounded by $nD$.

\item Let $e=(u,v)$ be an edge. We charge this edge (by inspecting both its endpoints) only if $\round_e(\delta(u))$ increases or $\round_e(\delta(v))$ increases. The number of such  charges to edge $e$ is bounded by $\frac{D}{\eps w(e)}$, and the total number of such inspections is bounded by $\sum_e\frac{D}{\eps w(e)}$.
\end{itemize}

We now describe an update operation, when an edge $(u,v)$ of the tree $T$ is deleted, where $u$ is the parent of $v$. As before, we maintain a heap $H$, to which we add all vertices that need to be inspected. We start with $H$ containing just the vertex $v$. In every iteration, we remove the vertex $x$ from the heap $H$ with smallest $\delta(x)$. We then consider, the vertex $y\in H_x$ with minimum $\delta_x(y)+w(x,y)$. If this value is no more than $\delta(x)$, then $y$ must be currently attached to the tree $T$, as we will see later. We attach $x$ to $y$.
Otherwise, we increase $\delta(x)$ by $1$. For every neighbor $z$ of $x$ for which $\round_{e=(x,z)}(\delta(x))$ increases, we update the value $\delta_z(x)$ of $x$ in the heap $H_z$ to be $\delta(x)$; if additionally $z$ is a child of $x$ in the tree $T$, then we add $z$ to the heap $H$.


Notice that throughout the algorithm, if a vertex $y$ of $T_v$ is not on the heap $H$ and is not attached to the tree $T$, then it has an ancestor $y'$ in $H$. From Invariants~\ref{inv2: approx father} and \ref{inv2: approx neighbor}, that ancestor has $\delta(y')<\delta(y)$. If $y$ is at the top of the heap $H_x$ and $\delta_x(y)+w(x,y)\leq \delta(x)$, then we know that $\delta(y)\leq \delta_x(y)<\delta(x)$, so $\delta(y')<\delta(x)$, and we should have processed $y'$ and not $x$. This concludes the correctness analysis.

Notice that when $\delta(x)$ increases, we need to be able to quickly figure out which edges incident to $x$ to process. This is implemented as follows. Each vertex $x$ has $m$ buckets. The $i$th bucket contains all edges $e$ incident to $x$, for which $\round_e(i)\neq \round_e(i+1)$. So whenever $\delta(x)$ decreases from $i+1$ to $i$, we need to inspect and charge all edges in the $i$th bucket. To initialize, each vertex creates $D$ buckets, which takes $O(nD)$ time. After that, each edge $e$ adds itself to the relevant buckets of its two endpoint: $D/\eps w(e)$ buckets per endpoint. So the total time to initialize the buckets is $O(nD)+O(\sum_e\frac{D}{\eps w(e)})$. Once the buckets are initialized, we don't need to do anything to maintain them, except inserting/deleting edges. 

One last part is edge insertion, which turns out to be tricky. Suppose we would like to insert an edge $e=(u,v)$, where $d(s,u)=1000$, $d(s,v)=1000$, and $w_e=1$. This insertion does not decrease distances. But because we maintain approximate distances from $s$, we may have $\delta(u)=1000$ and $\delta(v)=1000(1+\eps)$. We need to insert a copy $\delta_v(u)$ of $u$ into the heap of $v$, and it is not clear how to do this while maintaining the invariants. In particular, we are not allowed to let $\delta(v)$ decrease, since this will ruin our analysis.

The solution is a bit weird. (Below is my implementation of the idea that was sketched in Bernstein's paper; he refers to other papers for more details; I did not read them).

 Assume that we insert an edge is $e=(u,v)$ and that $\delta(u)\leq \delta(v)$. We add a copy $\delta_u(v)=\delta(v)$ to $H_u$ as usual, and add $e$ to all the relevant buckets of $u$. All invariants continue to hold.
 If $\delta(u)+w(u,v)\geq \delta(v)$, then we also add a copy $\delta_v(u)=\delta(u)$ to $H_v$ as usual and add $e$ to all the relevant buckets of $v$. However, if $\delta(u)+w(u,v)< \delta(v)$, then we say that $(e,v)$ is a \emph{problematic pair}, and we set $\delta_v(u)=\delta(v)-(u,v)$. We will not update this value $\delta_v(u)$ until $\delta(u)$ becomes greater than $\delta_v(u)$, at which point $(e,v)$ will stop being a problematic pair, and we will add $e$ to the relevant buckets of $v$, and continue as usual. But notice that, while $(e,v)$ remains a problematic pair, $\delta(v)$ will not grow, as $v$ can always connect to the tree through $u$. The intuitive idea for why this work is that the original value $\delta(v)$ was a $(1+\eps)$-approximation on $d(s,v)$, and, as long as $\delta(u)\leq \delta(v)-w(u,v)$, we know that $d(s,v)\leq \delta(v)$. Since the distances never decrease, we maintain a $(1+\eps)$-approximation.

The problem is that this change completely messes up our invariants, and we need to redo them. 
Invariant \ref{inv2: approx father} continues to hold. Invariant \ref{inv2: approx neighbor} holds for  all pairs $(e,v)$ where $(e,v)$ is not a problematic pair. But if $(e,v)$ is a problematic pair, then we are only guaranteed that: 

\[\delta(u)\leq \delta_v(u).\]


We now define a new set of basic invariants that hold throughout the algorithm.


\begin{properties}{I}
\item If $v=s$, then $\delta(v)=0$. Otherwise, if $p$ is the parent of $v$ in the current tree $T$, then $\delta(v)\geq \delta(p)+w(p,v)$; \label{inv12: father}
\item Let $u$ be a neighbor of $v$, and let $e=(u,v)$  be the corresponding edge. If $(e,v)$ is not a problematic pair, then $\delta(v)\leq \delta(u)+(1+\eps)w(u,v)$. \label{inv12: neighbor}
\end{properties}



\begin{claim}\label{claim: approx}
Throughout the algorithm, for each $v\in T$, $d(s,v)\leq \delta(v)\leq (1+\eps)d(s,v)$.
\end{claim}
\begin{proof}
As before, to see that $\delta(v)\geq d(s,v)$, we simply follow the path in the tree $T$ from $v$ to $s$. From the first invariant, $\delta(v)$ is at least the sum of weights of edges along this path, which is at least $d(s,v)$. We now turn to prove that $\delta(v)\leq (1+\eps)d(s,v)$.

The proof is by induction on time and the number of edges in the shortest path from $s$ to $v$. 
When the algorithm starts, for every vertex $v$, $\delta(v)=d(s,v)$. We now consider the state of the algorithm after some iteration $j$, and consider the shortest $s-v$ path.
If this path contains no edges, then $\delta(s)=0$, and we are done.  Assume now that the shortest $s$-$v$ path has $i>0$ edges, and let $u$ be the penultimate vertex on this path. 
Then $d(s,v)=d(s,u)+w(u,v)$.
Let $e=(u,v)$ be the corresponding edge. Assume first that $(e,v)$ is not a problematic pair.
From the induction hypothesis, $\delta(u)\leq (1+\eps)d(s,u)$. From the second invariant, $\delta(v)\leq \delta(u)+(1+\eps)w(u,v)\leq (1+\eps)d(s,u)+(1+\eps)w(u,v)=(1+\eps)d(s,v)$.

Finally, assume that $(e,v)$ is a problematic pair. 
When $e=(u,v)$ is added to the graph, $ \delta(v)\leq (1+\eps)d(s,v)$ held, from the induction hypothesis. As long as $(e,v)$ remains a problematic pair, $\delta(v)$ does not grow, but $d(s,v)$ may increase. Therefore, $\delta(v)\leq (1+\eps)d(s,v)$ continues to hold. 
\end{proof}


\paragraph{Final Running Time Analysis}
Let $E_0$ be the set of edges that were present from the beginning, and $E_1$ the set of edges that were inserted over the course of the algorithm. Then the total running time of the algorithm is: $O(nD)+O(\sum_{e\in E_0\cup E_1}\frac{D}{\eps w(e)})$.



\subsection*{Extension 3: Vertex Splitting}
The algorithm of Bernstein uses the following setting, that we will also use several times. We are given a basic graph $G$, and additionally a collection $\cset=\set{C_1,\ldots,C_r}$ of  disjoint subsets of its vertices, each of which contains at least two vertices. We need to maintain a graph $\hat G$, that is defined as follows. Its set of vertices consists of two subsets: $V_1=V(G)$, and $V_2=\set{v_C\mid C\in \cset}$. We call the vertices of $V_1$ \emph{regular vertices}, and the vertices of $V_2$ \emph{super-nodes}. The set of edges also consists of two subsets: set $E_1$ of edges contains all edges of $G$, with the same weights (that we assume to be integers between $1$ and $W$), and set $E_2$ of edges is defined as follows: for every super-node $v_C$, for every regular vertex $u\in C$, we add an edge $(u,v_C)$ of weight $1/2$ to $\hat G$. Therefore, every edge of $E_2$ connects a super-node to a regular vertex, and the sum of degrees of all super-nodes is $|E_2|\leq n$. Over the course of the algorithm, some sets $C\in \cset$ may be split into smaller subsets. This will require to split the corresponding super-node $v_C$. The edges in set $E_1$ are called type-1 edges, and the edges in set $E_2$ are called type-2 edges.



The input to the vertex splitting operation consists of a single set $C\in \cset$, and a subset $C'\subseteq C$ containing at most $|C|/2$ vertices. The idea is that we replace $C$ by two subsets: $C'$ and $C''=C\setminus C'$, and update the graph accordingly: that is, we rename $v_C$ by $v_{C''}$; insert a new vertex $v_{C'}$, that connects to every vertex of $C'$ with an edge of weight $1/2$, and delete all edges connecting $v_{C''}$ to the vertices of $C'$. The input is given as follows: we are only given a pointer to the vertex $v_C$ corresponding to the set $C$; the names $C',C''$ of the new sets into which $C$ is split; and an explicit list of the vertices of $C'$. Note that it is possible that $C'$ becomes a singleton vertex, in which case the update operation does not create a new vertex $v_{C'}$, but instead simply deletes the edge $(v_C,u)$, where $u$ is the unique vertex of $C'$.

%Let $v_C\in V_2$ be a super-node, and let $N(v)$ be the set of its neighbors. A \emph{split pattern} consists of an integer $r>1$ (the arity of the split), and a partition $S_1,S_2,\ldots,S_r$ of $N(v)$ into $r$ non-empty subsets, where for all $1<i\leq r$, $|S_1|\geq |S_i|$. In the corresponding split operation, we modify the current graph $G$, so that $v$ is deleted; $r$ new vertices $v_1,\ldots,v_r$ are inserted (the new vertices are all super-nodes and may be split again later); and for each $1\leq i\leq r$, vertex $v_i$ connects to all vertices of $S_i$; for each $x\in S_i$, the weight of the new edge $(v_i,x)$ is $1/2$. We think of the edge $(x, v_i)$ as being an identical copy of edge $(x,v)$, so we do not view this as edge deletion/insertion. Let $\hat G'$ be the graph obtained from the current graph $\hat G$ after the split.

 Bernstein says that an algorithm that can handle edge insertions/deletions can also handle vertex splits. He does not provide details, but points to other papers. Below are my attempts to fill in the details without reading those other papers.

We will maintain an augmented graph $G'$. Graph $G'$ contains all vertices and edges of $\hat G$. Additionally, for every super-node $v_C\in V_2$, 
we have $\ceil{4|C|\log |C|}$ extra copies of $v_C$; we denote this set of extra copies by $X(v_C)$. Each such extra-copy connects to $v$ with an edge of length $1$. The latter set of edges is denoted by $E_3$, and we call all edges in this set \emph{type-3 edges}. Whenever we would like to split some super-node $v_C$ using a subset $C'\subseteq C$ of at most $|C|/2$ vertices, we implement the split by a number of edge insertion and edge deletion operations.

First, we pick an arbitrary vertex of $X(v)$, that we denote by $v_{C'}$, and we rename $v_C$ as $v_{C''}$. We do the following edge-insertion operations:

\begin{itemize}
\item For every vertex $x\in C'$, insert the edge $(v_{C'},x)$ of weight $1/2$;

\item Select an arbitrary subset $X(v_{C'})$ of $\ceil{4|C'|\log |C'|}$ distinct vertices of $X(v_{C})$; denote this set of vertices by $X(v_{C'})$. Connect $v_{C'}$ to each such vertex with an edge of weight $1$.
\end{itemize}

Note that these insertions do not decrease the distances between vertices, and we insert at most $|C'|+1\leq |C|/2+1$ new edges into the graph.

We then perform the following deletion operations:

\begin{itemize}
\item For all $x\in C'$, delete the edge $(x,v_{C''})$; 
\item For all $x\in X(v_{C''})\setminus (X(v_{C'}))$, delete the edge $(x,v_{C''})$; 
\item If $X(v_{C''})$ contains more than $\ceil{4|C''|\log |C''|}$ vertices, select an arbitrary subset of $\ceil{4|C''|\log |C''|}$ vertices of $X(v_{C''})$; for each remaining vertex $x$, we delete the edge $(v_{C''},x)$ from the graph, and we discard $x$ from $X(V_{C''})$; and
\item Delete the edge $(v_{C'},v_{C''})$.
\end{itemize}

The number of edge insertions in one vertex split operation is bounded by $|C'|+1$, but $|C'|\leq |C|/2$. Therefore, the total number of edges that can be inserted over the course of the algorithm due to vertex splitting is bounded by $O(n\log n)$. If $m'$ denotes the total number of edges inserted directly through edge-insertion operations, then the total running time is $\tilde O((m+m'+n\log n)D)$.

We will also need to combine vertex splitting with the algorithm of Lemma~\ref{lem: WSES}.  We will do this accounting later.



\iffalse
Let $v\in V_2$ be a super-node, and let $N(v)$ be the set of its neighbors. A \emph{split pattern} consists of an integer $r>1$ (the arity of the split), and a partition $S_1,S_2,\ldots,S_r$ of $N(v)$ into $r$ non-empty subsets, where for all $1<i\leq r$, $|S_1|\geq |S_i|$. In the corresponding split operation, we modify the current graph $G$, so that $v$ is deleted; $r$ new vertices $v_1,\ldots,v_r$ are inserted (the new vertices are all super-nodes and may be split again later); and for each $1\leq i\leq r$, vertex $v_i$ connects to all vertices of $S_i$; for each $x\in S_i$, the weight of the new edge $(v_i,x)$ is $1/2$. We think of the edge $(x, v_i)$ as being an identical copy of edge $(x,v)$, so we do not view this as edge deletion/insertion. Let $\hat G'$ be the graph obtained from the current graph $\hat G$ after the split.

 Bernstein says that an algorithm that can handle edge insertions/deletions can also handle vertex splits. He does not provide details, but points to other papers. Below are my attempts to fill in the details without reading those other papers.

We will maintain an augmented graph $G'$. Graph $G'$ contains all vertices and edges of $\hat G$. Additionally, for every super-node $v_C\in V_2$, 
we have $|C|\log |C|$ extra copies of $v_C$; we denote this set of extra copies by $X(v_C)$. Each such extra-copy connects to $v$ with an edge of length $1$. Whenever we would like to split some super-node $v$ according to a split patter $(S_1,\ldots,S_r)$, we implement the split by a number of edge insertion and edge deletion operations.

First, we pick $r-1$ arbitrary vertices of $X(v)$, that we denote by $v_2,\ldots,v_r$, and we rename $v$ as $v_1$. We do the following Insert operations:

\begin{itemize}
\item For each $2\leq i\leq r$, for every vertex $x\in S_i$, add the edge $(v_i,x)$ of weight $1/2$;

\item For each $2\leq i\leq r$, select $|S_i|\log(|S_i|)$ distinct vertices of $X(v)$; denote this set of vertices by $X(v_i)$. Connect $v_i$ to each such vertex with an edge of weight $1$.
\end{itemize}

Note that these insertions do not decrease the distances between vertices. Moreover, if we denote $n'=|S_2|+|S_3|+\cdots+|S_r|$, then we insert $2n'$ new edges into the graph.

We then perform the following deletions operations:

\begin{itemize}
\item For all $x\in N(v)\setminus B_1$, delete the edge $(x,v)$; and
\item For all $x\in X(v)\setminus (X(v_1)\cup X(v_2)\cdots \cup X(v_r))$, delete the edge $(x,v)$.
\end{itemize}

The number of edge insertions in one vertex split operation is bounded by $n'=\sum_{i=2}^r|S_i|$. However, for $2\leq i\leq r$, $|S_i|\leq |N(v)|/2$. Therefore, each original edge of $E_2$ may participate in at most $2\log n$ splittings of its endpoints. The total number of edge insertions due to vertex splittings is then at most $O(n\log n)$. If $m'$ denotes the total number of edges inserted directly through edge-insertion operations, then the total running time is $O((m+m')\log^2(m+m'))$.

We will need to combine vertex splitting with the algorithm of Lemma~\ref{lem: WSES}.  We will do this accounting later.
\fi

%---------------------------------------------------
%---------------------------------------------------
%---------------------------------------------------
%---------------------------------------------------
\subsection{The Algorithm of Bernstein}
The following definitions are central to the algorithm. First, for every edge $e$, we let $\level(e)=\floor{\log w(e)}$ (in our case, all edges will have weights $2^i$ for integers $i$; the level of such an edge is $i$).

Given a vertex $v\in V(G)$, we denote by $I_i(v)$ the set of all edges of levels $1,2,\ldots,i$ that are incident to $v$, and by $I(v)$ the set of all edges incident to $v$.

Throughout, we assume that we are given some value $D$, and our goal is to approximately preserve the distances of all vertices from $s$, but only for those vertices $v$ with $D\leq d(s,v)\leq 2D$. (In our application, we are only interested in preserving the distance from $s$ to $t$, so we can assume that $D$ is the current estimate on this distance. Once the distance grows beyond $2D$, we can recompute the whole data structure from scratch). We use a threshold parameter \fbox{$\tau=\frac{3n\log n}{\eps D}$}.

For a vertex $v$, we let $\cutoff(v)$ be the largest integer $i$, such that $|I_i(v)|\geq \tau 2^i$. If no such index exists, we set  $\cutoff(v)=0$. Assume now that $\cutoff(v)=i$. We say that $v$ \emph{owns} all edges of $I_i(v)$, and all edges of $I_i(v)$ are called \emph{heavy} edges. Note that a heavy edge must be owned by at least one of its endpoints; but it can be owned by both endpoints.

Next, we define two graphs. The first graph, $G^H$ (called \emph{heavy graph}) contains all vertices of $G$ and all heavy edges of $G$. 
Let $\cset$ be the set of all connected components of $G^H$.
The second graph, $G^L$ (called \emph{light graph}) is defined as follows. The set of its vertices contains all vertices of $G$ -- we denote this set of vertices of $V_1$, and, for each $C\in \cset$, a \emph{super-node} $v_C$ -- we denote the set of all super-nodes by $V_2$. The set of edges also consists of two subsets. First, we add to $G^L$ all light edges of $G$, with their original weight; denote this set of edges by $E_1$. Notice that every edge of $E_1$ connects a pair of vertices of $V_1$. Next, for each connected component $C\in \cset$, we add an edge of weight $1/2$ between every vertex of $v$ and $v_C$ - we denote this set of edges by $E_2$.

\paragraph{Data Structures}
We maintain the graphs $G^H$ and $G^L$. Notice that, as the algorithm progresses, both graphs may change. For example, a heavy edge may become light, and we may need to delete it from $G^H$ and insert it into $G^L$. Also, a connected component of $G^H$ may get split, and we may need to split the corresponding super-node of $G^L$. Notice that we will only split the vertices of $V_2$, and we will only insert edges connecting pairs of vertices in $V_1$. These insertions do not decrease distances: suppose an edge $e=(u,v)$ stopped being heavy, and needs to be inserted into $G^L$. Before the insertion, $u$ and $v$ belong to the same connected component $C$ of $\cset$. So graph $G^L$ contains edges $(u,v_C)$, $(v,v_C)$ of weight $1/2$ each, and so currently, $d(u,v)\leq 1$. The insertion of the edge $(u,v)$, whose weight is at least $1$ will not decrease the distances.

For graph $G^H$, we use an algorithm that maintains all connected components of $H$ with update time $O(\log^2n)$ per edge deletion. This part takes $O(m\log^2n)$ total time. Once an edge $e=(u,v)$ of $G^H$ is deleted, we inspect its two endpoints, and, if any edge incident to $u$ or $v$ stops being heavy, we also delete that edge and add it to $G^L$. (If an edge $e'=(u,w)$ stops being heavy, this means that $w$ does not own $e'$, and $e'$ does not contribute to its set $I_i(w)$, where $i=\cutoff(w)$, so we don't need to inspect edges incident to $w$ and this deletion will not propagate). Next, we update all connected components of $G^H$ using the algorithm for maintaining the connected components. Figuring out which edges of $u$ and $v$ stop being heavy can be implemented by having buckets of level-$i$ edges incident to each vertex $x$, for each $i<\cutoff(x)$.

For graph $G^L$, we use the data structure from Lemma~\ref{lem: WSES}. In order to use it, we need to bound the number of edges of different levels that ever belong to $G^L$. Fix some level $1\leq i\leq \log n$, and consider a vertex $v\in V$. If, at the beginning of the algorithm, $\cutoff(v)<i$, then there are at most $2^i\tau$ vertices of level $i$ incident to $v$. Otherwise, if $\cutoff(v)\geq i$, then a level-$i$ edge incident to $v$ may only be added to $G^L$ when $\cutoff(v)$ decreases to be lower than $i$. At this moment, at most $2^i\tau$ edges of level $i$ are incident to $v$. Therefore, in total, over the course of the algorithm, the number of level-$i$ edges that ever belong to $G$ is bounded by $2^i\tau n$.

We also need to take care of vertex splitting. Recall that we construct an auxiliary graph $G'$, that contains the graph $G^L$, and additionally, for every super-node $v_C\in V_2$, we insert $|C|\log |C|$ extra-vertices, whose set we denote by $X(v_C)$. Therefore, $|V_2|\leq n\log n$. Over the course of the algorithm, every edge incident to a super-node $v_C$ may pay for up to $\log n$ edge insertions. So the total number of these extra edge insertions is bounded by $n\log n$. Therefore, the total number of edges of weight $1/2$ that are ever present in the graph is bounded by $O(n\log n)$. 

From Lemma~\ref{lem: WSES}, the total update time is $O(nD\log n)+O(\sum_e\frac{D}{\eps w(e)})$. For the second summand, for each $i\geq 1$, we will have at most $2^i\tau n\leq 2^in^2\log n/D$ edges of level $i$ ever present in the graph, so the corresponding summand for each $i$ becomes at most $O(\frac{n^2\log n}{\eps})$. Additionally, at most $O(n\log n)$ edges of weight $1/2$ will be present. So the total running time becomes $O(nD\log n)+O(\frac{n^2\log^2n}{\eps})=O(\frac{n^2\log^2n}{\eps})$.

Finally, we show that, throughout the algorithm, for every vertex $v\in V$ with $D\leq d(s,v)\leq 2D$, the algorithm maintains a $(1+\eps)$-approximation of $d(s,v)$. For that, it is enough to show that the distance from $s$ to $v$ in the graph $G^L$ is a $(1+\eps)$-approximation of $d(s,v)$. Let $P$ be the shortest path connecting $s$ to $v$ in $G^L$. We can assume that it is a simple path, so a super-node $v_C$ may appear on $P$ at most once. Let $D'$ denote the length of the path $P$. Notice that $D'\leq (1+\eps)d(s,v)$: let $P^*$ be the shortest $s$-$v$ path in $G$. We short-cut the path by contracting all clusters on it. This gives a path in $G^L$, whose length is at most $d(s,v)$. Since we maintain $(1+\eps)$-approximate shortest path in $G^L$, we are guaranteed that $D'\leq (1+\eps)d(s,v)$.

We now show that $d(s,v)\leq D'+\eps D$.  Let $v_{C_1},\ldots,v_{C_r}$ be all super-nodes that appear on the path $P$. For $1\leq j\leq r$, let $v_j$ be the regular vertex preceding $v_{C_j}$ on $P$, and let $u_j$ be the regular vertex following $v_{C_j}$ on $P$. Denote $n_j=|C_j|$. For each $1\leq j\leq r$, let $Q_j$ be the shortest $v_j-u_j$ path in graph $C_j$.

\begin{claim}\label{claim: length of path in heavy graph}
For all $1\leq i\leq \log n$ and $1\leq j\leq r$, the number of level-$i$ edges on $Q_j$ is at most $3n_j/(2^i\tau)$.
\end{claim}
\begin{proof}
Fix some $1\leq i\leq \log n$ and $1\leq j\leq r$, and let $e_1,\ldots,e_z$ be all level-$i$ edges on $Q_j$. Let $E'=\set{e_x\mid 1\leq x\leq z, x=1\mod 3}$. For each edge $e\in E'$, let $v(e)$ be an endpoint of $e$ that owns $e$ (that is, $\cutoff(v(e))\geq i$). Then $v(e)$ has at least $2^i\tau$ neighbors in graph $G^H$. Moreover, if $e,e'\in E'$ and $e\neq e'$, then the set of neighbors of $v(e)$ and the set of neighbors of $v(e')$ in graph $G^H$ are disjoint (otherwise we could have shortened the path $Q_j$). Therefore, $|E'|\leq \frac{n_j}{2^i\tau}$, and the total number of level-$i$ edges on $Q_j$ is at most $3n_j/(2^i\tau)$.
\end{proof}

Let $P^*$ be obtained from path $P$ by replacing the super-nodes $v_{C_j}$ with the corresponding paths $Q_j$.
We conclude that for each $1\leq i\leq \log n$, the total number of level-$i$ edges on $Q_1\cup\cdot\cup Q_r$ is at most $3n/(2^i\tau)$. Therefore, the total length of the paths $Q_1,\ldots,Q_r$ is at most $\frac{3n\log n}{\tau}\leq \frac{3n\eps D\log n}{3 n\log n}\leq \eps D$.

The total length of $P^*$ is then at most $D'+\eps D$, and so $d(s,v)\leq D'+\eps D$.

This concludes the exposition of Bernstein's algorithm. The main drawback of this algorithm is that it does not allow us to compute the shortest $s$-$t$ path (or an $s$-$v$ path). The reason is that we do not maintain shortest path trees in the connected components of the graph $G^H$. So we are only guaranteed that paths $Q_1,\ldots,Q_r$ of total length at most $\eps D$ exist, but we do not know how to find them. 




\newpage

\subsection{Extending Bernstein's Algorithm}
In this section we extend Bernstein's data structure, so that it can report the (approximate) shortest-paths from the source $s$, and not only their lengths. Our goal is to maintain a data structure, that, given a graph $G$ subject to edge deletions, and a source vertex $s$, can answer shortest-path queries: given a query vertex $v$, it must return a path from $s$ to $v$ of length at most $(1+\eps)d(s,v)$, in time $\tilde O(n)$. The total update time of the data structure is $O(n^2\poly\log n\log W/\eps)$, where $W$ is the largest edge weight.

As before, we use a parameter $D$, which is our estimate on the shortest-path distances: that is, our data structure will report approximate shortest paths correctly for all vertices $v$ with $D\leq d(s,v)\leq 2D$. 
Specifically, for a query vertex $v$, if $d(s,v)>2D$, then the data structure may not be able to return any $s$-$v$ path. Otherwise, if $d(s,v)\leq 2D$, the data structure is guaranteed to report some $s$-$v$ path. For every vertex $v$ for which the data structure reports an $s$-$v$ path, the path length is guaranteed to be at most $(1+\eps)d(s,v)+\eps D$. Therefore, for every vertex $v$ with $D\leq d(s,v)\leq 2D$, the algorithm is guaranteed to return a path of length at most $(1+2\eps)d(s,v)$. For a vertex $v$ with $d(s,v)<D$, the algorithm will return a valid $s$-$v$ path, that may be too long; and for a vertex $v$ with $d(s,v)>2D$ the algorithm may be unable to return any $s$-$v$ path. We keep a separate data structure for every value of $D$ that is an integral power of $2$ between $1$ and $nW$. Given a query vertex $v$, we run the query in each of these data structures, and return the shortest path that is returned by any of these data structures. From now on, we fix one value of $D$, $1\leq D\leq nW$, and describe a data structure for this value of $D$.

%We run separate algorithms for different scales of $D$ (for our specific application, we would need to use one value of $D$ at a time -- the current approximate length of the $s$-$t$ path). From now on, we assume that the value $D$ is fixed, and that we are only interested in vertices whose distances from $s$ are between $D$ and $4D$. 

We slightly modify the main parameter of Bernstein's algorithm, and set \fbox{$\tau=\frac{32n\log n}{\eps D}$}. The main definitions remain the same as before; we recap and extend them here.

\begin{itemize}
\item  For every edge $e$, we let $\class(e)=\floor{\log w(e)}$.

\item Given a vertex $v\in V(G)$, we denote by $I_i(v)$ the set of all edges of classes $1,2,\ldots,i$ that are incident to $v$, and by $I(v)$ the set of all edges incident to $v$.

\item For a vertex $v$, we let $\cutoff(v)$ be the largest integer $i$, such that $|I_i(v)|\geq \tau 2^i$. If no such index exists, we set  $\cutoff(v)=0$. Assume now that $\cutoff(v)=i>0$. We say that $v$ \emph{owns} all edges of $I_i(v)$, and all edges of $I_i(v)$ are called \emph{heavy} edges. Note that a heavy edge must be owned by at least one of its endpoints; but it may be owned by both endpoints.

\item For a vertex $v$, we define its \emph{effective degree} $\Delta(v)$ to be the number of edges that $v$ owns. In other words, if $\cutoff(v)=i$, then $\Delta(v)=|I_i(v)|$.

\item The two graphs $G^H$ and $G^L$ are defined exactly as before. We now only focus on the heavy graph $G^H$. Recall that its set of vertices is $V(G)$, and its set of edges consists of all heavy edges of $G$.
\end{itemize}


From Bernstein's algorithm, it is sufficient to design a data structure that can answer the following queries:

\begin{quote}
{\bf Query $(u,u')$:} \emph{Given two vertices $u,u'$ that belong to the same connected component $C$ of $G^H$,  return, in time $O(|C|\poly\log n)$, a path $Q\subseteq C$ connecting $u$ to $u'$, such that for each $1\leq i\leq \log n$, path $Q$ contains at most \fbox{$\frac{24|C|\log n}{2^i\tau}$} edges of class $i$.}
\end{quote}

(we note that such a path must exist from the analysis of Bernstein's algorithm).
Notice that the total length of the path $Q$ is at most $24|C|\log n/\tau$. 
We now show that being able to handle such queries is sufficient.

Recall that in the algorithm of Bernstein, we are given a query vertex $x\in V(G)$. Let $d'(s,x)$ be the distance from $s$ to $x$ in graph $G^L$, so $d'(s,x)\leq d(s,x)$. If $d'(s,x)>2D$, then we ignore this query and do not return a path (in this case, $x$ may not be included in the data structure). Assume now that $d'(s,x)\leq 2D$. Then the algorithm of Bernsten can be used to compute a simple path $P$, connecting $s$ to $x$ in $G^L$, whose length is at most $d'(s,x)(1+\eps)$ -- this is simply the path connecting $s$ to $x$ in the approximate \EST that he maintains. 
Let $v_{C_1},\ldots,v_{C_r}$ be the super-nodes lying on this path. For each such super-node $v_{C_j}$, let $u_j,u'_j$ be the regular vertices lying immediately before and immediately after $v_{C_j}$ on $P$, so $u_j,u'_j\in C_j$. Let $Q_j$ be the path connecting $u_j$ to $u'_j$ in $C_j$, that our algorithm returns, so the length of $Q_j$ is at most $24|C_j|\log n/\tau$. Let $P^*$ be the final path obtained from $P$, by replacing each super-node $v_{C_j}$ with the corresponding path $Q_j$. Then the length of $P^*$ is at most:

\[\begin{split} 
\ell(P)+\sum_j\frac{24|C_j|\log n}{\tau}&\leq (1+\eps)d'(s,x)+\frac{24n\log n}{\tau}
\\&\leq (1+\eps)d'(s,x)+\eps D\\
&\leq (1+\eps)d(s,x)+\eps D.\end{split}\]

Notice that, if $d(s,x)\leq 2D$, then $\ell(P^*)\leq (1+2\eps)d(s,x)$ as required. Let $\cset$ denote the set of all connected components of $G^H$. The total time that the algorithm spends to respond to the query $x$ in the data structure for this fixed value of $D$ is at most $O(n)+\sum_{C\in \cset}|C|\poly\log n=O(n\poly\log n)$, and the total query time is $O(n\poly\log n\log W)$.


We use two main tools. The first tool is the ES-trees. Given a connected graph $\hat G$, a designated source vertex $s(\hat G)$, and a length bound $ D(\hat G)$, we denote by $\EST(\hat G,s(\hat G), D(\hat G))$  the ES-tree data structure of $\hat G$ with respect to the source $s(\hat G)$, with the distance restriction $D(\hat G)$. We denote by $\ESIN(\hat G,e)$ and by $\ESDEL(\hat G,e')$ the procedures for inserting edge $e$ into the data structure $\EST(\hat G,s(\hat G), D(\hat G))$, and the procedure for deleting edge $e'$ from the data structure $\EST(\hat G,s(\hat G), D(\hat G))$, respectively. Both procedures include the necessary updates of the data structure.

In addition to ES-trees, we also need a data structure for connectivity. We will use the results of~\cite{dynamic-connectivity}, that provide a data structure, that we denote by $\CONN(\hat G)$, that, given an $n$-vertex graph $\hat G$ subject to edge deletions and edge insertions, responds to each connectivity query in $O(\log n/\log\log n)$ time, and has amortized running time of $O(\log^2n)$ per edge deletion or insertion. The data structure and the algorithm are deterministic.  In a connectivity query, we are given a pair $u,v$ of vertices of $\hat G$, and need to determine whether they are connected in $G$.
We denote by $\CONNIN(\hat G,e)$ and by $\CONNDEL(\hat G,e')$ the procedures for inserting an edge $e$ into and deleting an edge $e'$ from the data structure, respectively. We also denote by $\conn(\hat G,u,u')$ the connectivity query between $u$ and $u'$ in the data structure.


Before we define our data structure, we need a few additional definitions.
 For $1\leq j\leq \log n$, let $L_j$ contain the set of all vertices  $v$ of $G$ whose effective degree is: $2^j\leq \Delta(v)<2^{j+1}$.  We refer to vertices of $L_j$ as \emph{level-$j$ vertices}. For a vertex $v\in L_j$, we denote $\level(v)=j$.
 We let $1\leq\rho\leq\log n$ be the largest integer, for which $L_{\rho}\neq \emptyset$.
 We now define graphs $G_1,\ldots,G_{\rho}$ inductively, starting from graph $G_{\rho}$. For each graph $G_j$, we will also define an extended graph $G'_j$, that will allow us to handle super-node splitting. 
We then let $\cset_j$ be the set of all connected components of graph $G'_j$ that are not isolated vertices, and for each such component $C\in \cset_j$, we let $R(C)$ denote the set of all {\bf regular} vertices of $C$.

In order to define the graph $G_{\rho}$, we let the set of its vertices be $V(G)$. For every vertex $v\in L_{\log n}$, we add all edges that $v$ owns in $G_{\rho}$. The weight of each such edge is set to $1$, and they are called type-1 edges. The extended graph $G'_{\rho}=G_{\rho}$.

We now define graph $G_j$, for some integer $1\leq j<\rho$, assuming that graphs $G_{j+1}$ and $G'_{j+1}$ were defined. Recall that $\cset_{j+1}$ is the set of all connected components of graph $G'_{j+1}$ that are not isolated vertices, and for each such component $C\in \cset_{j+1}$, $R(C)$ is the set of all regular vertices lying in $C$. The set of vertices of $G_j$ consists of two subsets: set $V_1^j=V(G)$ of regular vertices, and set $V_2^j=\set{v_C\mid C\in \cset_{j+1}}$ of super-nodes. The set of edges consists of two subsets: set $E_1^j$ of type-$1$ edges contains, for every vertex $v\in L_j$, all edges owned by $v$. All edges of $E_1^j$ have weight $1$. Set $E_2$ of type-$2$ edges is defined as follows. For every component $C\in \cset_{j+1}$, for every regular vertex $u\in R(C)$, we add an edge $(u,v_C)$ of weight $1/2$ to $E_2$. (Note that $C$ may contain super-nodes $v_{C'}$, where $C'$ is a connected component of $G'_{j+2}$, and $v_{C'}$ does not belong to $G_j$; we only add edges connecting $v_C$ to regular vertices).

In order to define the extended graph $G'_j$, we start with $G'_j=G_j$. For every super-node $v_C\in V_2^j$, we add a set $X(v_C)$ of $\ceil{4|C|\log |C|}$ \emph{extra-vertices}, that all connect to $v_C$ with an edge of weight $1$ -- these edges are called type-3 edges. We say that super-node $v_C$ \emph{owns} all vertices of $X(v_C)$. Let $V_3^j$ denote the set of all extra-vertices of $G'_j$, and let $E_3^j$ be the set of all edges incident to them. Note that each extra-vertex has degree exactly $1$. 

As the algorithm progresses, the underlying graph $G$ changes, and the graphs $G_j$ and $G'_j$ evolve. When we refer to graph $G_j$ or $G'_j$, we refer to these graphs defined with respect to the current graph $G$. Similarly, for a vertex $x\in V(G)$, the values of $\cutoff(x)$, $\Delta(x)$, $\level(x)$ evolve as the algorithm progresses.
  Recall that $\cset_j$ is the set of all connected components of $G'_j$ that are not isolated vertices, and for each component $C\in \cset_j$, $R(C)$ is the set of all regular vertices of $C$. We then have the following simple observation and its corollary

\begin{observation}\label{obs: containment of CC's}
Let $1<j\leq \rho$ be an index, and let $C\in \cset_j$ be a non-singleton connected component of $G'_j$. Then there is some connected component $C'\in \cset_{j+1}$, such that $R(C)\subseteq C'$.
\end{observation}

\begin{corollary}\label{cor: containment of CC's}
For all $1\leq j'<j\leq \rho$, for every component $C\in \cset_j$, there is a component $C'\in \cset_{j'}$, such that $R(C)\subseteq C'$.
\end{corollary}


\subsubsection{Data Structures}
We now describe the data structures that we maintain.

\begin{itemize}
\item For each $1\leq j\leq \rho$, we maintain a list $\lset_j$ of all connected components of $G_j'$ that are not isolated vertices, so $\lset_j$ contains a list of all components of $\cset_j$. Every vertex of $G_j'$ that is not an isolated vertex, has a pointer to the connected component in $\lset_j$ to which it belongs. Additionally, for every component $C\in \lset_j$, there are bi-directional pointers between $C$ and the corresponding super-node $v_C$ in $G'_{j-1}$.

\item For every vertex $v\in V(G)$, we maintain a pointer from $v$ to its copies in each graph $G_j'$.

\item For each edge $e$, we maintain the information of which endpoints of $e$ own it, and pointers from its owners to $e$ and back. We also maintain pointers to the graphs $G'_j$ to which $e$ belongs (either one or two of them, depending on whether one or both endpoints of $e$ own it, and whether both endpoints belong to the same class), and to the corresponding copies of its endpoints.

\item For every regular vertex $v$, we maintain a list of all edges it owns, sorted into buckets, where bucket $B_i(v)$ contains all edges of class $i$ that $v$ owns. We also maintain the effective degree of $v$, $\Delta(v)$, and $\level(v)$.

\item For each $1\leq j\leq \log n$, we maintain the connectivity data structure $\CONN(G'_j)$.

\item For each $1\leq j\leq \log n$, for every connected component $C\in \cset'_j$, we select some vertex $s(C)$ to be a source, and we let $D(C)=12|C|/2^j$ be the distance bound for $C$. We later show that, as long as $C$ remains connected, the depth of the shortest-path tree from $s(C)$ is always at most $D(C)$. Finally, we maintain the data structure $\EST(C,s(C),D(C))$ for all $C\in \cset'_j$.
\end{itemize}





\begin{observation}\label{obs: size of cc's}
Throughout the algorithm, for all $1\leq j\leq \rho$, every connected component $C\in\cset_j$ contains at least $2^j$  regular vertices.
\end{observation}
\begin{proof}
The proof is by induction on $j$, starting from $j=\rho$. Graph $G'_{\rho}$ contains no super-nodes. If $C\in \cset_{\rho}$ is a connected component that is an isolated vertex, then it contains at least one edge. Since $G'_{\rho}$ has no super-nodes, every edge of $G'_{\rho}$ is a type-1 edge, that is, it is an edge of $G$ that is owned by some vertex $v\in L_{\rho}$. Let $e$ be any such edge that lies in $C$, and let $v\in L_{\rho}$ be the endpoint that owns it. Then $v\in L_{\rho}$, $\Delta(v)\geq 2^{\rho}$, and so $C$ contains at least $2^{\rho}$ vertices of $V(G)$.

We now assume that the claim is true for some $1<j\leq \rho$, and prove it for $j-1$. Let $C\in \cset_{j-1}$ be a connected component of $G'_{j-1}$, that is not an isolated vertex. Then some edge $e$ belongs to $C$. If one of the endpoints of $e$ is a super-node $v_{C'}$, for some $C'\in \cset_j$, then, from the induction hypothesis, $C'$ contains at least $2^{j}$ vertices of $V(G)$. Each such vertex connects to $v_{C'}$ with an edge in $G'_{j-1}$, and so $C$ contains at least $2^j$ regular vertices. Therefore, we assume that both endpoints of $e$ are regular vertices. Denote $e=(x,y)$. Since $e\in G_j'$ and its endpoints are regular vertices, $e\in E(G)$, and at least one of its endpoints (say $x$) owns it and belongs to $L_j$. Then the effective degree of $x$ is at least $2^j$, and all edges that $x$ owns belong to $C$. Therefore, $C$ contains at least $2^j$ regular vertices -- the endpoints of these edges.
\end{proof}

\begin{corollary}\label{cor: depth of tree bound}
Throughout the algorithm, for all $1\leq j\leq \log n$, for every connected component $C\in \cset_j$, for every vertex $x\in C$, the distance from $x$ to the source vertex $s(C)$ in $G'_j$ is at most $12|C|/2^j$.
\end{corollary}

\begin{proof}
Fix some $1\leq j\leq \log n$.
Recall that for every edge $e\in G'_j$, one of12dpoints of $e$ is either a super-node, or a vertex of $L_j$. In either case, the degree of this vertex in $G'_j$ is at least $2^j$. Consider now some connected component $C\in \cset_j$ and some vertex $x\in V(C)$. Let $P$ be the shortest path from $x$ to $s(C)$, and let $U\subseteq V(P)$ contain all super-nodes and all vertices of $L_j$ on this path. Then the length of the path $P$ is at most $2|U|$. Let $U'$ be obtained from $U$ by taking one vertex out of every $6$ consecutive vertices, so that $|U'|\geq |U|/6$. Then for every pair $v,v'\in U$ of vertices, $N_C(v)\cap N_C(v')=\emptyset$ (or we could shortcut the path $P$; notice that some edges have length $1/2$, and some edges have length $1$, which is why we take one vertex in $6$). Therefore, $|U'|\leq |C|/2^j$, and $\ell(P)\leq 12|C|/2^j$.
\end{proof}



Next, we describe how path queries are answered, and then how the data structure is updated.

\subsubsection{Path Queries}
Let $C$ be a connected component of $G^H$, and let $u,u'$ be any two vertices of $C$. 
We next describe an algorithm that answers the query $(u,u')$. Recall that the algorithm must return, in time $O(|C|\poly\log n)$, a path $Q\subseteq C$ connecting $u$ to $u'$, such that for each $1\leq i\leq \log n$, path $Q$ contains at most \fbox{$\frac{24|C|\log n}{2^i\tau}$} edges of class $i$.

Notice that $u,u'$ must lie in the same connected component of $G_1'$, that we denote by $C^*$. Let $s^*$ be the source vertex that we have selected for $C^*$. Consider the shortest-path tree $T(C^*)$ from $s^*$, that is maintained by the data structure $\EST(C^*,s(C^*),D(C^*))$. Let $x$ be the lowest common ancestor of $u$ and $u'$ in the tree, and let $P_1$ be the path obtained by concatenating the path from $u$ to $x$ and the path from $u'$ to $x$ in the tree $T(C^*)$. In order to compute $P_1$, we let $P$ be the path from $u$ to $s^*$, and $P'$ we let $P'$ be defined similarly for $u'$. We then traverse both paths in the reversed order, in order to identify the vertex $x$, and truncate them suitably.
 Note that $P_1$ does not contain any extra-vertices, since all extra-vertices have degree $1$, but it may contain super-nodes. We call $P_1$ a \emph{level-1 path}. Let $v_{C_1},\ldots,v_{C_r}$ be the super-nodes appearing on this path. For each $1\leq k\leq r$, let $u_k$ and $u'_k$ be the regular vertices appearing immediately before and immediately after $v_{C_k}$ on $P_1$. We then recursively find, for each $1\leq k\leq r$, a simple level-$2$ path $P^2_k$, connecting $u_k$ to $u'_k$ in $C_k$, by exploiting the paths connecting these two vertices to the source $s(C_k)$ in the tree $T(C_k)$ stored in the data structure $\EST(C_k,s(C_k),D(C_k))$ (as before, we truncate the two paths to the lowest common ancestor of $u_k$ and $u'_k$, so that $P^2_k$ is a simple path). We continue this process recursively, until we obtain a final path $P^*$, that only contains regular vertices. Notice that over the course of this process, for each $1\leq j\leq \rho$, we have computed a set $\pset_j$ of level-$j$ paths, that we denote by $\pset_j=\set{P_1^j,\ldots,P_{r_j}^j}$. Each such path $P_k^j$ lies in a distinct connected component $C^j_k$ of $\cset_j$ (because paths from previous levels were simple, and so each super-node could appear at most once, on at most one such path), and it was obtained by concatenating two paths of the ES-tree $T(C^j_k)$: a path from some vertex $u^j_k$ to the source $s^j_k$ of $C^j_k$, and a path from some vertex $\hat u^j_k$ to $s^j_k$ (after possibly deleting recurring vertices). In order to bound the approximation ratio, we prove the following claim.

\begin{claim}\label{claim: approx ratio full}
For each $1\leq i\leq \log n$, the number of class-$i$ edges that appear on the final path $P^*$ is at most $24|C^*|\log n/(2^i\tau)$.
\end{claim}

\begin{proof}
Let $E_i$ be the set of all level-$i$ edges that appear on $P^*$.
For each $1\leq j\leq \rho$, let $E_i^j\subseteq E_i$ be the set of all edges of $E_i$ that lie on the paths of $\pset_j$. 
It is enough show that for all $1\leq j\leq \log n$, $|E_i^j|\leq 24|C^*|/(2^i\tau)$.
We now fix some index $1\leq j\leq \log n$, and some path $P_k\in \pset_j$. Let $C_k\in \cset_j$ be the connected component to which $C_k$ belongs, and let $n_k=|R(C_k)|$. Recall that $P_k$ is a concatenation of two paths: a path  $Q$ from some vertex $u_k$ to the source $s_k$ of $C_k$, and a path $Q'$ from some vertex $\hat u_k$ to $s_k$, after we discard all vertices that appear on both paths, except for the lowest common ancestor of $u_k$ and $\hat u_k$ in $T(C_k)$. %Note that $Q$ may not contain extra-vertices, since each such vertex has degree $1$. 
Consider some edge $e\in E_i$ that lies on $Q$, and denote $e=(x,y)$. Since $e\in G'_j$, at least one of its endpoints (say $x$) owns $e$ and belongs to $L_j$. Therefore, if we denote $i'=\cutoff(x)$, then $i'\geq i$, and $|I_{i'}(x)|=\Delta(x)\geq 2^i\tau$, while, since $x\in L_j$, $2^j\leq \Delta(x)<2^{j+1}$. We conclude that $2^{j+1}>2^i\tau$. Consider the path $Q$, and let $U$ be the set of all vertices of $Q$ that belong to $L_j$. Let $U'\subseteq U$ be obtained by taking one out of every three consecutive vertices of $U$, so $|U'|\geq |U|/3$. Then each vertex of $U'$ has  effective degree at least $2^j\geq 2^i\tau/2$, and so it has at least $2^i\tau/2$ neighbors in $R(C_k)$. Moreover, for every pair $a\neq b$ of vertices in $U'$, $N_{C_k}(a)\cap N_{C_k}(b)=\emptyset$  (or we could decrease the length of $Q$ by connecting $a$ to $b$ through their common neighbor). Therefore, $|U'|\leq \frac{2|R(C_k)|}{2^i\tau}$, and $|U|\leq \frac{6|R(C_k)|}{2^i\tau}$. Therefore, the number of level-$i$ edges that lie on path $Q$ is bounded by $\frac{12|R(C_k)|}{2^i\tau}$ (as a vertex may be responsible for up to two such edges). We can use the same argument for path $Q'$. Overall, the number of level-$i$ edges that lie on $P_k$ is bounded by $\frac{24|R(C_k)|}{2^i\tau}$, and the total number of level-$i$ edges lying on paths of $\pset_j$ is at most $\frac{24}{2^i\tau}\sum_{C_k\in \cset_j}|R(C_k)|\leq \frac{24|C^*|}{2^i\tau}$.
\end{proof}


We now bound the running time of this algorithm.
For every level $1\leq j\leq \rho$, for every connected component $C\in \cset_j$, the algorithm spends up to $O(|C|)$ time to find the required path in the corresponding tree $T(C)$. We need to relate this bound to the number of regular vertices of $C$. Recall that each super-node $v_{C'}\in V(C)$ corresponds to a subset $C'\subseteq R(C)$ of regular vertices of $C$, and moreover, if $v_{C'}\neq v_{C''}$, then $C'\cap C''=\emptyset$. Therefore, there are at most $|R(C)|$ super-nodes in $C$. Each such super-node $v_{C'}\in C$ owns $O(|C'|\log |C'|)$ extra-vertices, so the total number of extra-vertices in $C$ is bounded by $\sum_{\stackrel{C'\in \cset_{j+1}:}{v_{C'}\in C}}O(|C'|\log |C'|)=O(|R(C)|\log |R(C)|)$. Overall, $|V(C)|=O(|R(C)|\log |R(C)|)$. The total time the algorithm spends on each layer $1\leq j\leq \rho$ is then at most $\sum_{C\in \cset_j}O(|R(C)|\log |R(C)|)=O(|C^*|\log |C^*|)$, and the total time for computing the answer to the query is $O(|C^*|\log^2n)$.



%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
\subsubsection{Maintaining the Data Structures}
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------

\paragraph{Initialization}

For every vertex $v$ in the original graph $G$, we compute $\cutoff(v)$, create the list of edges it owns partitioned into buckets by their level,  compute the effective degree of $v$ and $\level(v)$, in time $O(d_G(v))$. During this process we identify heavy edges. For each heavy edge $e$, we store pointers to its owner(s). All this takes $O(m)$ time.

Starting from $j=\log m$, we construct the graph $G_j$, the extended graph $G'_j$, and the set $\cset_j$ of connected components of $G'_j$. 
In order to do so, we construct the graph $G_j$, by adding one copy of every vertex in $V(G)$, and all edges owned by vertices on $L_j$. We then add, for every connected component $C\in \cset_{j+1}$, that is not a singleton vertex, a super-node $v_C$, that connects to every regular vertex of $C$, and a set $X(v_C)$ of $4|C|\log |C|$ extra-vertices, that connect to $v_C$ with edges. Since $\sum_{C\in \cset_{j+1}}|C|\leq n$, this can be done in time $O(m\log n)$ altogether. For every connected component $C$ of $G'_j$, we select an arbitrary vertex that is not an extra vertex to be its source $s(C)$ and set $D(C)=12|C|/2^j$. We then initialize $\EST(C,s(C),D(C))$. All this can also be done in total time $O(m\log n)$. %For every connected component $C\in \cset_j$, we set the bound $D(C)$ on the depth of the ES tree to be $12|C|/2^j$. From Corollary~\ref{cor: depth of tree bound}, the tree depth will always be bounded by this value.
We also initialize, for each $1\leq j\leq  \rho$, the data structure $\CONN(G'_j)$. This is done by starting from an empty data structure, and then adding the edges of $G'_j$ one-by-one.

%For accounting purposes, we also define potentials of the edges and the vertices of $G'_j$. Consider some connected component $C\in \cset_j$. For every edge $e=(u,v)$ of $C$, we let $\delta(e)$ denote $\min\set{d(s,u),d(s,v)}$. Throughout the algorithm, for every connected component $C\in \cset_j$, for every edge $e$ of $C$, the potential of $e$ is $4(D(C)-\delta(e))\tau$, where $\tau=O(\log n)$ is the time for a constant number of  heap operations. The potential of a vertex $v$ is $4(D(C)-d(s,v))\tau$.  We note that as the algorithm progresses and the clusters of $\cset_j$ are split into smaller clusters, we will define new bounds $D(C)$ on the cluster depth for the new clusters differently, to ensure that the potentials of the edges and the vertices do not increase.


\paragraph{Update Step.}

Suppose we need to delete an edge $e^*=(x,y)$. If $e^*$ is not a heavy edge, then the algorithm of Bernstein handles it. So we assume from now on that $e^*$ is a heavy edge. Assume first that $e^*$ is owned by exactly one of its endpoints - say $x$, and that $x\in L_j$. Then we need to delete the edge $e^*$ from the graph $G'_j$. As the result of this deletion, it is possible that the degree of $x$ will decrease below $2^j$, and so $x$ no longer belongs to $L_j$. Moreover, it is possible that $\cutoff(x)$ decreases, and so some of the edges that $x$ owned before the current iteration are no longer owned by $x$. In either case, we need to delete every type-$1$ edge $e'$ incident to $x$ from $G'_j$, unless $e'$ is owned by its other endpoint that belongs to $L_j$. We need to recompute the new effective degree and the new level $j'<j$ of $x$, and insert all edges that it still owns to the corresponding graph $G'_{j'}$. Moreover, as the result of all these edge-deletion operations, it is possible that some connected components of $G'_j$ split, and we will need
to split the corresponding super-nodes of $G'_{j-1}$ accordingly. This, in turn, can trigger more node-splitting in lower-level graphs. If the original edge $e^*$ is owned by both its endpoints, then it is possible that 
we need to delete it from two graphs, and repeat this whole process twice.


Therefore, over the course of the algorithm, we may need to delete edges from several graphs $G'_j$, where the deleted edge is either $e^*$, or it is an edge incident to a vertex whose effective degree decreases, or an edge may be deleted as a result of a vertex-splitting operation. Each one of these edge-deletion procedures may, in turn, trigger a vertex-splitting operation in the subsequent graph $G'_{j-1}$. Since vertex-splitting in $G'_{j-1}$ includes edge-deletion operations, this can in turn trigger vertex-splitting in $G'_{j-2}$, and so on. We now describe a procedure that deletes a given edge $e$ from a given graph $G'_j$.

\program{Delete-Edge($G'_j$,$e=(u,v)$)}{
\begin{enumerate}
\item Let $C$ be the connected component of $\cset_j$ that contains $e$ -- we can find it since $e$ points to it, and let $T(C)$ be the tree maintained by $\EST(C,s(C),D(C))$. If $e$ is not an edge of $T(C)$, delete $e$ from $G'_{j}$, and terminate the procedure. From now on, we assume that $e\in T(C)$.

\item Execute $\CONNDEL(G'_j,e)$. Check whether $u$ and $v$ are still connected in the new graph $G'_j$, by calling procedure $\conn(G'_j,u,v)$. 

\item If $u,v$ are still connected in the new graph $G'_j$:
execute $\ESDEL(C,e)$ and terminate the algorithm.

From now on we assume that $u,v$ are no longer connected in $G'_j$. We assume that $u$ is the parent of $v$ in the tree $T(C)$. Let $T_v$ be the sub-tree of $T$ rooted at $v$, and let $T'=T\setminus T_v$. Note that $C$ now decomposes into two connected components: one spanned by $V(T_v)$, and one spanned by $V(T')$. Next, we establish which of the two components contains fewer vertices.


\item Perform a BFS of $T_v$ from $v$ and a BFS of $T'$ from $s(C)$ in parallel, so both algorithms discover the same number of vertices at each step. Terminate the algorithm once all vertices in one of the two trees are explored. We assume w.l.o.g. that it is $T_v$; the other case is dealt with symmetrically.
\label{step: BFS}

\item 
We denote the connected component of $G'_{j+1}$ containing all vertices of $T_v$ by $C'$, and the connected component containing all vertices of $T'$ by $C''$. Set $s(C')=v$ and $D(C')=12|C'|/2^j$. Similarly, set $s(C'')=s(C)$ and $D(C'')=12|C''|/2^j$.
 Notice that $T_v$ is a shortest-path tree for $C'$ and $s(C')$, and $T'$ is a shortest-path tree of $C''$ and $s(C'')$. Initialize two new data structures: $\EST(C',s(C'),D(C'))$ using the tree $T_v$ and $\EST(C'',s(C''),D(C''))$ using tree $T'$, and the original data structure $\EST(C,s(C),D(C))$. Notice that the labels $\delta(x)$ for $x\in T_v$ have changed, and need to be set to $d(x,v)$ instead of $d(x,s)$. However, we know that $d(x,v)=d(x,s)-\delta(v)$, where $\delta(v)$ is the label of $v$ before the current update. Instead of updating the labels $\delta(x)$, we simply remember the value $\offset(C')=\delta(v)$ and treat each label $\delta(x)$ as $d(v,x)+\offset(C')$. We follow this pattern as the labels $\delta(x)$ get updated over the course of the algorithm. (We may not be able to afford to update all labels $\delta(x)$ for $x\in V(T_v)$, if $T_v$ contains more than half the vertices of $C$). \label{step: split ES-trees}

\item If $C'$ consists of a single vertex $v$:  \label{step: if one vertex}


\begin{enumerate}
\item update $v$ so that it no longer points to any connected component of $\lset_j$ and execute $\DE(G'_{j-1},e'=(v,v_C))$.
\item if $C''$ consists of a single vertex $u$: delete $C$ from the list $\lset_j$ of connected components of $G'_j$; update $u$ so that it no longer points to any component of $\lset_j$; execute $\DE(G'_{j-1},e'=(u,v_C))$.
\end{enumerate}

\item Otherwise: $C'$ and $C''$ contain more than one vertex each. \label{step: of more than one vertex}

\begin{enumerate}
 \item Add $C'$ to the list $\lset_j$ of connected components of $G'_j$ and add pointers from every vertex of $C'$ to $C'$; rename $C$ by $C''$ in $\lset_j$.
 
 \item Execute $\VS(G'_{j-1},v_C,C')$. \label{step: execute split cluster}
\end{enumerate}.
\end{enumerate}
}


\program{Vertex-Split($G'_j$,$v_C$, $C'$)}{
The procedure receives as input index $j$ of graph $G'_j$, and a super-node $v_C$ in this graph, such that cluster $C\in G'_{j+1}$ was split into $C'$ and $C''$, with $1<|C'|\leq |C''|$. The procedure is also given the list of vertices of $C'$, and a pointer to $C'$ and $C''=C\setminus C'$ in the list $\lset_j$ of components of $G'_{j+1}$. Let $\hat C\in \cset_j$ be the connected component of $G'_j$ containing $v_C$.

\begin{enumerate}
%\item If $C'$ contains a single vertex, that we denote by $u$, then execute $\DE(G'_j,(v_C,u))$ and terminate the algorithm. We now assume that $|C'|>1$.

\item Select disjoint subsets $X(v_{C'})$ of $\ceil{4|C'|\log |C'|}$ vertices of $C$ and $X(v_{C''})$ of $\ceil{4|C''|\log |C''|}$ vertices of $C$, and an additional vertex of $X(C)$ denoted by $v_{C'}$. Add a pointer from $v_{C'}$ to the component $C'$ on list $\lset_{j+1}$.

\item For each $x\in C'$, execute $\ESIN(\hat C, (v_{C'},x))$, and $\CONNIN(G'_j,(v_{c'},x))$.

\item For each $y\in X(v_{C'})$, execute $\ESIN(\hat C,(v_{C'},y))$, $\CONNIN(G'_j,(v_C',y))$, $\ESDEL(\hat C,(v_{C'},y))$, and $\CONNDEL(G_{j}',(v_{C'},y)$  (Notice that vertex $x$ has  degree $1$ in the original and in the new graph $G'_j$, so there is no need to run the full Procedure $\DE(G'_j,(v_C,y))$.)

\item For each $x\in C'$, and for each $x\in X(C)\setminus X(C'')$, execute $\DE(G'_j,(v_C,x))$ (notice that this includes $x=v_{C'}$).

%\item Execute $\DE(G'_j(v_C,v_{C'}))$.

\item Rename $v_C$ as $v_{C''}$ and add a pointer from it to $C''$ in the list $\lset_{j+1}$ of connected components of $G'_{j+1}$.
\end{enumerate}
}


We need to argue that operations $\ESIN$ that we perform do not decrease distances of vertices from $s(\hat C)$.
Notice that we only insert edges that connect $x_{C'}$ to the regular vertices of $C'$ and to the vertices of $X(C')$. At the moment of the insertion of these edges, all these vertices are connected to $v_C$ with an edge of length $1$, and the neighbors of $v_{C'}$ are a subset of the neighbors of $x_C$. \mynote{Need to fix this. Distance from $s(\hat C)$ to $v_{C'}$ may shorten.}

 Let $e^*=(x,y)$ be the edge that we need to delete from $G^H$. Let $z\in \set{x,y}$ be an endpoint of $e^*$ that owns it, and assume that $\level(z)=j$. We execute $\DE(G'_j,e^*)$. We then inspect both endpoints of $e^*$. We say that endpoint $z'$ of $e^*$ is bad if all of the following hold:
 
 \begin{itemize}
 \item $z'$ owned $e^*$ at the beginning of the update;
 \item $z'\in L_j$ at the beginning of the update; and
 \item $\Delta(z')<2^j$ after $e^*$ is deleted.
 \end{itemize}
 
For each bad endpoint $z'$ of $e^*$ we do the following:

\begin{itemize}
\item Recompute $\cutoff(z')$. If $\cutoff(z')$ decreased, then for every edge $e$ that $z'$ originally owned, but does not own anymore, update this information in edge $e$ and in $z'$.

\item Recompute the new effective degree of $z'$. If there is some index $1\leq j'\leq \rho$, such that $2^{j'}\leq \Delta(z')<2^{j'+1}$, add $z'$ to $L_{j'}$; for every edge $e$ that $z'$ still owns: execute $\ESIN(G'_{j'},e)$ and $\CONNIN(G'_{j'},e)$.

\item Inspect every edge $e\neq e^*$ that $z'$ owned before the update. 
Let $y_e$ be the other endpoint of this edge. If $y_e\not \in L_j$, or if $y_e$ does not own $e$, execute $\DE(G'_j,e)$.
\end{itemize}

Notice that, if $e^*$ is owned by both its endpoints, and these endpoints have different levels, we may need to execute the above procedure twice.

We need to verify that, when an edge is inserted into an $\EST$ data structure, the distances from the source do not increase. We only insert an edge $e=(a,b)$ into $G'_{j'}$ if both endpoints $a,b$ of $e$ belong to the same connected component of $G'_j$ for some $j>j'$. From Corollary~\ref{cor: containment of CC's}, $a$ and $b$ belong to the same connected component of $G'_{j'+1}$, that we denote by $\hat C$. Therefore, graph $G'_{j'+1}$ contains a vertex $v_{\hat C}$, to which both $a$ and $b$ are connected with edges of weight $1/2$. The insertion of the edge $(a,b)$ of length $1$ does not decrease any distances in $G'_{j'+1}$.



\paragraph{Time Analysis}
Fix some $1\leq j\leq \rho$. We first bound the total number of vertices of $G'_j$, and the total number of edges that ever belong to $G'_j$. To bound $|V(G'_j)|$, recall that it contains $n$ regular vertices, up to $n$ super-nodes, and up to $O(n\log n)$ extra-vertices, so $|V(G'_j)|=O(n\log n)$.

We now bound the total number of edges that either belong to $G'_j$ from the beginning, or are added to it over the course of the algorithm. Notice that every regular vertex $v$ may belong to $L_j$ at the start of the algorithm (time $0$), or it may start belonging to $L_j$ over the course of the algorithm. Whenever vertex $v$ is first added to $L_j$, either at the beginning of the algorithm, or later, it owns at most $2^{j+1}$ edges, that are added to $G'_j$ as type-$1$ edges. Therefore, the total number of type-$1$ edges that ever belong to $G'_j$ is bounded by $2^{j+1}\cdot n$.

We now bound the number of type-$2$ and type-$3$ edges. At the beginning of the algorithm, we are given some set $\cset_{j+1}$ of connected components of $G_{j+1}$, that are not isolated vertices. Denote these components by $C_1,\ldots,C_r$. Each component $C_i$ has $|C_i|$ type-$2$ edges incident to $v_{C_i}$, and $O(|C_i|\log |C_i|)$ type-$3$ edges incident to it. We charge the vertices of $C_i$ for these edges, so each vertex of $C_i$ is charged for one type-$2$ edge -- the edge that is incident to it, and $O(\log n)$ type-$3$ edges.

Consider now an iteration when $C_i$ is split into $C'_i$ and $C''_i$, with $|C'_i|\leq |C''_i|$. We then insert $|C'_i|$ new type-2 edges, and $O(|C'_i|\log |C'_i|)$ new type-$3$ edges. As before, we charge every vertex of $C'_i$ for one new type-$2$ edge, and for $O(\log n)$ new type-$3$ edge. Notice however that $|C'_i|\leq |C_i|/2$, so every vertex of $G$ can be charged at most $\log n$ times. Overall, the total number of type-$2$ edges that are ever added to $G'_j$ is bounded by $O(n\log n)$, and the bound for type-$3$ edges is $O(\log^3n)$.

Since the amortized update time for $\CONN(G_j')$ is $O(\log^2n)$, the total amount of time spent on $\CONNIN$ and $\CONNDEL$ operations is bounded by $O(n\poly\log n)$. Moreover, we only call query $\conn(G'_j,u,u')$ when the edge $(u,u')$ is deleted from $G'_j$. So the number of such queries over the course of the algorithm is $O(n\poly\log n)$, and the total time spent handling them is $O(n\poly\log n)$. From now on we can ignore all calls to the data structures $\CONN(G_j')$ over the course of our algorithm.



In order to analyze the remainder of the algorithm, we define potentials. Throughout the algorithm, for every vertex $v\in G_j'$, if $v$ is an isolated vertex then its potential $\phi(v)=0$. Otherwise, if $v$ belongs to a connected component $C\in \cset_j$, then $\phi(v)=(D(C)-d(v,s(C)))d(v)\eta$, where $d(v)$ is the degree of $v$ in $G_j'$, and $\eta=O(\log n)$ is time needed to perform a constant number of standard heap operations.
We then let $\phi(G_j')=\sum_{v\in V(G_j')}\phi(v)$.

At the beginning of the algorithm, for every connected component $C\in \cset_j$, $D(C)\leq n/2^j$. The total potential is then bounded by:

\[\phi(G_j')=\sum_{v\in V(G_j')}\phi(v)\leq \sum_{v\in V(G_j')}\frac{n}{2^j}\eta |E(G_j')|\leq \frac{n}{2^j}\eta n\cdot 2^j\leq O(n^2\poly\log n).\]


Whenever an edge is inserted into $G'_j$, the potential may increase by up to $2\cdot\frac{n}{2^j}\cdot \eta$, and the total number of edges every inserted into $G'_j$ is bounded by $O(n\log n\cdot 2^j)$, so the total increase in the potential is bounded by $O(n^2\poly\log n)$.

Consider now an execution of procedure $\DE(G'_j,e=(u,v))$, and assume that $u$ and $v$ lie in the connected component $C\in \cset_j$ before the current iteration. If the deletion of $e$ does not cause the split of $C$, then, ignoring the calls to $\CONN$ data structure, we execute one call to $\ESDEL$ data structure. As discussed before, the time spend on executing such a call is bounded by the decrease in the total potential.

Assume now that after $e=(u,v)$ is removed, component $C$ is split into $C'$ and $C''$, with $|C'|\leq |C''|$. Step~\ref{step: BFS} of Procedure $\DE$ takes $O(|C'|)$ time; we charge it to the $\VS$ procedure that is executed in Step~\ref{step: execute split cluster}. The remaining steps of the procedure take $O(1)$ time. However, once we split $C$ into $C'$ and $C''$, we set the new bounds $D(C')$ and $D(C'')$ on the cluster depths, and the potentials of the edges change. We assume w.l.o.g. that $C'$ is the cluster corresponding to the tree $T_v$. Notice that now, for every vertex $x\in T_v$, we need to take into account the distance of $x$ from the new source $v$, instead of $s$, in the potential $\phi(x)$. First, for every vertex $x\in C''$, $d(x,s(C''))=d(x,s(C))$ does not change, while $D(C'')<D(C)$ holds, so $\phi(x)$ may only decrease. We now consider some vertex $x\in V(C')$, and show that its potential also can only decrease. The original potential is:

\[\phi'(x)=(D(C)-d(x,s(C)))d(x)\eta=\left (\frac{12|C|}{2^j}-d(x,s(C))\right )d(x)\eta.\]

The new potential is:

\[\phi(x)=(D(C')-d(x,v))d(x)\eta=\left (\frac{12|C'|}{2^j}-d(x,v)\right )d(x)\eta.\]

Notice that $d(x,v)=d(x,s(C))-d(v,s(C))$, where all these distances are taken before the deletion of the edge $(u,v)$; this is since $v$ is on the shortest path from $x$ to $s(C)$. Therefore, in order to prove that the potential of $x$ does not increase, it is enough to show that:

\[\frac{12|C'|}{2^j}-d(x,s(C))+d(s(C),v)\leq \frac{12|C|}{2^j}-d(x,s(C)),\]

or, equivalently that:

\[d(s(C),v)\leq \frac{12(|C|-|C'|}{2^j}).\]

This is done in a way similar to the proof of Corollary~\ref{cor: depth of tree bound}. We let $U$ be the set of all vertices on the path $P$ from $s(C)$ to $v$ (before the deletion of the edge), that either lie in $L_j$ or are super-node. At least half of the vertices of $P$ belong to $U$, and each such vertex must have at least $2^j$ neighbors, each of which lies in $|C|-|C'|$. We then let $U'$ contain one vertex out of every $6$ consecutive vertices of $P$, and observe that for all $a,b\in U'$, $N(a)\cap N(b)=\emptyset$. Therefore, $|U'|\leq (|C|-|C'|)/2^j$... \mynote{need to switch 12 to 24}.

Finally, we analyze Procedure \VS. The running time of this procedure, excluding the calls to $\ESDEL$, $\ESIN$, $\CONNIN$ and $\CONNDEL$ is $O(|C'|)$


==> decremental-sssp.tex <==
\newpage
\section{Decremental Single-Source Shortest Paths with Path Queries}

Pointer to Bernstein's paper: "Deterministic Partially Dynamic Single Source Shortest Paths in Weighted Graphs", \url{https://arxiv.org/abs/1705.10097}


The goal of this section is to prove the following theorem that extends the results of Bernstein~\cite{Bernstein}.

\begin{theorem}\label{thm: decremental shortest path main}
There is a deterministic algorithm, that, given an undirected $n$-vertex graph $G=(V,E)$ with integral weights $w(e)\geq 1$ on edges $e\in E$, that is subject to edge deletions, and an error parameter $0<\eps<1$, maintains, for every vertex $v\in V$, a value $\delta(v)$, such that $\dist(s,v)\leq \delta(v)\leq (1+\eps)\dist(s,v)$, in total update time $O(n^2(\poly\log n)(\log W)/\eps^2)$, where $W=\max_{e\in E}\set{w(e)}$. Moreover, the algorithm can answer approximate shortest-path queries that are interspersed with updates, in time $O(n\poly\log n)$ per query. In every query, the algorithm is given a vertex $v$, and needs to return a path from $s$ to $v$ in $G$, of length at most $(1+\eps)\dist(s,v)$.
\end{theorem}

%Throughout this section, the graphs we consider are undirected, and all algorithms are deterministic.
%In the decremental single-source shortest paths problem, we are given a graph $G=(V,E)$, a source vertex $s$, and weights $w_e> 0$ on the edges of $G$. In every iteration, some edge is deleted from $G$. We would like to maintain the (approximate) distances of all vertices from the source. We assume that all edge weights are integers between $1$ and $W$. Bernstein showed a deterministic algorithm, that maintains $(1+\eps)$-approximate distances from $s$ to every vertex in total update time $O(m\log^2n\log(nW)+n^2\log n\log(nW)/\eps^2)=\tilde{O}(n^2/\eps^2)$. 
%The drawback of his algorithm is that the data structure he maintains does not allow us to recover the path itself. In this section, we will try to rectify this drawback.
We note that Bernstein~\cite{Bernstein} showed a similar result, except that his algorithm cannot handle shortest-path queries. Our algorithm follows the high-level framework of Bernstein, but modifies his algorithm and the data structure in a way that allows us to compute the approximate shortest paths. 

 \mynote{this should go to one of previous sections}
A quick note on how we decide which edges to delete in the algorithm for vertex sparsest cut. 
Recall that our algorithm executes a number of phases, where in each phase, we choose an approximate shortest $s$-$t$ path $P$. We do not necessarily delete the edges of $P$ from the graph.
Recall that for each edge $e=(u,v)$ in the original graph $G$, we have added $\log^2n$ copies of $e$ to the new graph $G'$. For $1\leq i,j\leq \log^2n$, copy $e_{i,j}$ has weight $2^i+2^j$, and it is present in $G'$, as long as $v$ participates in fewer than $i/\alpha$ paths and $u$ participates in fewer than $j/\alpha$ paths. 
Throughout the algorithm, we maintain, for every vertex $v$ of $G$, a counter $p(v)$ that counts the number of paths in which $v$ participated so far. For each $1\leq i\leq \log n$, let $B_i(v)$ be the set of all edges of the new graph $G'$, that contains, for each edge $e=(u,v)$ of $G$ incident to $v$, the copies $\set{e_{i,j}\mid 1\leq j\leq \log n}$ of $e$. We add bi-directional links between the copies of $e_{i,j}$ in $B_i(v)$ and $B_j(u)$.

Once a path $P$ is chosen for the current phase, we perform procedure that we call \procetd, whose goal is to produce the set $E'$ of edges that need to be deleted from $G'$ in the current phase. Procedure \procetd updates the counters $p(v)$ for every vertex $v\in V(P)$. For every vertex $v\in P$, if $p(v)$ reaches an integral multiple of $1/\alpha$, say $i/\alpha$, all edges that currently belong to $B_i(v)$ are added to $E'$, to be deleted from $G'$. For each such edge $e_{i,j}$, where $e=(v,u)$, we  also delete $e_{i,j}$ from $B_j(u)$.
The running time of \procetd is proportional to the number of edges that are eventually added to the set $E'$, and deleted from $G'$. Therefore, over the course of the algorithm, we will spend at most $O(|E(G')|)=O(|E(G)|\cdot \log^2n)$ time on Procedure \procetd.

\mynote{end of part that needs to move to another section}



The main data structure that we use is an extension of ES-trees, that we call  \EESF. 
Suppose we are given a graph $G$ with integral weights $w(e)\geq 1$ on its edges $e\in E$, a source $s$, and a distance bound $D\geq 1$. \EST algorithm maintains, for every vertex $v$ with $\dist(s,v)\leq D$, the distance $\dist(s,v)$, under the deletion of edges from $G$. We denote the corresponding data structure, that we describe later, by $\EST(G,s,D)$. When the distance bound $D$ is unbounded (that is, $D=nW$, where $W=\max_{e\in E}\set{w(e)}$), then we denote the data structure by $\EST(G,s)$.
The total running time of the algorithm, including the initialization and all edge deletions, is $O(m\cdot D\log n)$, where $m=|E|$.

\ESTs also support edge insertions, in some limited cases. An edge $e=(u,v)$ can be inserted into the current graph $G$ if at least one of the following two conditions hold: (i) if the insertion of the edge $e$ does not decrease the distance of any vertex from $s$, or (ii) if one of the endpoints of $e$ is an isolated vertex. \ESTs also support insertion of isolated vertices into the graph $G$.

Assume now that we are given a graph $G=(V,E)$, and, additionally,  a partition $\sset=\set{S_1,\ldots,S_r}$ of the vertices of $G$ into  disjoint subsets, that we refer to as \emph{clusters}. We define an extended graph $\hat G=\hat G_{\sset}$ associated with $G$ and $\sset$, as follows. The set of vertices of $\hat G$ consists of two subsets: set $V_1=V(G)$ of \emph{regular vertices}, and set $V_2=\set{v_S\mid S\in \sset}$ of \emph{super-nodes}.  The set of edges also consists of two subsets: set $E_1$ of edges contains all edges of $G$, with the same weights as in $G$ (that we have assumed to be integers between $1$ and $W$), and another set $E_2$ of edges, that is defined as follows. For every super-node $v_S$, for every regular vertex $u\in S$, we add an edge $(u,v_S)$ of weight $1/2$ to $E_2$. Therefore, every edge of $E_2$ connects a super-node to a regular vertex, and the sum of degrees of all super-nodes is $|E_2|= n$. 
Assume now that we are given some source vertex $s\in V(\hat G)$, and a distance bound $D\geq 1$. The Extended ES-Tree data structure needs to maintain, for every vertex $v\in V(\hat G)$, the distance $\dist_{\hat G}(s,v)$ under three operations: deletion of regular edges; insertion of eligible regular edges; and cluster splitting. We now describe each of these operations in turn. Our final data structure, \EESF, is a generalization of \EEST.

\paragraph{Edge Deletion.} In an edge deletion operation, we are given some regular edge $e\in E(G)$, that is deleted from $G$. We need to delete the edge from $\hat G$ and update the data structure accordingly. This operation is denoted $\EESTDEL(\hat G,e)$.

\paragraph{Edge Insertion.} Let $(u,v)$ be a pair of vertices of $G$. We say that $(u,v)$ is an edge that is eligible for insertion, if the insertion of $(u,v)$ into $G$ does not decrease $\dist_{G}(s,x)$ for any $x\in V(G)$. %; or (ii) at least one of the vertices $u,v$ is an isolated vertex that was just inserted into $G$. 
In an edge-insertion operation, that is denoted by $\EESTIN(\hat G,e)$, we are given a pair $u,v\in V(G)$ of vertices, such that $(u,v)$ is an edge eligible for insertion, and we need to insert edge $(u,v)$ into $G$ and $\hat G$, and update the data structure accordingly.

%\paragraph{Vertex Insertion.} In a vertex insertion operation, we are given a new vertex $v$ that is inserted into $G$ as an isolated vertex. We denote this operation by $\EESTVIN(\hat G,v)$.

\paragraph{Cluster Splitting.} In a cluster-splitting operation, we are given a set $S\in \sset$, and a partition of $S$ into two subsets $S',S''$, with $|S'|\leq |S''|$. We assume that the set $S'$ is given explicitly by a list of all its vertices; we are not given the list of vertices of $S''$, but we know that $S''=S\setminus S'$. We need to replace $S$ with $S'$ and $S''$ in $\sset$ and to update $\hat G$ and the data structure accordingly. This operation is denoted by $\EESTSPLIT(\hat G,S,S')$. We note that it is possible that the source vertex $s=v_S$ corresponds to the cluster we split; we then set the new source $s=v_{S''}$ after the splitting operation.

The following theorem follows from~\cite{BernsteinChechik,Bernstein}. 

\begin{theorem}\label{thm: EEST}
There is an algorithm, that, given a graph $G$ with unit edge lengths, a partition $\sset$ of its vertices into clusters, a distance bound $D$, and a source vertex $s$ in the corresponding  extended graph $\hat G_{\sset}$, maintains, for every vertex $v\in V(\hat G_{\sset})$ with $\dist_{\hat G_{\sset}}(s,v)\leq D$, the distance $\dist_{\hat G_{\sset}}(s,v)$, under operations $\EESTIN,\EESTDEL$, and $\EESTSPLIT$. The total running time of the algorithm is $O((m+n\log n)D\log(m+n\log n))$, where $n=|V(G)|$ and $m$ is the total number of {\bf regular} edges that were ever present in $\hat G$, including the edges that were inserted. Moreover, the algorithm can answer shortest-path queries that are interspersed with updates, in time $O(n)$ per query. In every query, the algorithm is given a vertex $v\in V(\hat G_{\sset})$, and needs to return a shortest path from $s$ to $v$ in $\hat G_{\sset}$, if $\dist_{\hat G_{\sset}}(s,v)\leq D$.
\end{theorem}

We note that if an edge is inserted into and deleted from the graph multiple times, we view each new copy of the edge as a new edge and count it separately.
We rely on the above theorem for our generalization to Extended ES-Forests. Since we do not use it as a black-box, we provide its proof in the Appendix.

We now turn to describe \EESFs. This data structure is very similar to \EEST, except that now, for every connected component $C$ of the extended graph $\hat G_{\sset}$, we will choose an arbitrary vertex $s(C)$ as its source, and we will maintain an \EST in $C$ with the source $s(C)$, for each connected component $C$ of $\hat G$.

The operations that \EESF supports are: 
\begin{itemize}
\item Deletion of a regular edge $e$, denoted by $\EESFDEL(\hat G,e)$; notice that, as a result of this operation, some connected components of $\hat G$ may split into two, and we will need to choose a source vertex for each of them, and to maintain an \EST in each of them.

%\item Insertion of a new isolated vertex $v$, denoted by $\EESFVIN(\hat G,v)$;

\item Insertion of an eligible edge $e=(u,v)$, denoted by $\EESFIN(\hat G,e)$. Edge $e=(u,v)$ is eligible if %either (i) at least one of $u,v$ is an isolated vertex; or (ii) 
both $u,v$ belong to the same connected component $C$ of $\hat G$, and the insertion of $e$ does not decrease $\dist(s(C),x)$ for any $x\in C$; and

\item Splitting of a cluster $S\in \sset$ into two new clusters $S',S''$, with $|S'|\leq |S''|$, denoted by $\EESFSPLIT(\hat G,S,S')$. As before, the vertices of $S'$ are listed explicitly as input to this operation, but not the vertices of $S''$. We need to update the extended graph $\hat G$ and the data structure. Notice that, as the result of this operation, some connected components of $\hat G$ may split, and we will need to choose a source vertex for each of them, and to maintain an \EST for each of them. 
\end{itemize}



Unlike \EEST, where we are given a distance bound $D$, and we only need to maintain distances from $s$ to vertices that are at distance at most $D$ from $s$, in \EESF we will use different distance bounds $D(C)$ for connected components $C$ of $\hat G$. We will assume that we are given some value $\gamma$, and we will set $D(C)=|C|/\gamma$. This will be sufficient for us, since we will only use \EESF for graphs that are $\gamma$-bounded, as defined below.

\begin{definition}
Let $G$ be a graph, $\sset$ a partition of its vertices, and $\hat G=\hat G_{\sset}$ the corresponding extended graph. We say that $\hat G$ is $\gamma$-restricted, for some parameter $\gamma\geq 1$, iff for every connected component $C$ of $\hat G$, for every pair $u,v\in V(C)$ of its vertices, $\dist_{\hat G}(u,v)\leq |C|/\gamma$.
\end{definition}



The next theorem generalizes Theorem~\ref{thm: EEST} to \EESF.

\begin{theorem}\label{thm: EESF}
There is an algorithm, that, given a graph $G$ with unit edge lengths, a partition $\sset$ of its vertices into clusters, and a parameter $\gamma>1$, does the following. For every connected component $C$ of the corresponding  extended graph $\hat G_{\sset}$, it chooses an arbitrary source vertex $s(C)\in C$, and maintains, for every vertex $v\in C$ with $\dist_{\hat G_{\sset}}(s(C),v)\leq |C|/\gamma$, the distance $\dist_{\hat G_{\sset}}(s(C),v)$. The algorithm supports operations $\EESFIN,\EESFDEL$, and $\EESFSPLIT$. Moreover, if the original graph $\hat G$ is $\gamma$-restricted, and if it stays so after each of the above operations, then the total running time of the algorithm is $O\left(\frac{nm\log(n+m)}{\gamma}\right)+O((m+n)\log^2m)$, where $n$ and $m$ are the total number of vertices and edges, respectively, that were ever present in $\hat G$. The algorithm can also answer shortest-path queries that are interspersed with updates, in time $O(n\poly\log n)$ per query. In every query, the algorithm is given a vertex $v\in V(\hat G_{\sset})$, and needs to return a shortest path from $s(C)$ to $v$, where $C$ is the connected component of $\hat G$ in which $v$ lies, if $\dist_{\hat G_{\sset}}(s(C),v)\leq |C|/\gamma$.
\end{theorem}




One unfortunate property of the \ESTs is that the total running time of the algorithm is $O(mD)$.  Bernstein's algorithm uses the \ESTs only in a sub-graph of the original graph $G$, where large-degree vertices are deleted. If the original graph $G$ were unweighted, we could use a threshold $\tau=n/D$, and ignore all vertices whose degree is greater than $\tau$ -- such vertices are taken care of by an auxiliary structure. The total running time of the \EST algorithm then becomes $O(mD)=O(n\tau D)=O(n^2)$. However, when edges have large weights, in order to ensure that the algorithm always returns a good approximation to the distances from the source $s$, we need to set the threshold $\tau$ differently for different weight classes. Because of this, for each $i$, we may have up to $n^2\cdot 2^i/D$ edges of weight roughly $2^i$ in the resulting graph. Bernstein modifies \ESTs, so that edges of greater weight contribute less to the running time of the algorithm, at the cost of maintaining the shortest paths approximately. The total running time is the sum of $O(nD)$ and $\sum_{e\in E}\frac{D}{\eps w(e)}$. This is a perfect tradeoff, because there are at most $n^22^i/D$ edges of weight roughly $2^i$ in the graph he maintains, so the total running time becomes $O(nD)+\tilde O(n^2(\log W)/\eps)$. His algorithm allows edge deletions and insertion of edges that do not increase distances from $s$. It also allows increase in edge weights, but we do not need this part. The algorithm is called WSES (weight-sensitive Even-Shiloach).

Below is a restatement of Lemma 4.3 from [Bernstein]; for completeness we provide its proof in Appendix.

\begin{theorem}\label{thm: WSES}
There is an algorithm, that, given a graph $G$ with integer edge weights $w(e)\geq 1$ a partition $\sset$ of $V(G)$ into clusters, a source vertex $s$ in the corresponding extended graph $\hat G$, and a length bound $D\geq 1$, maintains, for every vertex $v\in V(\hat G)$ with $d(s,v)\leq 2D$, an  approximate distance $d'(s,v)$, such that, if $D\leq d(s,v)\leq 2D$, then:

\[d(s,v)\leq d'(s,v)\leq (1+\eps)d(s,v).\]

The algorithm supports operations $\EESTDEL$, $\EESTIN$ and $\EESTSPLIT$.
The total update time of the algorithm is $O(nD)+O\left (\sum_{e\in E_0\cup E_1}\frac{D}{\eps w(e)}\right )$, where $E_0$ is the original set of edges of $G$, $E_1$ is the set of edges that were ever inserted, and $n$ is the total number of vertices that were ever present in the graph. Moreover, the algorithm can answer shortest-path queries that are interspersed with updates, in time $O(n)$ per query. In every query, the algorithm is given a vertex $v\in V(\hat G_{\sset})$, and needs to return an path from $v$ to $s$ of length at most $(1+\eps)\dist(s,v)$, if $D\leq \dist(s,v)\leq 2D$; otherwise it returns $\infty$.
\end{theorem}

%In the above theorem, an edge $e=(u,v)$ is eligible for insertion if the insertion of $e$ does not decrease $\dist(s,x)$ for any $x\in \hat G$.

The data structure from Theorem~\ref{thm: WSES} is denoted by $\WSES(G,D,s)$
%Notice that if all edge weights are unit, then the running time of $\WSES(G,D,s)$ becomes $O(mD)$ as before. But if many edges have large weights, we may save on the running time.








%The second data structure is Even-Shiloach trees (ES-trees). Unlike the connectivity data structure that we use in a black-box manner, we will need to make some extensions to ES-trees (similar to those in~\cite{BernsteinChechik,Bernstein}). In the next subsection, we describe the ES-trees and the necessary extensions.


%----------------------------------
%----------------------------------
%----------------------------------
\section{Proof of Theorems~\ref{thm: EEST}, \ref{thm: EESF}, \ref{thm: WSES}}

\mynote{This section goes to Appendix}

In this section we prove Theorems~\ref{thm: EEST}, \ref{thm: EESF} and \ref{thm: WSES}. All data structures in these theorems are based on \ESTs, that we describe in the following subsection.


%----------------------------------
%----------------------------------
%----------------------------------
\subsection{ES-Trees}\label{subsec: ES-trees}
%----------------------------------
%----------------------------------
%----------------------------------
Even-Shiloach tree (\EST) is a deterministic data structure for decremental single-source shortest-path. Given a graph $G=(V,E)$ with integral weights $w(e)\geq 1$ on its edges $e\in E$, a source $s$, and a distance bound $D\geq 1$, the data structure maintains, for every vertex $v$ with $\dist(s,v)\leq D$, the distance $\dist(s,v)$, under three operations:

\paragraph{Edge Deletion.} In this operation, denoted by $\ESTDEL(G,e)$, we are given an edge $e\in E(G)$, that is deleted from the graph.

\paragraph{Vertex Insertion.} In this operation, denoted by $\ESTVIN(G,v)$, we are given a new isolated edge $v$ that is added to the graph.
\paragraph{Edge Insertion.} In this operation, denoted by $\ESTIN(G,e)$, we are given an eligible edge $e=(u,v)$ that is inserted into $G$. An edge is eligible if either (i) at least one endpoint of $e$ is an isolated vertex; or (ii) the insertion of $e$ into $G$ does not decrease $\dist(s,x)$ for any $x\in V(\hat G)$.

We denote the corresponding data structure, that we describe below, by $\EST(G,s,D)$. %When the distance bound $D$ is unbounded (that is, $D=nW$, where $W=\max_{e\in E}\set{w(e)}$), then we denote the data structure by $\EST(G,s)$.
The total running time of the algorithm, including the initialization and updates, is $O(mD\log m)+O(n)$, where $m$ is the total number of edges that were ever present in the graph, and $n$ is the total number of vertices ever present in the graph.


Throughout the algorithm, we maintain a shortest-path tree $T$ from $s$, up to distance $D$. The algorithm is partitioned into phases, where in every phase one of the operations $\ESTDEL,\ESTVIN$ or $\ESTIN$ is performed, and the data structure is updated -- we call the latter step an update procedure. 

The algorithm uses a number of heaps, where the number of elements in each heap is bounded by $m$. We perform basic operations on heaps, that include: returning an element with smallest key; inserting an element; and deleting an element. Each such operation can be executed in $O(\log m)$ time. We let $\eta=c\log m$ for large enough constant $c$, so that in time $\eta$ we can execute a constant number (say $20$) of basic heap operations. 

\subsubsection{The Data Structure}
Throughout the algorithm, we maintain a shortest-path tree $T$ from $s$, up to distance $D$. We also maintain, for every vertex $v\in V$, a label $\delta(v)$. The algorithm guarantees that for all $v\in V$, if $\dist(s,v)\leq D$, then $\delta(v)=\dist(s,v)$, except during an update procedure for $\ESTDEL$, when it only guarantees that $\delta(v)\leq \dist(s,v)$. If $\dist(s,v)>D$, then the algorithm guarantees that $\delta(v)=\infty$ and $v\not \in T$.

For every vertex $v\in V$, we maintain a heap $H(v)$, that stores, for every neighbor $u$ of $v$ in $G$, the vertex $u$ with the key $w(u,v)+\delta(u)$. Vertex $v$ has pointers to all its copies in the heaps of all its neighbors.

\paragraph{Initialization.}
To initialize, we build a shortest-path tree $T$ from $s$, using the algorithm of Thorup~\cite{linear-sssp} in $O(m)$ time, and compute the labels $\delta(v)$ for all vertices $v\in V$. We also initialize the heaps $H(v)$ for every vertex $v$. In order to do so, for every vertex $v\in V$, we start with an empty heap $H_v$, and then, for every neighbor $u$ of $v$, we insert the vertex $u$ into $H_v$ with the key $\delta(u)+w(u,v)$, adding pointers between $u$ and its copy in $H_v$.  All this can be done in time $O(m)$.


\subsubsection{Edge Deletion}
The bulk of the work in \ESTs is done in the \ESTDEL operations. In this subsection, we assume that only \ESTDEL operation is allowed and describe the \EST algorithm; later we will extend it to include the remaining operations. We now describe an update procedure for $\ESTDEL$ operation.


Over the course of the update procedure, we inspect a number of vertices. An inspection of a vertex $v$ consists of a constant number of basic heap operations, and its running time is bounded by $\eta$.
The key invariant of the algorithm, that allows us to bound its total running time, is that we only inspect a vertex $v$ in one of the following three cases:

\begin{enumerate}
\item If an edge incident to $v$ is deleted -- there can be at most $2m$ such inspections over the course of the algorithm;

\item If $\delta(v)$ increases -- this can happen at most $D$ times for each vertex $v$, so the total number of such inspections, over the course of the algorithm,  is bounded by $nD$; %Each such inspection is charged to the vertex $v$; 
and

\item If $\delta(u)$ increases for one of the neighbors of $u$. For every vertex $v$, for each increase of $\delta(v)$, we may need to inspect up to $d(v)$ vertices -- the neighbors of $v$ in $G$. As $\delta(v)$ may grow at most $D$ times, the total number of such inspections, over the course of the algorithm, is bounded by $\sum_{v\in V}D\cdot d(v)=O(mD)$. %If we inspect $u$ because $\delta(v)$ increases for one of its neighbors $v$, we charge this inspection to the edge $(u,v)$, so every edge is charged at most $2D$ times.
\end{enumerate}

Clearly, if the above invariant holds throughout the algorithm, the total update time of the algorithm is $O(mD\eta)=O(mD\log n)$. (Recall that for now we only allow \ESTDEL operations.)




\paragraph{Update Procedure.}
Consider a phase when some edge $e=(u,v)$ is deleted from the graph. If this edge does not belong to the current tree $T$, then the distances $\dist(s,x)$ for vertices $x\in V$ do not change, and we terminate the update procedure. Therefore, we assume from now on that $e$ is an edge of the tree $T$, and we assume w.l.o.g. that $u$ is the parent of $v$ in $T$. Let $T_v$ be the sub-tree of $T$ rooted at $v$. Note that $\dist(s,v)$ may change as the result of deleting $e$, and this change may propagate to vertices of $T_v$.


Throughout the update procedure, we will maintain a heap $H$, containing vertices of $T_v$ that we need to inspect. The key stored with each vertex $x$ in $H$ is the current value $\delta(x)$. As the update procedure progresses, $\delta(x)$ may grow. 
At the beginning, $H$ contains a single vertex -- the vertex $v$.
Over the course of the algorithm, every vertex $x$ of $T_v$ is in one of the following four states:

\begin{itemize}
\item {\bf Untouched:} we have never inspected $x$, and it is not currently attached to the tree $T$. If $x$ is untouched, then it does not belong to $H$, and we do not know whether $\dist(s,x)$ has increased. The value $\delta(x)$ did not change during the current update procedure yet.
\item {\bf Settled:} we attached $x$ to the tree, and its current value $\delta(x)=\dist(s,x)$ in the new graph. A settled vertex does not belong to the heap $H$.
\item {\bf Suspicious:} We have added $x$ to the heap $H$ but we did not inspect it yet, and $\delta(x)$ has not changed yet. However, if $y$ is the parent of $x$ in $T_v$, then $\delta(y)$ has increased. A suspicious vertex is not attached to the tree $T$; and
\item {\bf Changed:} we have increased $\delta(x)$ in the current iteration, but we do not yet know the value of $\dist(s,x)$. All changed vertices belong to $H$, and a changed vertex is not attached to the tree. When a vertex becomes changed for the first time, all its children are added to $H$ as suspicious vertices.
\end{itemize}



Intuitively, if we consider the tree $T_v$ during any point of the update procedure, then the vertices that were added to $H$ over the course of the update procedure so far (including the vertices that later became settled) induce a connected sub-tree of $T_v$ that includes $v$. Let us denote this sub-tree by $T'$. The leaves of $T'$ are the vertices $x$ for which $\delta(x)$ has not yet changed -- these are the vertices that were added to $H$ as suspicious vertices but have not yet become changed vertices; some of them may have become settled. The inner vertices of $T'$ are those vertices $x$ for which $\delta(x)$ has increased over the course of the update procedure -- these are the vertices that became changed, and some of them may have become settled. As we will see, if any vertex $x$ is untouched, then it has some ancestor that currently belongs to the heap $H$ as a suspicious vertex.


Formally, we ensure that throughout the update procedure, the following invariants hold:

\begin{properties}{I}
\item For all $x\in T_v$, $\delta(x)\leq \dist(s,x)$. Moreover, if $x$ is a settled vertex, then $\delta(x)=\dist(s,x)$; \label{inv: delta}

\item For all $x\in T_v$, if $x$ is or was a changed vertex, then all its children were added to $H$ when $x$ became changed; and \label{inv: changed children}

\item If $x\in T_v$ is an untouched vertex, then some ancestor of $x$ is currently a suspicious vertex. \label{suspicious: ancestor}
\end{properties}

Assuming that the above invariants hold, we obtain the following observation.

\begin{observation}\label{obs: smallest key}
Let $x$ be a vertex in $H$, with minimum $\delta(x)$, and let $y\in H_x$ be the vertex minimizing $\delta(y)+w(x,y)$. Assume further that $ \delta(y)+w(x,y)\leq \delta(x)$. Then either $y\in T\setminus T_v$, or $y$ is settled; in other words, $y$ is currently attached to $T$. Moreover, $\delta(x)=\delta(y)+w(x,y)$.
\end{observation}
\begin{proof}
Assume that $y$ is not currently attached to $T$. Then either $y\in H$, or $y$ is untouched. If $y\in H$, then $\delta(y)\geq \delta(x)$ from the choice of $x$, and, since $w(x,y)\geq 1$, it is impossible that $\delta(y)+w(x,y)\leq \delta(x)$. Therefore, $y$ is untouched. But then $y$ has an ancestor $y'$ that is a suspicious vertex. Therefore, $\delta(y')$ did not grow during the current update operation yet, and so $\delta(y')<\delta(y)$ still holds. As $y'$ is a suspicious vertex, $y'\in H$. From the choice of $x$, $\delta(x)\leq \delta(y')<\delta(y)$, a contradiction. Therefore, $y$ is currently attached to the tree $T$.

From Invariant~\ref{inv: delta}, $\delta(y)=\dist(s,y)$, and $\delta(x)\leq \dist(s,x)$. Since there is a path from $x$ to $s$ of length $\delta(y)+w(x,y)\leq \delta(x)$, it follows that $\delta(x)=\delta(y)+w(x,y)$.
\end{proof}

We are now ready to describe the update procedure. At the beginning, the heap $H$ only contains the vertex $v$, which is a suspicious vertex. All other vertices of $T_v$ are untouched. Observe that all invariants hold. We now describe an iteration of the update procedure, assuming that all invariants hold at the beginning of the iteration.

Let $x\in H$ be the vertex with the smallest key $\delta(x)$. If $\delta(x)>D$, then we terminate the update procedure -- every vertex $y$ that is not currently attached to the tree $T$ has $\dist(s,y)>D$. Each such vertex either belongs to $H$, or is a descendant, in the original tree $T_v$, of a vertex in $H$. For each such vertex $y$, we set $\delta(y)=\infty$, and we delete $y$ from the heaps of its neighbors. Notice that this operation is performed at most once per vertex over the course of the algorithm, and contributes at most $O(m\eta)$ to the total running time.

Therefore, we assume that $\delta(x)\leq D$. Let $y\in H_x$ be the vertex minimizing $\delta(y)+w(x,y)$. We now consider two cases. The first case happens when  $\delta(y)+w(x,y)\leq \delta(x)$. Then, from Observation~\ref{obs: smallest key}, $y$ is currently attached to the tree $T$, and $\delta(y)+w(x,y)= \delta(x)$. We attach $x$ to the tree $T$ as a child of $y$, and $x$ becomes a settled vertex. (Note that if $x$ was not yet inspected in this update procedure, that is, we never changed $\delta(x)$, then all its descendants are untouched, and they get attached to the tree together with $x$. In that case, all descendants of $x$ become settled vertices. Otherwise, $x$ was a changed vertex at the beginning of this iteration, and so all its children were added to the heap $H$. We do not reattach any of its descendants to the tree then.) It is immediate to verify that all invariants continue to hold.

Otherwise, $\delta(y)+w(x,y)> \delta(x)$. Then from Invariant~\ref{inv: delta}, we know that the current estimate of $\delta(x)$ is too small. We then increase $\delta(x)$ by $1$ and return $x$ to $H$. If this is the first time that $\delta(x)$ is increased in the current iteration, then it becomes a changed vertex, and all its children in the tree $T_v$ become suspicious and are added to the heap $H$. In any case, we update the key of $x$ in the heaps $H_z$ for all neighbors $z$ of $x$.  It is immediate to verify that all invariants continue to hold.

We now analyze the running time of the update procedure. Consider an iteration when a vertex $x$ is processed. We need to perform two basic heap operations: delete $x$ from $H$ and find the smallest element of $H_x$. We now consider two cases. The first case happens when  $\delta(x)$ increases in the current iteration. Then we need to update all the heaps $H_z$ of every neighbor $z$ of $x$, where each update involves a single basic heap operation (increase the key associated with $x$). Additionally, for every child vertex $z'$ of $x$ that becomes suspicious but never becomes changed, we will later inspect $z$, and charge the processing time of this inspection to $x$. 

Assume now that $\delta(x)$ does not increase, that is, $x$ becomes a settled vertex. If $x$ was a changed vertex, then we charge this inspection of $x$ to $x$ itself. If $x$ was a suspicious vertex, then this inspection (that only involves two basic heap operations) is charged to its (changed) parent in the tree (in the case where $x=v$, we charge the deleted edge $(u,v)$). We do not need to explicitly update the status of its descendants to ``settled'': the algorithm naturally ensures that these vertices are never added to $H$.

Overall, the inspection of a vertex requires a constant number of calls to basic heap operations, and we assume that the running time of such an inspection is at most $\eta$. A vertex $x$ is inspected either when it is incident to an edge that was deleted, or if $\delta(x)$ grows, or if there is some neighbor $z$ of $x$, such that $\delta(z)$ grows. As discussed above, the total update time of the algorithm is then bounded by $O(mD\eta)=O(mD\log n)$.
So far we have assumed that only $\ESTDEL$ operations are allowed. Next, we extend this algorithm to handle $\ESTIN$ and $\ESTVIN$ operation.



\subsubsection{Edge Insertion and Vertex Insertion}
Recall that in $\ESTVIN(G,v)$ operation, we are given a new vertex $v$, that is inserted into $G$ as an isolated vertex. In this case, we simply initiate $H_v=\emptyset$, and set $\delta(v)=\infty$.

In the $\ESTIN(G,e)$ operation, we are given an edge $e=(u,v)$ that does not currently belong to $G$, such that either the insertion of $e$ does not decrease the distances between any pair of vertices, or at least one of the endpoints of $e$ is an isolated vertex. We need to insert the edge $e$ into $G$. 

Assume first that neither endpoint of $e$ is an isolated vertex. Notice that in that case, the tree $T$ does not change, and neither do the labels $\delta(x)$ for vertices $x\in V$. We update the heaps $H_u$ and $H_v$ by inserting $v$ into $H_u$ with key $\delta(v)+w(u,v)$, and $u$ into $H_v$, with key $\delta(u)+w(u,v)$, using two basic heap operations.

Assume now that endpoint $v$ of $e$ is an isolated vertex. If $u$ is not attached to $T$, then no update in the data structure is necessary. Therefore, we assume that $u$ is attached to $T$. We modify the tree $T$ by attaching $v$ as a child of $u$, and set $\delta(v)=\delta(u)+w(e)$. As before, we update the heaps $H_u$ and $H_v$ by inserting $v$ into $H_u$ with key $\delta(v)+w(u,v)$, and $u$ into $H_v$, with key $\delta(u)+w(u,v)$, using two basic heap operations.


We now analyze the total running time of the algorithm, including all three operations: \ESTIN, \ESTDEL, and \ESTVIN. 

Let $E_0$ be the set of all edges that were present in the original graph, and let $E_1$ be the set of all edges that were inserted through \ESTIN operation. We denote $m=|E_0\cup E_1|$. As before, if an edge is deleted and then inserted back, then we count this as two different edges.

Recall that $\eta=O(\log m)$ is an upper bound on the time spent on inspection of a single vertex, which involves a constant number of basic heap operations.
For every vertex $v$ in the graph $G$, we define its potential as follows. If $v$ is currently attached to $T$, then $\phi(v)=(D+1-\delta(v))\cdot d(v)\cdot \eta$, and otherwise $\phi(v)=0$. The potential of the graph $G$ is defined to be $\phi(G)=\sum_{v\in V(G)}\phi(v)$.

We now analyze the change in the potential and the running time of each procedure.

\paragraph{\ESTDEL.} We claim that the amount of time spent on an update procedure of \ESTDEL is bounded by the decrease of the potential $\phi(G)$. Indeed, if $e=(u,v)$ is the edge that was deleted, then we may need to inspect one of its endpoints, say $v$ (if $e$ belongs to the tree $T$, and $u$ is the parent of $v$ in the tree). The inspection takes time at most $\eta$, but the potential of $v$ decreases by at least $\eta$, since its degree decreases by $1$. Additionally, for every vertex $x\in T(v)$, if $\delta(x)$ decreases by $\Delta$, then we may spend $\Delta\eta d(x)$ time on inspecting $x$ and its neighbors (as $\delta(x)$ may increase up to $\Delta$ times). 
The potential of $x$ decreases by $\Delta\eta d(x)$, so the total time spent on inspecting $x$ and its neighbors that is charged to $x$ is bounded by the decrease in $\phi(x)$.
Recall that if, during the update procedure, the vertex $x\in H$ with minimum value $\delta(x)$ has $\delta(x)\geq D$ (in which case equality must hold as we increase $\delta(x)$ by at most $1$ at a time), then our algorithm processes each vertex $z$ that is not currently attached to $T$ and sets
$\delta(z)=\infty$, while also deleting $z$ from the heaps of its neighbors. Let $V'$ denote the set of vertices that are not currently attached to $T$. Every vertex in $V'$ either belongs to $H$, or it is a descendant, in $T_v$, of a vertex in $H$, so we an process all vertices in $V'$ in time $\sum_{z\in V'}d(z)\eta$. However, the potential of every vertex  $z\in V'$ decreases by at least $\eta d(z)$, and so overall, the total time spent on the update procedure is bounded by the total decrease in the potential.




\paragraph{\ESTVIN.} This procedure does not change $\phi(G)$, and it takes $O(1)$ time per vertex insertion. The total running time spent on $\ESTVIN$ procedure is then bounded by $O(n)$.


\paragraph{\ESTIN.} After each edge-insertion operation, the potential increases by at most $2(D+1)\eta$, as the endpoints of the inserted edge $e$ may have their potential increase by $(D+1)\eta$ each. The amount of time we spend on a single edge insertion is $2\eta$. 

Let $G_0$ be the graph $G$ at the beginning of the algorithm. We conclude that the total running time of the algorithm is bounded by $\phi(G_0)+O(n)+O(D\eta |E_1|)=O(mD\eta)+O(n)=O(mD\log m)+O(n)$.


\paragraph{Shortest Path Queries.}
Suppose, at any time during the algorithm's execution, we get a shortest-path query for a vertex $v$. We can check whether $\dist(s,v)\leq D$ in $O(1)$ time by checking $\delta(v)$. If $\delta(v)\leq D$, then we can return the path in $T$ connecting $v$ to $s$ in time $O(n)$. Therefore, shortest-path queries can be answered in $O(n)$ time.


%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
\subsection{Proof of Theorem~\ref{thm: EEST}}

%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
We simply maintain an \EST for the graph $\hat G$, with the source vertex $s$ and the distance bound $D$. The operations $\EESTIN(\hat G,e)$, $\EESTVIN(\hat G,v)$ and $\EESTDEL(\hat G,e)$ will be implemented by $\ESTIN(\hat G,e)$, $\ESTVIN(\hat G,v)$ and $\ESTDEL(\hat G,e)$, respectively. We only need to show how $\EESTSPLIT(\hat G,S,S')$ is implemented. The idea is to implemented through existing operations, $\ESTVIN,\ESTIN$, and $\ESTDEL$.

Suppose we are given a cluster $S\in \sset$, that we need to split into two clusters: cluster $S'\subseteq S$ whose elements are given explicitly, and cluster $S''=S\setminus S'$. We proceed as follows:

\begin{enumerate}
\item Insert a new isolated vertex $v_{S'}$ into $\hat G$, by running $\ESTVIN(\hat G,v_{S'})$; we also rename $v_S$ as $v_{S''}$.

\item Let $x\in S'$ be the vertex with minimum $\delta(x)$. Insert the edge $e_x=(v_{S'},x)$ of weight $1/2$ into $\hat G$ through the $\ESTIN(\hat G,e_x)$ operation. Note that $e_x$ is an eligible edge since $v_{S'}$ is an isolated vertex.

\item For each $y\in S'\setminus\set{x}$, insert the edge $e_y=(v_{S'},y)$ of weight $1/2$ into $\hat G$ through the $\ESTIN(\hat G,e_y)$ operation. We will show later that $e_y$ is an eligible edge. \label{cluster-splitting-edge-insertion-step}

\item For each $z\in S'$, delete the edge $e'_z=(v_{S''},z)$ from $\hat G$ through the $\ESTDEL(\hat G,e'_z)$ operation.
\end{enumerate}

It is clear that the above algorithm updates the graph $\hat G$ correctly. We now show that every edge inserted in Step~{cluster-splitting-edge-insertion-step} is an eligible edge. Let $y\in S'\setminus\set{x}$, and let $e_y=(v_{S'},y)$ be the newly inserted edge. Assume for contradiction that the insertion of $e_y$ into $\hat G$ decreases $\dist(s,a)$ for some vertex $a\in V(\hat G)$. 
Assume first that $a\neq v_{S'}$. The new shortest path from $a$ to $s$ has to contain the new edge $e_y$ and hence the vertex $v_{S'}$. However, every neighbor of $v_{S'}$ is also a neighbor of $v_{S''}$, and so we could replace $v_{S'}$ with $v_{S''}$ on this path, obtaining a path of the same length in the original graph. Therefore, $a=v_{S'}$ must hold. But then the length of the new shortest path from $v_{S'}$ to $s$ becomes $\delta(y)+1/2$. But from the choice of $x$, this is at most $\delta(x)+1/2$, a contradiction. 
We conclude that all edges inserted over the course of the procedure were eligible edges.

We now bound the total number of vertices and edges that were inserted into the graph as a part of cluster splitting operation. Notice that when a cluster $S$ is split into $S'$ and $S''$, with $|S'|\leq |S''|$, we insert one new vertex and $|S'|$ new edges into the graph: one edge incident to every vertex of $S'$. We say that every vertex of $S'$ is responsible for the unique new edge that is inserted into the graph and is incident to it. Since $|S'|\leq |S|/2$, every regular vertex of $G$ will be responsible for at most $\log n$ edge insertions, and the total number of edges inserted into the graph due to cluster splitting is $O(n\log n)$. It is easy to verify that the total number of vertices inserted into the graph due to cluster splitting is $O(n)$.

Let $m$ be the total number of regular edges that were ever present in $G$ -- these are the edges that were either originally present in $G$, or were inserted through $\EESTIN$ operation. From the analysis of \ESTs, we get that the total running time of $\EEST$ is $O((m+n\log n)D\log(m+n\log n)$.

The shortest path queries are handled exactly like in the \EST algorithm, with running time $O(n)$ per query.

\newpage
%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
\subsection{Proof of Theorem~\ref{thm: EESF}}

%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
In addition to \ESTs, we need to use another data structure that supports connectivity queries in a given unweighted undirected graph undergoing edge insertions and edge deletions. We use the results of~\cite{dynamic-connectivity}, who provide a deterministic data structure, that we denote by $\CONN(G)$, that, given an $n$-vertex unweighted undirected graph $G$, that is subject to edge deletions and edge insertions, responds to each connectivity query in $O(\log n/\log\log n)$ time, and has amortized update time of $O(\log^2n)$ per edge deletion or insertion.  In a connectivity query, the input is a pair $u,v$ of vertices of $G$, and the output is ``yes'' if $u$ and $v$ are connected in $G$, and ``no'' otherwise.
We denote by $\CONNIN(G,e)$ and by $\CONNDEL(G,e')$ the procedures for inserting an edge $e$ into and deleting an edge $e'$ from the data structure, respectively. We also denote by $\conn(G,u,u')$ the connectivity query for $u$ and $u'$ in the data structure.

We now describe all data structures that we use.
First, we maintain the data structure $\CONN(\hat G)$ for the graph extended graph $\hat G$ of $G$ (in fact, we will maintain it for a graph consisting of $\hat G$ and $O(n)$ additional isolated vertices, that may be later used as new super-nodes; abusing the notation we still denote the data structure by $\CONN(\hat G)$). We also maintain a list $\cset$ of connected components of $\hat G$, and, for every vertex of $\hat G$, a pointer from that vertex to the connected component of $\cset$ to which it belongs. For every component $C\in \cset$, we maintain a source vertex $s(C)\in V(C)$, and data structure $\EST(C,s(C),D(C)$, where $D(C)=|C|/\gamma$.

\paragraph{Initialization.}
In order to initialize data structure $\CONN(\hat G)$, we start with a graph whose vertex set consists of all vertices of $G$, and $2n$ additional vertices, that will be exploited as super-nodes (these include the super-nodes in the original graph $\hat G$, and new super-nodes that arise from vertex splitting). We then add the edges of $\hat G$ to $\CONN(\hat G)$ one-by-one, using $\CONNIN(\hat G,e)$ operation. We initialize the list of connected components of $\hat G$, and, for each such component $C\in \cset$, we select an arbitrary vertex $s(C)$ as its source, and construct a shortest-path tree, initializing the data structure $\EST(C,s(C),D(C))$. If we ignore the operations $\CONNIN(\hat G,e)$, that will be analyzed separately, the total running time of the initialization step is $O(|E(\hat G)|)=O(m)$.

Next, we describe the implementation of procedures $\EESFDEL$, $\EESFIN$ and $\EESFSPLIT$. As before, the bulk of the work is done in procedure $\EESFDEL$.

Procedure $\EESFDEL$ is described in Figure~\ref{fig: EESFDEL}. Recall that in this procedure we are given a regular edge $e=(u,v)$ that is deleted from $G$, and hence from $\hat G$.

\begin{figure}
\program{$\EESFDEL(\hat G,e=(u,v))$}{

Let $C$ be the connected component of $\cset$ that contains $e$ -- we can find it since the endpoints of $e$ point to it, and let $T(C)$ be the tree maintained by $\EST(C,s(C),D(C))$. 



\begin{enumerate}
\item Execute $\CONNDEL(\hat G,e)$. Check whether $u$ and $v$ are still connected in the new graph $\hat G$, by calling procedure $\conn(\hat G,u,v)$.

\item If $u,v$ are still connected in the new graph, execute $\ESTDEL(C,e)$ and terminate the algorithm.

From now on we assume that $u,v$ are no longer connected in $\hat G$. In particular, $e$ must be an edge of the tree $T(C)$. Assume w.l.o.g. that  $u$ is the parent of $v$ in $T(C)$. Let $T_v$ be the sub-tree of $T(C)$ rooted at $v$, and let $T'=T(C)\setminus T_v$. Note that $C$ now splits into two connected components: one spanned by $V(T_v)$, and one spanned by $V(T')$. The next step establishes which of the two components contains fewer vertices.


\item  \label{step: BFS} Perform a BFS of $T_v$ from $v$ and a BFS of $T'$ from $s(C)$ in parallel, so both algorithms discover the same number of vertices at each step. Terminate the algorithm once all vertices in one of the two trees are explored. We assume w.l.o.g. that it is $T_v$; the other case is dealt with symmetrically.

\item 
Denote the connected component of $\hat G$ corresponding to $T_v$ by $C'$, and the connected component corresponding to $T'$ by $C''$. Set $s(C')=v$ and $D(C')=|C'|/\gamma$. Set $s(C'')=s(C)$ and $D(C'')=|C''|/\gamma$.

 Notice that $T_v$ is a shortest-path tree for $C'$ and $s(C')$, and $T'$ is a shortest-path tree of $C''$ and $s(C'')$. 
 
 \item Add $C'$ to the list $\cset$ of connected components of $\hat G$ and add pointers from every vertex of $C'$ to $C'$; rename $C$ by $C''$ in $\cset$. \label{last step of EESF-delete}
 
 
\item Delete $v$ from $H_u$ and delete $u$ from $H_v$ in $\EST(C,s(C),D(C))$.\label{step: delete mutually from heaps}

\item Initialize new data structure $\EST(C'',s(C''),D(C''))$, whose shortest path tree is $T'$; the labels $\delta(x)$ of vertices and their heaps $H_x$ remain the same as in $\EST(C,s(C),D(C)$.

\item Initialize new data structure $\EST(C',s(C'),D(C'))$, whose shortest path tree is $T_v$. Notice that the labels $\delta(x)$ for $x\in T_v$ have changed, and need to be set to $d(x,v)$ instead of $d(x,s(C))$. However, for each $x\in V(T_v)$, $d(x,v)=d(x,s(C))-\delta(v)$, where $\delta(v)$ is the label of $v$ before the current update. Instead of updating the labels $\delta(x)$ and keys of vertices in heaps $H_x$, we keep the same labels and the same heaps and simply remember the value $\offset(C')=\delta(v)$. Throughout the rest of the algorithm we treat each label $\delta(x)$ as $d(v,x)+\offset(C')$.  (We may not be able to afford to update all labels $\delta(x)$ for $x\in V(T_v)$, if $T_v$ contains more than half the vertices of $C$). 


\end{enumerate}
}
\caption{Procedure \EESFDEL\label{fig: EESFDEL}}
\end{figure}



In order to execute procedure $\EESFIN(\hat G,e=(u,v))$, recall that $u$ and $v$ must belong to the same connected component of $\hat G$, that we denote by $C$, and that the insertion of $e$ cannot decrease $\dist(s(C),x)$ for any vertex $x\in V(C)$. We simply run the procedure $\ESTIN(C,e)$. 

Finally, procedure $\EESFSPLIT(S,S')$ is again implemented by combining calls to $\EESFDEL,\EESFIN$, and $\ESTVIN$ as before. Since we will need to slightly modify this procedure later, we provide its full description in Figure~\ref{ffig: EESFSPLIT}.

\begin{figure}
\program{$\EESFSPLIT(\hat G,S,S')$}{
Input: set $S\in \sset$, subset $S'\subseteq S$ given explicitly, with $|S'|\leq |S|/2$. Let $C\in \cset$ be the connected component of $\hat G$ containing vertex $v_S$.

\begin{enumerate}
\item Insert a new isolated vertex $v_{S'}$ into $C$, by running $\ESTVIN(C,v_{S'})$. Rename $v_S$ as $v_{S''}$ in $\EST(C,s(C),D(C))$ and $\CONN(\hat G)$. Select an arbitrary isolated vertex of the graph maintained by $\CONN(\hat G)$ that does not currently participate in $\hat G$ and name it $v_{S'}$. 
 

\item Let $x\in S'$ be the vertex with minimum value $\delta(x)$ in $\EST(C,s(C),D(C))$. Insert the edge $e_x=(v_{S'},x)$ of weight $1/2$ into $\hat G$ by running $\ESTIN(\hat G,e_x)$ and $\CONNIN(\hat G,e_x)$. Note that $e_x$ is an eligible edge  for \ESIN since $v_{S'}$ is an isolated vertex. \label{SPLIT - insert first edge}

\item For each $y\in S'\setminus\set{x}$, insert the edge $e_y=(v_{S'},y)$ of weight $1/2$ into $\hat G$ by running $\ESTIN(\hat G,e_y)$ and $\CONNIN(\hat G,e_y)$. As in the analysis of $\EESTSPLIT$, edge $e_y$ is an eligible edge for \ESIN. \label{cluster-splitting-edge-insertion-step}

\item For each vertex $z\in S'$, delete the edge $e'_z=(v_{S''},z)$ from $\hat G$ by running $\EESFDEL(\hat G,e'_z)$ and $\CONNDEL(\hat G,e'_z)$. \label{cluster splitting - delete extra edges}
\end{enumerate}
}
\caption{Procedure \EESFSPLIT. \label{ffig: EESFSPLIT}}
\end{figure}

Notice that it is possible that $v_S$ was the source vertex $s(C)$ of the cluster $C$; in that case, the new vertex $v_{S''}$ becomes a source vertex of $C$. It is also possible that following some calls to the $\EESFDEL$ operation, the cluster $C$ will be split into smaller clusters, and that one of these clusters will have the new super-node $v_{S'}$ as its source vertex.

Assume that the graph $\hat G$ before the call to procedure $\EESFSPLIT(\hat G,S,S')$ was $\gamma$-restricted, and that it remains so after the procedure is completed. For the sake of analysis, we need to show that $\hat G$ remains $\gamma$-restricted before every call to the $\EESFDEL$ procedure from within Procedure $\EESFSPLIT$. 
\mynote{need to fix this}


\paragraph{Analysis.}

Since the amortized update time for $\CONN(\hat G)$ is $O(\log^2n)$, the total amount of time spent on $\CONNIN$ and $\CONNDEL$ operations is bounded by $O(m\log^2 n)$. Moreover, we only call query $\conn(\hat G,u,u')$ when the edge $(u,u')$ is deleted from $\hat G$. So the number of such queries over the course of the algorithm is $O(m)$, and the total time spent handling them is $O(m\log n/\log\log n)$. The total running time associated with all calls to $\CONN(\hat G)$ over the course of the algorithm is $O(m\log^2n)$. From now on we ignore all such calls and analyze the remainder of the algorithm.



In order to do so, we define vertex potentials. Throughout the algorithm, for every vertex $v\in V(\hat G)$, we define the potential $\phi(v)$ as follows.  if $v$ is an isolated vertex then its potential $\phi(v)=0$. Otherwise, if $v$ belongs to a connected component $C\in \cset$, then $\phi(v)=(4D(C)-\dist(v,s(C)))d(v)\eta$, where $d(v)$ is the degree of $v$ in $G$, and $\eta=O(\log n)$ is time needed to perform a constant number of standard heap operations.
We then let $\phi(\hat G)=\sum_{v\in V(\hat G)}\phi(v)$.

Recall that for each connected component $C\in \cset$, $D(C)=|C|/\gamma$. Therefore, the total potential at the beginning of the algorithm is bounded by:

\[\phi(\hat G)=\sum_{v\in V(\hat G)}\phi(v)\leq \sum_{v\in V(\hat G)}\frac{4n\eta |E(\hat G)|}{\gamma}=O\left (\frac{nm\eta}{\gamma}\right).\]


Whenever an edge is inserted into $\hat G$, whether directly by $\EESFIN$ operation, or as part of $\EESFSPLIT$,  the total potential may increase by up to $\frac{4n\eta}{\gamma}$, and so the total increase in potential due to edge insertion is bounded by $O(nm\eta/\gamma)$.

Consider now an execution of procedure $\EESFDEL(\hat G,e=(u,v))$, that is either called directly, or as part of $\EESFSPLIT$ procedure. 
We assume that $\hat G$ was $\gamma$-restricted at the beginning of the call to $\EESFDEL$, and that it remains so after the edge $e$ is deleted from it. 
Assume that $u$ and $v$ lie in the connected component $C\in \cset$ at the beginning of the call to $\EESFDEL$. If $C$ remains connected after the deletion of $e$, then, ignoring the calls to the $\CONN$ data structure, we execute a single $\ESDEL$ operation. As discussed before, the time spent on executing this operation is bounded by the decrease in the potential $\phi(\hat G)$.

Assume now that, after $e=(u,v)$ is removed, component $C$ is split into $C'$ and $C''$, with $|C'|\leq |C''|$. Steps~\ref{step: BFS} and \ref{last step of EESF-delete} of Procedure $\EESFDEL$ take $O(|C'|)$ time in total. Since $|C'|\leq |C|/2$, the total time that the is spent on these steps over the course of the algorithm is $O(n\log n)$. We ignore these two steps from now on. The remaining steps of the procedure take $O(1)$ time, except for Step~\ref{step: delete mutually from heaps}, that takes time $2\eta$. However, as the potentials of $u$ and $v$ increase by at least $\eta$ each (since their degrees decrease by $1$), time spent on this step can be charged to the decrease in the potential. 

Finally, observe that, once we split $C$ into $C'$ and $C''$, we obtain the new bounds $D(C')$ and $D(C'')$ on the depths of these clusters, and the potentials of the vertices are updated accordingly. We show below that the potential of every vertex may only decrease. Assume w.l.o.g. that $C'$ is the cluster corresponding to the tree $T_v$ (but we no longer assume that $|C'|\leq |C''|$).   For every vertex $x\in V(C'')$, $\dist(x,s(C''))= \dist(x,s(C))$ holds, while $D(C'')<D(C)$, and so $\phi(x)$ may only decrease. We now consider some vertex $x\in V(C')$, and show that its potential also can only decrease. The original potential is:

\[\phi'(x)=(4D(C)-\dist(x,s(C)))d(x)\eta=\left (\frac{4|C|}{\gamma}-\dist(x,s(C))\right )d(x)\eta.\]

The new potential is:

\[\phi(x)=(4D(C')-\dist(x,v))d(x)\eta=\left (\frac{4|C'|}{\gamma}-\dist(x,v)\right )d(x)\eta.\]

In order to show that the potential does not increase, it is enough to show that:

\[\dist(x,s(C))-\dist(x,v)   \leq \frac{4(|C|-|C'|)}{\gamma}=\frac{4|C''|}{\gamma},\]

where all distances are before the deletion of the edge $(u,v)$.
But, since $v$ is on the shortest path from $x$ to $s(C)$, $\dist(x,v)=\dist(x,s(C))-\dist(v,s(C))$. Therefore, it is now enough to show that:

\[\dist(v,s(C))\leq \frac{4|C''|}{\gamma}.\]


First, if $C''$ consists of a single vertex (which must be $u$), then

Recall that $\dist(s(C''),u)\leq |C''|/\gamma$ must hold, since $C''$ has the relaxed $\gamma$-restricted property (@@@???), and $\dist(s(C''),v)\leq \dist(s(C''),u)+1\leq \frac{|C''|}{\gamma}+1$. We claim that $\frac{|C''|}{\gamma}\geq 1/2$ must hold: (???) \mynote{what if $C''$ only consists of $u$?}


Finally, we analyze Procedure $\EESFSPLIT(\hat G,S,S')$. The running time of this procedure, excluding the calls to $\ESDEL$, $\ESIN$, $\CONNIN$ and $\CONNDEL$ is $O(|S'|)$.



\paragraph{Shortest Path Queries}
 

\section{The Fix?}
\subsection{Problem Description}
The problem with the above approach is the following. It is possible that, when we remove an edge $e=(u,v)$ from $C$, cluster C splits into two sub-clusters. If $u$ is the father of $v$ in the shortest path tree $T(C)$, one sub-cluster will now have $v$ as its source and the sub-tree of $T(C)$ rooted at $v$ as its tree, the other cluster will have the old source and the remainder of the old tree. All this works well, except if $u$ is the root of $T(C)$, and $v$ is its only child. Then the distance of every vertex to $v$ (the new root) is strictly less than their distance from $u$. Now we allow them to go up to distance $|C|/\gamma$ from $v$ and not from $u$, so now each of them gains one additional potential future increase in the distance, which potentially can cost us $O(m)$ time overall.

Specific troublesome scenario: we start with a single cluster and build shortest-path tree $T$ rooted at some vertex $s$. Then the adversary repeatedly deletes all edges incident to $s$. If the last edge to be deleted is $(s,s')$, then our new source becomes $s'$. The adversary then switches to deleting all edges incident to $s'$, and so on. It looks like we could go on like that for $n$ iterations. If we consider some iteration $i$, and the current root of the tree is $s_i$, then, as we delete edges incident to $s_i$, it is possible that for every vertex, its distance to $s_i$ increases by 1, and it now connects to $s_i$ through the next root $s_{i+1}$. Because of this, we spend $O(m)$ time updating the whole data structure between the iterations. Then once we delete $s_{i}$, the distance to the new root decreases to what it was before, and so it goes on. Paying $O(m)$ per iteration, weÕll spend $O(mn)$ time overall.

We first describe a fix for the max flow problem (the fix will lead to $\poly\log n$-approximation for it, instead of $(1+\eps)$), and then we describe a fix for decremental single-source shortest path, where we support vertex deletions, and not edge deletions.

%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
\subsection{High-Level Description of the Fix}
%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
We focus on a graph $G_i$ that belongs to one of the levels, so it contains all vertices of  $G$, and all edges incident to vertices of degree $h$ to $2h$, in addition to super-nodes that we ignore for now. WeÕll work with every connected component $C$ of the graph individually. Consider one such component $C$, and assume that currently its average vertex degree in $G_i$ is $d$.


\begin{observation}\label{obs: avg degree}
$d\leq h$.
\end{observation}

\begin{proof}
Let $N'$ denote the number of heavy vertices in $C$ and let $N=|C|$. Then $|E(C)|=Nd/2$, but also from the definition of $G_i$, $|E(C)|\leq 2N' h$. Therefore, $2N'h \geq Nd/2$. Since $N\geq N'$, this means that $d\leq h$. 
\end{proof} 


 An iteration of the algorithm is when we find one path, so there are $n$ iterations. We say that one phase has passed w.r.t. $C$ if one of the following three happened:
 
 
 \begin{itemize}
 \item $d/10$ iterations have passed; or
 \item we have split $C$ into smaller connected components, each of which contains fewer than $|C|-d/\poly\log n$ vertices; or 
 
 \item we have deleted at least $d/\poly\log n$ vertices from $C$ (a vertex is deleted once it participates in $\alpha$ paths, or once its degree falls to below $h/2$ due to deletions of its neighbors).
 \end{itemize}
 
  We claim that, once a phase ends, we can afford to spend $O(|E(C)|)=O(d|C|)$ time to process $C$. Why this is true: if the phase ends due to the first reason, then we charge to each of the $d$ paths we found in this phase $|C|$ units. This gives us total charge of $d|C|$, which is sufficient. Combining over all clusters, each path is charged at most $n$ units, and there are at most $n$ paths, so the total charge over the course of the algorithm is $O(n^2)$. To handle the other two reason for termination of a path, we give to every vertex $v$ of $G_i$ a budget of $|C|poly log n$, where $C$ is the cluster to which $v$ belongs. The total budget of all vertices is $O(n^2polylog n)$. Assume now that $C$ is split into pieces, and let $C'$ be a piece (not necessarily connected) that contains fewer than $|C|/2$ vertices, but at least $d/\poly\log n$ vertices. Then the budget of every vertex in $C'$ went down by at least $(|C|\poly\log n)/2$, and, as $|C'|\geq d/\poly\log n$, the total decrease in the budget is at least $|C|d\poly\log n$, which is sufficient for us. If $d$ vertices are deleted from $C$, we can use all their budget, which is $d|C|\poly\log n$. 

From now on we focus on a single cluster $C$, with average vertex degree $d$. 


\begin{definition}
We say that a sub-graph $C'\subseteq C$ is a \emph{valid core} of $C$ if the following holds:

\begin{itemize}
\item $|C'|\geq d/10$ and every vertex in $C'$ has degree at least $d/4$ in $G_i$;
\item $C'$ contains no super-nodes;
\item There is a subset $\Gamma\subseteq C'$ of vertices, such that every vertex $v\in C'\setminus \Gamma$ has at least $d/4$ neighbors that lie in $C'$, and $|\Gamma|\leq |C'|/\log^zn$, for some constant $z$; and
\item Graph $C'$ is $1/\log^{z-1}n$-expanding with respect to vertex cuts.
\end{itemize}
\end{definition}

We assume now that we have computed a core $C'$ for $C$; we show how to do this below. We call the vertices of $C'\setminus \Gamma$ \emph{inner} vertices of $C'$, and vertices of $\Gamma$ are called \emph{boundary} vertices of $C$. Notice however that an inner vertex of $C$ is allowed to have a neighbor that does not lie in $C$.


We create a source vertex $s(C)$, that connects to every inner vertex  of $C'$ with an edge of length $1/2$. Then we construct an ES-tree of $C$, starting from $s(C)$, and going up to depth $|C|/\gamma$. We then proceed to run iterations (that is, reporting $s$--$t$ paths and updating the data structure based on congested vertices), until a phase is completed with respect to $C$. Once a phase is completed, we process $C$ from scratch (that is, we compute the core and the ES-tree of the resulting clusters). As long as a phase does not complete, if cluster $C$ gets split, then $s(C)$ remains connected to at least $d/10$ vertices in the first cluster, and we can use the current spanning tree for it, deleting the part that gets disconnected. The second cluster will contain fewer than $d/\poly\log n$ vertices (because the phase is not completed yet), and so in particular it may not contain a heavy vertex or a super-node; in other words, it becomes a collection of isolated vertices that can be ignored (but even if this did not happen, we could afford to recompute a core for the new cluster and the ES tree there from scratch: Since the number of vertices in that cluster is less than $|C|/2$, we can afford to do it (recompute ES-tree each time the cluster size decreases by factor 2)).

As before, an iteration consists of computing a single $s$-$t$ path $P$. But now the path is allowed to use the vertex $s(C)$, and we donÕt yet specify how it will be routed inside $C'$. When a phase ends, we are allowed to use $O(|E(C)|)$ time to reorganize things. Now we look at all paths that use $s(C)$. Their entry/exit points to $C'$ define a collection of demand pairs, where every vertex may participate in up to $\alpha$ demand pairs, where $\alpha$ is the allowed congestion. In the following subsection weÕll argue that we can connect these demand pairs inside $C'$ with congestion at most $\alpha\poly\log n$, in time $O(|E(C)|\poly\log n)$. A useful thing to notice is that  we only need to route all sources to all destinations to obtain a valid set of paths, we donÕt need to pair them correctly, but we do need to route them on short paths. WeÕll route them on paths of length at most $\poly\log n$.

Inside a single phase, all distances from $s(C)$ will be at most $n/h$. So the time we will spend is $|C|d\cdot  n/h\leq |C|n$ since $d\leq h$. (This is the only place where we need the layers. If we took all the layers together, then heavy vertices would have degree more than $h$, but it is possible that average vertex degree is much higher than $h$ which is a problem in the above calculation). 


We needed to take care of edge insertions and super-node splitting - this is how the different layers interact. Edge insertions can only help with the core, and in the ES-tree we treat them as usual. The only subtle point is that the insertion of edges may increase average degree, which affects our running time. But then once the average degree in $C$ doubles, we can recompute everything from scratch and make the edge insertions pay for that (the edge insertion happens when some heavy vertex from a higher level lost most of its degree and is demoted to the current level, together with all edges that it owns).

For splitting super-nodes: we can ensure that the core has no super-nodes, by deleting all super-nodes before the core is computed. This is OK to do because this deletion will decrease the average vertex degree by at most 1. Inside the ES-tree the splitting is done by first inserting a new isolated vertex that becomes one of the two new supernodes; inserting edges from this new supernode to the relevant vertices; and deleting some edges incident to the old super-node. All this is implemented by standard edge deletion and edge insertion operations. The only problem is that the cluster may split as the result of this operation, but this is treated exactly as before: we are now guaranteed that each of the 2 new clusters has at least $d$ vertices, and so the phase ends and we can recompute everything.


%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
\subsection{Routing in the Core}
%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
Now we have a graph $C'$ that is $1/\poly\log n$ expanding w.r.t. vertex cuts. For concreteness, letÕs make it $1/\log^4n$-expanding. We have a set $S$ of sources and a set $T$ of destinations, and we need to connect them with paths, but both $S$ and $T$ are multi-sets. A vertex may appear up to $\alpha$ times in $S$ or in $T$, where $\alpha$ is the allowed congestion.

We build a source $s$ connecting to everyone in $S$, and destination $t$ connecting to everyone in $T$, and then do single-source shortest paths from $s$ to $t$. We iteratively choose a path from $s$ to $t$ of length at most $\log^9 n$. A vertex that was used in more than $\alpha$ paths gets deleted. Also, every copy of a vertex in $S$ and in $T$ can be used at most once, so we will route a correct number of paths from each source/destination (as before weÕll make a special copy that will be used as a source/destination, and a regular copy that can be used up to $\alpha$ times as an inner vertex). This whole procedure, including the decremental shortest path, takes $O(|E(CÕ)|\poly\log n)$ time. We claim that at least $|S|/\poly\log n$ demand pairs are routed, so weÕll only run it $\poly\log n$ times.

Let $S',T'$ be the remaining sets to be routed, so there is no path of length less than $\log^9n$ from $S'$ to $T'$. Since they are multi-sets, let $S'',T''$ be the corresponding sets containing just 1 copy of each vertex, so $|S''|\geq |S'|/\alpha$, and $|T''|\geq |T'|/\alpha$. Assume that $|S''|<|T''|$. Every path from $S''$ to $T''$ has at least $\log^9 n$ vertices. So there is some vertex cut that separates $S''$ from $T''$ and it has sparsity less than $1/log^5n$ (if every cut had sparsity more than $1/log^5n$, we could have reached from $S''$ to $T''$ in $\log^6n$ steps). Let $(A,X,B)$ be this vertex cut, with $S''\subseteq A$, so that $|X|\leq |A|/\log^5n$. Originally, cut $A$ had vertex expansion $1/\log^4n$. So we have deleted at least $|A|/\log^5n$ vertices from the graph. Each vertex is deleted if it is used by $\alpha$ paths, and every path is using at most $\log^9n$ vertices. So we have routed at least $|A|\alpha/log^{14}n\geq |S''|\alpha/\log^{14}n\geq |S'|/\log^{14}n$ paths. If $|S'|\geq |S|/2$, thatÕs $|S|/\poly\log n$ paths. If $|S'|<|S|/2$, then we route $|S\setminus S'|\geq |S|/2$ paths.
So after $\poly\log n$ iterations like that we will be done.

%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
\subsection{Computing the Core}
%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
We assume that average vertex degree in $C$ is $d$. We delete all super-nodes from $C$ (that decreases average vertex degree by at most $1$, because the edges between the supernodes and the regular vertices are a collection of disjoint stars). We also iteratively delete from $C$ all vertices whose degree is less than $d/4$, so in the end we get a cluster $C'$, such that every vertex in $CÕ$ has degree at least $d/4$. Note that $C'$ may not even be connected - in such a case we let $C'$ be one of its connected components that is not an isolated vertex. We then iterate. In every iteration, we will try to find a $1/log^6n$-sparse vertex cut $(A,X,B)$ of $C'$ (we discuss below how to do it). Suppose we find it and suppose that $|A|\leq |B|$. Then we let $C'=C[A\cup X]$, and continue. The vertices of $X$ are added to the set $\Gamma$ of boundary vertices of $C'$. As we keep cutting the cluster, the boundary keeps on growing. But because of the sparsity value, at the end of the algorithm, if $\Gamma$ denotes set of all boundary vertices of $C'$, then $|\Gamma|\leq |C'|/\log^5n$. 

In particular, when we are done with our procedure, we obtain a connected cluster $C'$, with $\Gamma|\leq |C'|/\log^5n$. If $v$ is an inner vertex of $C'$, then all neighbors that $v$ had before we started computing the sparsest cuts (there were at least $d/4$ of them) belong to $C'$. Therefore, $|C'|\geq d/4$. It is now easy to verify that $C'$ is a valid core.

Note that there will only need $\log n$ sparsest cut calculations, and that we donÕt need to find sparsest cut: just a $1/\log^6n$-sparse cut, if say $1/\log^{10}n$-sparse cut exists. WeÕll need to use our $m\alpha$-time algorithm for this, with $\alpha=
\poly\log n$ (we didnÕt yet verify that the algorithm works; there is a part of it that depends on RaeckeÕs decomposition that needs to be checked).


Note that, if the above approach is used for max-flow with vertex capacities, we will incur a $\poly\log n$-congestion due to the routing in the cores, which might mean that we are only getting $\poly\log n$-approximation.

%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
\section{Decremental Single-Source Shortest Paths with Vertex Deletions}

%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
 
 Here we assume that we are allowed to delete vertices from the graph, and not edges Ñ this is what we need in any case for vertex cuts and flows. We can think of it as having $\log n$ different copies of every vertex, each of which corresponding to the different weights $2^i$. Once a vertex is used $i\alpha$ times, we delete the $i$th copy of this vertex from the graph. We may also need to delete a given vertex from a layer, if its degree fell enough due to the deletions of its neighbors. 

Consider now some layer $G_i$ as before, where heavy vertices have degrees between $h$ and $2h$. Let $C$ be some cluster in that layer, and let $d$ be the average vertex degree in $C$. We need to support vertex deletion, edge insertion (that does not decrease distances) and super-node splitting. We say that a phase ends with respect to $C$ if either (i) at least $d/\poly\log n$ vertices have been deleted, or (ii) cluster $C$ is split into pieces, each of which having fewer than $|C|-d/\poly\log n$ vertices (in the latter case, the smaller clusters will have no edges, since we need at least one heavy vertex with degree $h\geq d$ to have a cluster that is not an isolated vertex). As before, we can afford to spend $O(|E(C)|)$ time to recompute the data structure once a phase ends.

We compute the core $C'$ and set up the ES-tree exactly as before. We claim that, as long as fewer than $d/\poly\log n$ vertices are deleted from $C$, for every pair $u,v$ of {\bf inner} vertices of $C'$, there is a path of length at most $\poly\log n$ connecting them in $C'$.
Indeed, each of $u,v$ had at least $d/4$ neighbors inside $C'$, most of which survived. Let $S$ be the set of surviving neighbors of $u$, and $T$ the set of surviving neighbors of $v$. Set $S$ has at least $|S|/\log^4 n>d/\log^4n$ neighbors in $C'$ due to the expansion properties of the core, and most of them have survived. Add them to $S$. We keep going like that from both sides until they merge. So within each phase of the algorithm, we can route through the core via paths of length at most $\log^5n$. The question is how to find such paths.

Here is a trick to do it. Before the phase starts, we build an expander $H$ on $|C'|$ vertices and embed it into $C'$ via the cut-matching game, so that every edge $e$ of $H$ is mapped to a path $P(e)$ in $C'$; the length of the path is at most $\poly\log n$; and every vertex of $H$ participates in at most $\poly\log n$ such paths. WeÕll need to use the entropy-based algorithm with Raecke to do this, because weÕll only be able to route a constant fraction of the flow in each iteration, especially if we require short paths. If that part works out, we should be able to do it in $O(|E(C')|\poly\log n)$ time. Every vertex $v$ of $C'$ will keep a pointer to every edge $e$ of $H$, such that $v \in P(e)$.

When we delete a vertex $v$ from $C$, we delete all edges $e$ with $v\in P(e)$ from $H$. So as long as we delete fewer than $d/\poly \log n$ vertices from $C$, we delete at most $d/\poly\log n$ edges from H. Assume now that we are given two inner vertices $u$ and $v$ of $C'$, and we would like to connect them by a path. As before, $u$ had at least $d/4$ neighbors in $C'$, most of which are still alive; call this set $S$. Similarly, $v$ had at least $d/4$ neighbors in $C'$, most of which are still alive; call this set $T$. We now know that the expander $H$ contains a path of length $\poly\log n$, connecting $S$ to $T$, for the same reason as before: there are $|S|/\poly\log n$ edges in $H$ leaving $S$, most of which are still alive, and so on. We can spend $O(|E(H)|)$ time finding this path. This gives $O(|C'|\poly\log n)$ time per query to the core, which will result in $O(n \poly\log n)$ total time per query.

If this works, this should give an $O(n^2\poly\log n)$-time algorithm for flows with vertex capacities, giving $(1+\eps)$-approximation, that is, the $\poly\log n$ congestion due to routing in the core will be avoided.


%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
\iffalse

%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------

The algorithm of Bernstein uses the following setting, that we will also use several times. We are given a basic graph $G$, and additionally a collection $\cset=\set{C_1,\ldots,C_r}$ of  disjoint subsets of its vertices, each of which contains at least two vertices. We need to maintain a graph $\hat G$, that is defined as follows. Its set of vertices consists of two subsets: $V_1=V(G)$, and $V_2=\set{v_C\mid C\in \cset}$. We call the vertices of $V_1$ \emph{regular vertices}, and the vertices of $V_2$ \emph{super-nodes}. The set of edges also consists of two subsets: set $E_1$ of edges contains all edges of $G$, with the same weights (that we assume to be integers between $1$ and $W$), and set $E_2$ of edges is defined as follows: for every super-node $v_C$, for every regular vertex $u\in C$, we add an edge $(u,v_C)$ of weight $1/2$ to $\hat G$. Therefore, every edge of $E_2$ connects a super-node to a regular vertex, and the sum of degrees of all super-nodes is $|E_2|\leq n$. Over the course of the algorithm, some sets $C\in \cset$ may be split into smaller subsets. This will require to split the corresponding super-node $v_C$. The edges in set $E_1$ are called type-1 edges, and the edges in set $E_2$ are called type-2 edges.



The input to the vertex splitting operation consists of a single set $C\in \cset$, and a subset $C'\subseteq C$ containing at most $|C|/2$ vertices. The idea is that we replace $C$ by two subsets: $C'$ and $C''=C\setminus C'$, and update the graph accordingly: that is, we rename $v_C$ by $v_{C''}$; insert a new vertex $v_{C'}$, that connects to every vertex of $C'$ with an edge of weight $1/2$, and delete all edges connecting $v_{C''}$ to the vertices of $C'$. The input is given as follows: we are only given a pointer to the vertex $v_C$ corresponding to the set $C$; the names $C',C''$ of the new sets into which $C$ is split; and an explicit list of the vertices of $C'$. Note that it is possible that $C'$ becomes a singleton vertex, in which case the update operation does not create a new vertex $v_{C'}$, but instead simply deletes the edge $(v_C,u)$, where $u$ is the unique vertex of $C'$.

%Let $v_C\in V_2$ be a super-node, and let $N(v)$ be the set of its neighbors. A \emph{split pattern} consists of an integer $r>1$ (the arity of the split), and a partition $S_1,S_2,\ldots,S_r$ of $N(v)$ into $r$ non-empty subsets, where for all $1<i\leq r$, $|S_1|\geq |S_i|$. In the corresponding split operation, we modify the current graph $G$, so that $v$ is deleted; $r$ new vertices $v_1,\ldots,v_r$ are inserted (the new vertices are all super-nodes and may be split again later); and for each $1\leq i\leq r$, vertex $v_i$ connects to all vertices of $S_i$; for each $x\in S_i$, the weight of the new edge $(v_i,x)$ is $1/2$. We think of the edge $(x, v_i)$ as being an identical copy of edge $(x,v)$, so we do not view this as edge deletion/insertion. Let $\hat G'$ be the graph obtained from the current graph $\hat G$ after the split.

 Bernstein says that an algorithm that can handle edge insertions/deletions can also handle vertex splits. He does not provide details, but points to other papers. Below are my attempts to fill in the details without reading those other papers.

We will maintain an augmented graph $G'$. Graph $G'$ contains all vertices and edges of $\hat G$. Additionally, for every super-node $v_C\in V_2$, 
we have $\ceil{4|C|\log |C|}$ extra copies of $v_C$; we denote this set of extra copies by $X(v_C)$. Each such extra-copy connects to $v$ with an edge of length $1$. The latter set of edges is denoted by $E_3$, and we call all edges in this set \emph{type-3 edges}. Whenever we would like to split some super-node $v_C$ using a subset $C'\subseteq C$ of at most $|C|/2$ vertices, we implement the split by a number of edge insertion and edge deletion operations.

First, we pick an arbitrary vertex of $X(v)$, that we denote by $v_{C'}$, and we rename $v_C$ as $v_{C''}$. We do the following edge-insertion operations:

\begin{itemize}
\item For every vertex $x\in C'$, insert the edge $(v_{C'},x)$ of weight $1/2$;

\item Select an arbitrary subset $X(v_{C'})$ of $\ceil{4|C'|\log |C'|}$ distinct vertices of $X(v_{C})$; denote this set of vertices by $X(v_{C'})$. Connect $v_{C'}$ to each such vertex with an edge of weight $1$.
\end{itemize}

Note that these insertions do not decrease the distances between vertices, and we insert at most $|C'|+1\leq |C|/2+1$ new edges into the graph.

We then perform the following deletion operations:

\begin{itemize}
\item For all $x\in C'$, delete the edge $(x,v_{C''})$; 
\item For all $x\in X(v_{C''})\setminus (X(v_{C'}))$, delete the edge $(x,v_{C''})$; 
\item If $X(v_{C''})$ contains more than $\ceil{4|C''|\log |C''|}$ vertices, select an arbitrary subset of $\ceil{4|C''|\log |C''|}$ vertices of $X(v_{C''})$; for each remaining vertex $x$, we delete the edge $(v_{C''},x)$ from the graph, and we discard $x$ from $X(V_{C''})$; and
\item Delete the edge $(v_{C'},v_{C''})$.
\end{itemize}

The number of edge insertions in one vertex split operation is bounded by $|C'|+1$, but $|C'|\leq |C|/2$. Therefore, the total number of edges that can be inserted over the course of the algorithm due to vertex splitting is bounded by $O(n\log n)$. If $m'$ denotes the total number of edges inserted directly through edge-insertion operations, then the total running time is $\tilde O((m+m'+n\log n)D)$.

We will also need to combine vertex splitting with the algorithm of Lemma~\ref{lem: WSES}.  We will do this accounting later.

%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------
\fi

%--------------------------------------------------------
%--------------------------------------------------------
%--------------------------------------------------------



%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
\subsection{Proof of Theorem~\ref{thm: WSES}}

%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------
%---------------------------------------------------------

\mynote{It may be OK to delete this; it repeats Bernstein's paper except it shows all details, and mentions how we do shortest path queries which he didn't need.}

The lemma is proved by modifying the ES algorithm. Recall that the original ES algorithm stored, together with every vertex $v$, a value $\delta(v)$, which was the distance from $s$ to $v$. Now we will no longer ensure that $\delta(v)=d(s,v)$. Instead we ensure the following: between updates, the values $\delta(v)$ for $v\in V$ will have the following two properties:

\begin{properties}{I}
\item If $v=s$, then $\delta(v)=0$. Otherwise, if $p$ is the parent of $v$ in the current tree $T$, then $\delta(v)\geq \delta(p)+w(p,v)$; and \label{inv1: father}
\item For every neighbor $u$ of $v$, $\delta(v)\leq \delta(u)+(1+\eps)w(u,v)$. \label{inv1: neighbor}
\end{properties}

We first show that, if the above invariants are maintained, then we indeed maintain approximate shortest paths from $s$.

\begin{claim}\label{claim: approx}
Assume that the values $\delta(v)$ for $v\in T$ obey the above invariants. Then for each $v\in T$, $d(s,v)\leq \delta(v)\leq (1+\eps)d(s,v)$.
\end{claim}
\begin{proof}
To see that $\delta(v)\geq d(s,v)$, we simply follow the path in the tree $T$ from $v$ to $s$. From the first invariant, $\delta(v)$ is at least the sum of weights of edges along this path, which is at least $d(s,v)$. We now turn to prove that $\delta(v)\leq (1+\eps)d(s,v)$.

The proof is by induction on the number of edges in the shortest path from $s$ to $v$. If the shortest path contains just one edge $e$, then 
$\delta(v)\leq \delta(s)+(1+\eps)w(e)$. Assume now that the shortest $s$-$v$ path has $i>1$ edges, and let $u$ be the penultimate vertex on this path. Then $d(s,v)=d(s,u)+w(u,v)$. From the induction hypothesis, $\delta(u)\leq (1+\eps)d(s,u)$. From the second invariant, $\delta(v)\leq \delta(u)+(1+\eps)w(u,v)\leq (1+\eps)d(s,u)+(1+\eps)w(u,v)=(1+\eps)d(s,v)$.
\end{proof}



\begin{definition}
Let $e$ be an edge and let $x$ be an integer. $\round_e(x)$ is the smallest integer $y>x$ that is an integral multiple of $\eps w(e)$.
\end{definition}


Recall that in the ES-procedure, whenever $\delta(v)$ increases, we immediately update the copies of $v$ in the heaps $H_u$ of its neighbors to reflect this change. In the modified algorithm, every neighbor $u$ of $v$ will keep a copy $\delta_u(v)$ of the value $\delta(v)$, that is not necessarily up to date. We replace the invariants~\ref{inv1: father} and \ref{inv1: neighbor} with the following two approximation invariants, that hold for every vertex $v$:

\begin{properties}{A}
\item If $v=s$, then $\delta(v)=0$. Otherwise, let $u$ be the parent of $v$ in the tree. Then $\delta(v)=\delta_v(u)+w(u,v)$. (that is, we use the approximate local estimate on $\delta(u)$ in order to establish $\delta(v)$). Moreover, $u$ is the neighbor of $v$ with minimum $\delta_v(u)+w(u,v)$.
\label{inv2: approx father}


\item If $u$ is a neighbor of $v$, then $\delta(u)\leq \delta_v(u)\leq \round_{e=(u,v)}(\delta(u))$.\label{inv2: approx neighbor}
\end{properties}


Observe that, if Invariants~\ref{inv2: approx father} and \ref{inv2: approx neighbor} hold, then so do Invariants~\ref{inv1: father} and \ref{inv1: neighbor}. Indeed, Invariant~\ref{inv1: neighbor} follows immediately from Invariant~\ref{inv2: approx father}, and from the fact that $\delta_v(u)\geq \delta(u)$. For Invariant~\ref{inv1: neighbor}, denote $e=(u,v)$, and observe that:

\[\delta(v)\leq \delta_v(u)+w(e)\leq \round_e(\delta(u))+w(e)\leq \delta(u)+(1+\eps)w(e).\]

Therefore, it is now enough to maintain Invariants~\ref{inv2: approx father} and \ref{inv2: approx neighbor}.


In order to obtain the improved running time, we implement the following changes:

\begin{itemize}
\item Whenever $\delta(v)$ increases, we can inspect it, and charge the vertex for the inspection. However, we do not immediately inspect its neighbors. The number of such inspections is bounded by $nD$.

\item Let $e=(u,v)$ be an edge. We charge this edge (by inspecting both its endpoints) only if $\round_e(\delta(u))$ increases or $\round_e(\delta(v))$ increases. The number of such  charges to edge $e$ is bounded by $\frac{D}{\eps w(e)}$, and the total number of such inspections is bounded by $\sum_e\frac{D}{\eps w(e)}$.
\end{itemize}

We now describe an update operation, when an edge $(u,v)$ of the tree $T$ is deleted, where $u$ is the parent of $v$. As before, we maintain a heap $H$, to which we add all vertices that need to be inspected. We start with $H$ containing just the vertex $v$. In every iteration, we remove the vertex $x$ from the heap $H$ with smallest $\delta(x)$. We then consider, the vertex $y\in H_x$ with minimum $\delta_x(y)+w(x,y)$. If this value is no more than $\delta(x)$, then $y$ must be currently attached to the tree $T$, as we will see later. We attach $x$ to $y$.
Otherwise, we increase $\delta(x)$ by $1$. For every neighbor $z$ of $x$ for which $\round_{e=(x,z)}(\delta(x))$ increases, we update the value $\delta_z(x)$ of $x$ in the heap $H_z$ to be $\delta(x)$; if additionally $z$ is a child of $x$ in the tree $T$, then we add $z$ to the heap $H$.


Notice that throughout the algorithm, if a vertex $y$ of $T_v$ is not on the heap $H$ and is not attached to the tree $T$, then it has an ancestor $y'$ in $H$. From Invariants~\ref{inv2: approx father} and \ref{inv2: approx neighbor}, that ancestor has $\delta(y')<\delta(y)$. If $y$ is at the top of the heap $H_x$ and $\delta_x(y)+w(x,y)\leq \delta(x)$, then we know that $\delta(y)\leq \delta_x(y)<\delta(x)$, so $\delta(y')<\delta(x)$, and we should have processed $y'$ and not $x$. This concludes the correctness analysis.

Notice that when $\delta(x)$ increases, we need to be able to quickly figure out which edges incident to $x$ to process. This is implemented as follows. Each vertex $x$ has $m$ buckets. The $i$th bucket contains all edges $e$ incident to $x$, for which $\round_e(i)\neq \round_e(i+1)$. So whenever $\delta(x)$ decreases from $i+1$ to $i$, we need to inspect and charge all edges in the $i$th bucket. To initialize, each vertex creates $D$ buckets, which takes $O(nD)$ time. After that, each edge $e$ adds itself to the relevant buckets of its two endpoint: $D/\eps w(e)$ buckets per endpoint. So the total time to initialize the buckets is $O(nD)+O(\sum_e\frac{D}{\eps w(e)})$. Once the buckets are initialized, we don't need to do anything to maintain them, except inserting/deleting edges. 

One last part is edge insertion, which turns out to be tricky. Suppose we would like to insert an edge $e=(u,v)$, where $d(s,u)=1000$, $d(s,v)=1000$, and $w(e)=1$. This insertion does not decrease distances. But because we maintain approximate distances from $s$, we may have $\delta(u)=1000$ and $\delta(v)=1000(1+\eps)$. We need to insert a copy $\delta_v(u)$ of $u$ into the heap of $v$, and it is not clear how to do this while maintaining the invariants. In particular, we are not allowed to let $\delta(v)$ decrease, since this will ruin our analysis.

The solution is a bit weird. (Below is my implementation of the idea that was sketched in Bernstein's paper; he refers to other papers for more details; I did not read them).

 Assume that we insert an edge is $e=(u,v)$ and that $\delta(u)\leq \delta(v)$. We add a copy $\delta_u(v)=\delta(v)$ to $H_u$ as usual, and add $e$ to all the relevant buckets of $u$. All invariants continue to hold.
 If $\delta(u)+w(u,v)\geq \delta(v)$, then we also add a copy $\delta_v(u)=\delta(u)$ to $H_v$ as usual and add $e$ to all the relevant buckets of $v$. However, if $\delta(u)+w(u,v)< \delta(v)$, then we say that $(e,v)$ is a \emph{problematic pair}, and we set $\delta_v(u)=\delta(v)-(u,v)$. We will not update this value $\delta_v(u)$ until $\delta(u)$ becomes greater than $\delta_v(u)$, at which point $(e,v)$ will stop being a problematic pair, and we will add $e$ to the relevant buckets of $v$, and continue as usual. But notice that, while $(e,v)$ remains a problematic pair, $\delta(v)$ will not grow, as $v$ can always connect to the tree through $u$. The intuitive idea for why this work is that the original value $\delta(v)$ was a $(1+\eps)$-approximation on $d(s,v)$, and, as long as $\delta(u)\leq \delta(v)-w(u,v)$, we know that $d(s,v)\leq \delta(v)$. Since the distances never decrease, we maintain a $(1+\eps)$-approximation.

The problem is that this change completely messes up our invariants, and we need to redo them. 
Invariant \ref{inv2: approx father} continues to hold. Invariant \ref{inv2: approx neighbor} holds for  all pairs $(e,v)$ where $(e,v)$ is not a problematic pair. But if $(e,v)$ is a problematic pair, then we are only guaranteed that: 

\[\delta(u)\leq \delta_v(u).\]


We now define a new set of basic invariants that hold throughout the algorithm.


\begin{properties}{I}
\item If $v=s$, then $\delta(v)=0$. Otherwise, if $p$ is the parent of $v$ in the current tree $T$, then $\delta(v)\geq \delta(p)+w(p,v)$; \label{inv12: father}
\item Let $u$ be a neighbor of $v$, and let $e=(u,v)$  be the corresponding edge. If $(e,v)$ is not a problematic pair, then $\delta(v)\leq \delta(u)+(1+\eps)w(u,v)$. \label{inv12: neighbor}
\end{properties}



\begin{claim}\label{claim: approx}
Throughout the algorithm, for each $v\in T$, $d(s,v)\leq \delta(v)\leq (1+\eps)d(s,v)$.
\end{claim}
\begin{proof}
As before, to see that $\delta(v)\geq d(s,v)$, we simply follow the path in the tree $T$ from $v$ to $s$. From the first invariant, $\delta(v)$ is at least the sum of weights of edges along this path, which is at least $d(s,v)$. We now turn to prove that $\delta(v)\leq (1+\eps)d(s,v)$.

The proof is by induction on time and the number of edges in the shortest path from $s$ to $v$. 
When the algorithm starts, for every vertex $v$, $\delta(v)=d(s,v)$. We now consider the state of the algorithm after some iteration $j$, and consider the shortest $s-v$ path.
If this path contains no edges, then $\delta(s)=0$, and we are done.  Assume now that the shortest $s$-$v$ path has $i>0$ edges, and let $u$ be the penultimate vertex on this path. 
Then $d(s,v)=d(s,u)+w(u,v)$.
Let $e=(u,v)$ be the corresponding edge. Assume first that $(e,v)$ is not a problematic pair.
From the induction hypothesis, $\delta(u)\leq (1+\eps)d(s,u)$. From the second invariant, $\delta(v)\leq \delta(u)+(1+\eps)w(u,v)\leq (1+\eps)d(s,u)+(1+\eps)w(u,v)=(1+\eps)d(s,v)$.

Finally, assume that $(e,v)$ is a problematic pair. 
When $e=(u,v)$ is added to the graph, $ \delta(v)\leq (1+\eps)d(s,v)$ held, from the induction hypothesis. As long as $(e,v)$ remains a problematic pair, $\delta(v)$ does not grow, but $d(s,v)$ may increase. Therefore, $\delta(v)\leq (1+\eps)d(s,v)$ continues to hold. 
\end{proof}


\paragraph{Final Running Time Analysis}
Let $E_0$ be the set of edges that were present from the beginning, and $E_1$ the set of edges that were inserted over the course of the algorithm. Then the total running time of the algorithm is: $O(nD)+O(\sum_{e\in E_0\cup E_1}\frac{D}{\eps w(e)})$.




\newpage
%---------------------------------------------------
%---------------------------------------------------
%---------------------------------------------------
%---------------------------------------------------
\subsection{The Algorithm of Bernstein}
The following definitions are central to the algorithm. First, for every edge $e$, we let $\level(e)=\floor{\log w(e)}$ (in our case, all edges will have weights $2^i$ for integers $i$; the level of such an edge is $i$).

Given a vertex $v\in V(G)$, we denote by $I_i(v)$ the set of all edges of levels $1,2,\ldots,i$ that are incident to $v$, and by $I(v)$ the set of all edges incident to $v$.

Throughout, we assume that we are given some value $D$, and our goal is to approximately preserve the distances of all vertices from $s$, but only for those vertices $v$ with $D\leq d(s,v)\leq 2D$. (In our application, we are only interested in preserving the distance from $s$ to $t$, so we can assume that $D$ is the current estimate on this distance. Once the distance grows beyond $2D$, we can recompute the whole data structure from scratch). We use a threshold parameter \fbox{$\tau=\frac{3n\log n}{\eps D}$}.

For a vertex $v$, we let $\cutoff(v)$ be the largest integer $i$, such that $|I_i(v)|\geq \tau 2^i$. If no such index exists, we set  $\cutoff(v)=0$. Assume now that $\cutoff(v)=i$. We say that $v$ \emph{owns} all edges of $I_i(v)$, and all edges of $I_i(v)$ are called \emph{heavy} edges. Note that a heavy edge must be owned by at least one of its endpoints; but it can be owned by both endpoints.

Next, we define two graphs. The first graph, $G^H$ (called \emph{heavy graph}) contains all vertices of $G$ and all heavy edges of $G$. 
Let $\cset$ be the set of all connected components of $G^H$.
The second graph, $G^L$ (called \emph{light graph}) is defined as follows. The set of its vertices contains all vertices of $G$ -- we denote this set of vertices of $V_1$, and, for each $C\in \cset$, a \emph{super-node} $v_C$ -- we denote the set of all super-nodes by $V_2$. The set of edges also consists of two subsets. First, we add to $G^L$ all light edges of $G$, with their original weight; denote this set of edges by $E_1$. Notice that every edge of $E_1$ connects a pair of vertices of $V_1$. Next, for each connected component $C\in \cset$, we add an edge of weight $1/2$ between every vertex of $v$ and $v_C$ - we denote this set of edges by $E_2$.

\paragraph{Data Structures}
We maintain the graphs $G^H$ and $G^L$. Notice that, as the algorithm progresses, both graphs may change. For example, a heavy edge may become light, and we may need to delete it from $G^H$ and insert it into $G^L$. Also, a connected component of $G^H$ may get split, and we may need to split the corresponding super-node of $G^L$. Notice that we will only split the vertices of $V_2$, and we will only insert edges connecting pairs of vertices in $V_1$. These insertions do not decrease distances: suppose an edge $e=(u,v)$ stopped being heavy, and needs to be inserted into $G^L$. Before the insertion, $u$ and $v$ belong to the same connected component $C$ of $\cset$. So graph $G^L$ contains edges $(u,v_C)$, $(v,v_C)$ of weight $1/2$ each, and so currently, $d(u,v)\leq 1$. The insertion of the edge $(u,v)$, whose weight is at least $1$ will not decrease the distances.

For graph $G^H$, we use an algorithm that maintains all connected components of $H$ with update time $O(\log^2n)$ per edge deletion. This part takes $O(m\log^2n)$ total time. Once an edge $e=(u,v)$ of $G^H$ is deleted, we inspect its two endpoints, and, if any edge incident to $u$ or $v$ stops being heavy, we also delete that edge and add it to $G^L$. (If an edge $e'=(u,w)$ stops being heavy, this means that $w$ does not own $e'$, and $e'$ does not contribute to its set $I_i(w)$, where $i=\cutoff(w)$, so we don't need to inspect edges incident to $w$ and this deletion will not propagate). Next, we update all connected components of $G^H$ using the algorithm for maintaining the connected components. Figuring out which edges of $u$ and $v$ stop being heavy can be implemented by having buckets of level-$i$ edges incident to each vertex $x$, for each $i<\cutoff(x)$.

For graph $G^L$, we use the data structure from Lemma~\ref{lem: WSES}. In order to use it, we need to bound the number of edges of different levels that ever belong to $G^L$. Fix some level $1\leq i\leq \log n$, and consider a vertex $v\in V$. If, at the beginning of the algorithm, $\cutoff(v)<i$, then there are at most $2^i\tau$ vertices of level $i$ incident to $v$. Otherwise, if $\cutoff(v)\geq i$, then a level-$i$ edge incident to $v$ may only be added to $G^L$ when $\cutoff(v)$ decreases to be lower than $i$. At this moment, at most $2^i\tau$ edges of level $i$ are incident to $v$. Therefore, in total, over the course of the algorithm, the number of level-$i$ edges that ever belong to $G$ is bounded by $2^i\tau n$.

We also need to take care of vertex splitting. Recall that we construct an auxiliary graph $G'$, that contains the graph $G^L$, and additionally, for every super-node $v_C\in V_2$, we insert $|C|\log |C|$ extra-vertices, whose set we denote by $X(v_C)$. Therefore, $|V_2|\leq n\log n$. Over the course of the algorithm, every edge incident to a super-node $v_C$ may pay for up to $\log n$ edge insertions. So the total number of these extra edge insertions is bounded by $n\log n$. Therefore, the total number of edges of weight $1/2$ that are ever present in the graph is bounded by $O(n\log n)$. 

From Lemma~\ref{lem: WSES}, the total update time is $O(nD\log n)+O(\sum_e\frac{D}{\eps w(e)})$. For the second summand, for each $i\geq 1$, we will have at most $2^i\tau n\leq 2^in^2\log n/D$ edges of level $i$ ever present in the graph, so the corresponding summand for each $i$ becomes at most $O(\frac{n^2\log n}{\eps})$. Additionally, at most $O(n\log n)$ edges of weight $1/2$ will be present. So the total running time becomes $O(nD\log n)+O(\frac{n^2\log^2n}{\eps})=O(\frac{n^2\log^2n}{\eps})$.

Finally, we show that, throughout the algorithm, for every vertex $v\in V$ with $D\leq d(s,v)\leq 2D$, the algorithm maintains a $(1+\eps)$-approximation of $d(s,v)$. For that, it is enough to show that the distance from $s$ to $v$ in the graph $G^L$ is a $(1+\eps)$-approximation of $d(s,v)$. Let $P$ be the shortest path connecting $s$ to $v$ in $G^L$. We can assume that it is a simple path, so a super-node $v_C$ may appear on $P$ at most once. Let $D'$ denote the length of the path $P$. Notice that $D'\leq (1+\eps)d(s,v)$: let $P^*$ be the shortest $s$-$v$ path in $G$. We short-cut the path by contracting all clusters on it. This gives a path in $G^L$, whose length is at most $d(s,v)$. Since we maintain $(1+\eps)$-approximate shortest path in $G^L$, we are guaranteed that $D'\leq (1+\eps)d(s,v)$.

We now show that $d(s,v)\leq D'+\eps D$.  Let $v_{C_1},\ldots,v_{C_r}$ be all super-nodes that appear on the path $P$. For $1\leq j\leq r$, let $v_j$ be the regular vertex preceding $v_{C_j}$ on $P$, and let $u_j$ be the regular vertex following $v_{C_j}$ on $P$. Denote $n_j=|C_j|$. For each $1\leq j\leq r$, let $Q_j$ be the shortest $v_j-u_j$ path in graph $C_j$.

\begin{claim}\label{claim: length of path in heavy graph}
For all $1\leq i\leq \log n$ and $1\leq j\leq r$, the number of level-$i$ edges on $Q_j$ is at most $3n_j/(2^i\tau)$.
\end{claim}
\begin{proof}
Fix some $1\leq i\leq \log n$ and $1\leq j\leq r$, and let $e_1,\ldots,e_z$ be all level-$i$ edges on $Q_j$. Let $E'=\set{e_x\mid 1\leq x\leq z, x=1\mod 3}$. For each edge $e\in E'$, let $v(e)$ be an endpoint of $e$ that owns $e$ (that is, $\cutoff(v(e))\geq i$). Then $v(e)$ has at least $2^i\tau$ neighbors in graph $G^H$. Moreover, if $e,e'\in E'$ and $e\neq e'$, then the set of neighbors of $v(e)$ and the set of neighbors of $v(e')$ in graph $G^H$ are disjoint (otherwise we could have shortened the path $Q_j$). Therefore, $|E'|\leq \frac{n_j}{2^i\tau}$, and the total number of level-$i$ edges on $Q_j$ is at most $3n_j/(2^i\tau)$.
\end{proof}

Let $P^*$ be obtained from path $P$ by replacing the super-nodes $v_{C_j}$ with the corresponding paths $Q_j$.
We conclude that for each $1\leq i\leq \log n$, the total number of level-$i$ edges on $Q_1\cup\cdot\cup Q_r$ is at most $3n/(2^i\tau)$. Therefore, the total length of the paths $Q_1,\ldots,Q_r$ is at most $\frac{3n\log n}{\tau}\leq \frac{3n\eps D\log n}{3 n\log n}\leq \eps D$.

The total length of $P^*$ is then at most $D'+\eps D$, and so $d(s,v)\leq D'+\eps D$.

This concludes the exposition of Bernstein's algorithm. The main drawback of this algorithm is that it does not allow us to compute the shortest $s$-$t$ path (or an $s$-$v$ path). The reason is that we do not maintain shortest path trees in the connected components of the graph $G^H$. So we are only guaranteed that paths $Q_1,\ldots,Q_r$ of total length at most $\eps D$ exist, but we do not know how to find them. 





\newpage

\section{Current Plan for an Algorithm}
\iffalse
This describes an algorithm for a single layer, where we allow vertex deletions.
We will define the layers slightly differently from Bernstein.
The layers are defined from top to bottom (highest to lowers degree). At the beginning, we start with $G$, and iteratively delete from it every vertex that has degree less than $n/2$, together with all its edges. In the graph that's left, every vertex has degree between $n/2$ and $n$, and in the deleted graph the total number of edges is at most $n^2/2$. We then continue like that. Let $G'$ be the current residual graph (excluding the  edges that belong to higher levels), and assume that we are building a level corresponding to degree roughly $h$. We will guarantee that the number of edges in $G'$ is at most $2hn$. We iteratively delete from $G'$ every vertex whose degree is less than $h$. The remainder becomes the graph of the current layer; it has at most $2hn$ edges, and all vertices in it have degree at least $h$. We denote by $G''$ the graph obtained by taking the deleted vertices in edges; this graph has at most $hn$ edges. We keep on doing this, until we reach the layer corresponding to the "light" graph. (but here it's not just the degrees that play a role, but also levels of edges, so this should be defined more carefully). (also, it looks like a vertex may be downgraded many times and may belong to several layers, so this may not work)
\fi

We focus on a single layer, where we assume that average vertex degree is $h$, and the total number of edges is $O(hn)$ . 


 The algorithm is partitioned into phases, and we work with each connected component $C$ of the current layer individually. A phase ends with respect to $C$ when we have either deleted $h/\poly\log n$ vertices from $C$; or we split $C$ into pieces, each of which has fewer than $|C|-h/\poly\log n$ vertices. When a phase ends, we can afford to spend $O(|E(C)|)=O(|C|h)$ time on reorganizing things.
 
 We temporarily remove from $C$ vertices that have degree less than $h/10$ (iteratively); we will add them back later. (Notice that this may break $C$ into pieces).
 
 At the beginning of the phase, we partition the cluster $C$ into vertex-expanders, as follows. Start with $\cset=\set{C}$, then iterate. For each cluster $S\in \cset$, if there is a vertex cut $(A,X,B)$ of $S$ of sparsity less than $1/\log^4n$, replace $S$ with two cluster: $A\cup X$ and $X\cup B$. The vertices of $X$ become boundary vertices. The vertices that remain non-boundary vertices until the end are called inner vertices. At the end, at most $|C|/\log^3n$ vertices will be boundary vertices; denote them by $B$. A cluster is called good if it has at least one inner vertex. In such a case, it has at least $h$ vertices overall. To do the decomposition, in one round we try to cut every cluster currently in $\sset$. Finding such a cut in $S\in \sset$ takes time $\tilde O(|E(S)|)$ \mynote{Can we do it in time $O(m)$ using algorithm like Raecke's?}
 
 
 We keep the good clusters, and then keep repeating this process, as follows. Take the set $B$ of boundary vertices, and let $H$ be the sub-graph of the current layer induced by them. Iteratively delete from $H$ vertices whose degrees in $H$ are less than $h/\log^3n$. Do the decomposition again in the remaining graph $H$, and repeat from scratch. Overall, we'll do $O(log n)$ such decompositions. The final set $B$ will have the property that, after we iteratively delete all vertices of degree less than $h/\log^3n$ in $H$, $B$ becomes empty. From here, it is easy to see that every vertex of $B$ can reach one of the good clusters in $\log n$ steps. This remains true even if we delete up to $h/\log^5n$ vertices from the graph. (intuitively, the first vertex of $B$ that we remove has $h(1-1/\log^3n)$ edges connecting it to good clusters, but only $h/\log^3n$ edges that can be used for future vertices that are deleted from $B$. We can build BFS layers starting from the good clusters: when a vertex from $B$ is deleted from $H$, it has at least $h(1-1/\log^3n)$ edges connecting it to the vertices that are currently in the BFS. We put it in a layer, such that it has at least $h/\log n$ edges connecting it to the previous layer. If no such layer, put it aside. The key is that the number of vertices in layer $i$ will be at most the number of vertices in layer $(i-1)$ divided by $\log^2n$. So we will never have more than $\log n$ layers.
 
 Now we will keep the following data structures:
 
 \begin{itemize}
 \item Connectivity (spanning tree) of the cluster $C$.
 
 \item Single-source shortest path, whose root is a new vertex $s$, that connects to every good cluster with an edge. (For a good cluster, we contract all its inner vertices). Note that every vertex of $B$ will have a path of length at most $\log n$ to the source. Together with each such vertex $v$, we store the name of the good cluster it currently connects to (in whose sub-tree it lies).
 \end{itemize}
 
 We will later show that inside each good cluster, we can find a path of length $\poly\log n$ between every pair of its inner vertices, even if up to $h/\poly\log n$ vertices are deleted. 
 
 
 Now suppose we want to find some path between a  pair $u,v$ of vertices. Using the connectivity structure, we find some initial path $P=(v_1,v_2,\ldots,v_r)$, which is a simple path. Then we replace each $v_i$ with the name of the good cluster $S(v_i)$ to which it connects. Whenever some good cluster appears twice, we delete the part of $P$ between the two appearances. So in the end, every good cluster will appear at most once on this path. The number of the good clusters is at most $n/h$, so now the path is short.  Then using the paths connecting the corresponding vertices of $B$ to the good clusters, we build a path from $u$ to $v$, of length at most $|C|\poly\log n/h$, that contains good clusters. The last step is routing between pairs of inner vertices of good clusters. Note that a boundary vertex (or even an inner vertex of a cluster) may serve as a boundary vertex of another cluster, so the resulting path may not be simple. But we can simplify it as before.
 
 Finally, the routing in the good clusters is done as before. We claim that, as long as fewer than $d/\poly\log n$ vertices are deleted from $C$, for every pair $u,v$ of {\bf inner} vertices of $C'$, there is a path of length at most $\poly\log n$ connecting them in $C'$.
Indeed, each of $u,v$ had at least $d/4$ neighbors inside $C'$, most of which survived. Let $S$ be the set of surviving neighbors of $u$, and $T$ the set of surviving neighbors of $v$. Set $S$ has at least $|S|/\log^4 n>d/\log^4n$ neighbors in $C'$ due to the expansion properties of the core, and most of them have survived. Add them to $S$. We keep going like that from both sides until they merge. So within each phase of the algorithm, we can route through the core via paths of length at most $\log^5n$. The question is how to find such paths.

Here is a trick to do it. Before the phase starts, we build an expander $H$ on $|C'|$ vertices and embed it into $C'$ via the cut-matching game, so that every edge $e$ of $H$ is mapped to a path $P(e)$ in $C'$; the length of the path is at most $\poly\log n$; and every vertex of $H$ participates in at most $\poly\log n$ such paths. WeÕll need to use the entropy-based algorithm with Raecke to do this, because weÕll only be able to route a constant fraction of the flow in each iteration, especially if we require short paths. If that part works out, we should be able to do it in $O(|E(C')|\poly\log n)$ time. Every vertex $v$ of $C'$ will keep a pointer to every edge $e$ of $H$, such that $v \in P(e)$.

When we delete a vertex $v$ from $C$, we delete all edges $e$ with $v\in P(e)$ from $H$. So as long as we delete fewer than $d/\poly \log n$ vertices from $C$, we delete at most $d/\poly\log n$ edges from H. Assume now that we are given two inner vertices $u$ and $v$ of $C'$, and we would like to connect them by a path. As before, $u$ had at least $d/4$ neighbors in $C'$, most of which are still alive; call this set $S$. Similarly, $v$ had at least $d/4$ neighbors in $C'$, most of which are still alive; call this set $T$. We now know that the expander $H$ contains a path of length $\poly\log n$, connecting $S$ to $T$, for the same reason as before: there are $|S|/\poly\log n$ edges in $H$ leaving $S$, most of which are still alive, and so on. We can spend $O(|E(H)|)$ time finding this path. This gives $O(|C'|\poly\log n)$ time per query to the core, which will result in $O(n \poly\log n)$ total time per query.
 
 
 We also need to add back the low-degree vertices we have removed and make sure the algorithm works with them. 


\newpage

\subsection{Extending Bernstein's Algorithm}
In this section we extend Bernstein's data structure, so that it can report the (approximate) shortest-paths from the source $s$, and not only their lengths. Our goal is to maintain a data structure, that, given a graph $G$ subject to edge deletions, and a source vertex $s$, can answer shortest-path queries: given a query vertex $v$, it must return a path from $s$ to $v$ of length at most $(1+\eps)d(s,v)$, in time $\tilde O(n)$. The total update time of the data structure is $O(n^2\poly\log n\log W/\eps)$, where $W$ is the largest edge weight.

As before, we use a parameter $D$, which is our estimate on the shortest-path distances: that is, our data structure will report approximate shortest paths correctly for all vertices $v$ with $D\leq d(s,v)\leq 2D$. 
Specifically, for a query vertex $v$, if $d(s,v)>2D$, then the data structure may not be able to return any $s$-$v$ path. Otherwise, if $d(s,v)\leq 2D$, the data structure is guaranteed to report some $s$-$v$ path. For every vertex $v$ for which the data structure reports an $s$-$v$ path, the path length is guaranteed to be at most $(1+\eps)d(s,v)+\eps D$. Therefore, for every vertex $v$ with $D\leq d(s,v)\leq 2D$, the algorithm is guaranteed to return a path of length at most $(1+2\eps)d(s,v)$. For a vertex $v$ with $d(s,v)<D$, the algorithm will return a valid $s$-$v$ path, that may be too long; and for a vertex $v$ with $d(s,v)>2D$ the algorithm may be unable to return any $s$-$v$ path. We keep a separate data structure for every value of $D$ that is an integral power of $2$ between $1$ and $nW$. Given a query vertex $v$, we run the query in each of these data structures, and return the shortest path that is returned by any of these data structures. From now on, we fix one value of $D$, $1\leq D\leq nW$, and describe a data structure for this value of $D$.

%We run separate algorithms for different scales of $D$ (for our specific application, we would need to use one value of $D$ at a time -- the current approximate length of the $s$-$t$ path). From now on, we assume that the value $D$ is fixed, and that we are only interested in vertices whose distances from $s$ are between $D$ and $4D$. 

We slightly modify the main parameter of Bernstein's algorithm, and set \fbox{$\tau=\frac{32n\log n}{\eps D}$}. The main definitions remain the same as before; we recap and extend them here.

\begin{itemize}
\item  For every edge $e$, we let $\class(e)=\floor{\log w(e)}$.

\item Given a vertex $v\in V(G)$, we denote by $I_i(v)$ the set of all edges of classes $1,2,\ldots,i$ that are incident to $v$, and by $I(v)$ the set of all edges incident to $v$.

\item For a vertex $v$, we let $\cutoff(v)$ be the largest integer $i$, such that $|I_i(v)|\geq \tau 2^i$. If no such index exists, we set  $\cutoff(v)=0$. Assume now that $\cutoff(v)=i>0$. We say that $v$ \emph{owns} all edges of $I_i(v)$, and all edges of $I_i(v)$ are called \emph{heavy} edges. Note that a heavy edge must be owned by at least one of its endpoints; but it may be owned by both endpoints.

\item For a vertex $v$, we define its \emph{effective degree} $\Delta(v)$ to be the number of edges that $v$ owns. In other words, if $\cutoff(v)=i$, then $\Delta(v)=|I_i(v)|$.

\item The two graphs $G^H$ and $G^L$ are defined exactly as before. We now only focus on the heavy graph $G^H$. Recall that its set of vertices is $V(G)$, and its set of edges consists of all heavy edges of $G$.
\end{itemize}


From Bernstein's algorithm, it is sufficient to design a data structure that can answer the following queries:

\begin{quote}
{\bf Query $(u,u')$:} \emph{Given two vertices $u,u'$ that belong to the same connected component $C$ of $G^H$,  return, in time $O(|C|\poly\log n)$, a path $Q\subseteq C$ connecting $u$ to $u'$, such that for each $1\leq i\leq \log n$, path $Q$ contains at most \fbox{$\frac{24|C|\log n}{2^i\tau}$} edges of class $i$.}
\end{quote}

(we note that such a path must exist from the analysis of Bernstein's algorithm).
Notice that the total length of the path $Q$ is at most $24|C|\log n/\tau$. 
We now show that being able to handle such queries is sufficient.

Recall that in the algorithm of Bernstein, we are given a query vertex $x\in V(G)$. Let $d'(s,x)$ be the distance from $s$ to $x$ in graph $G^L$, so $d'(s,x)\leq d(s,x)$. If $d'(s,x)>2D$, then we ignore this query and do not return a path (in this case, $x$ may not be included in the data structure). Assume now that $d'(s,x)\leq 2D$. Then the algorithm of Bernsten can be used to compute a simple path $P$, connecting $s$ to $x$ in $G^L$, whose length is at most $d'(s,x)(1+\eps)$ -- this is simply the path connecting $s$ to $x$ in the approximate \EST that he maintains. 
Let $v_{C_1},\ldots,v_{C_r}$ be the super-nodes lying on this path. For each such super-node $v_{C_j}$, let $u_j,u'_j$ be the regular vertices lying immediately before and immediately after $v_{C_j}$ on $P$, so $u_j,u'_j\in C_j$. Let $Q_j$ be the path connecting $u_j$ to $u'_j$ in $C_j$, that our algorithm returns, so the length of $Q_j$ is at most $24|C_j|\log n/\tau$. Let $P^*$ be the final path obtained from $P$, by replacing each super-node $v_{C_j}$ with the corresponding path $Q_j$. Then the length of $P^*$ is at most:

\[\begin{split} 
\ell(P)+\sum_j\frac{24|C_j|\log n}{\tau}&\leq (1+\eps)d'(s,x)+\frac{24n\log n}{\tau}
\\&\leq (1+\eps)d'(s,x)+\eps D\\
&\leq (1+\eps)d(s,x)+\eps D.\end{split}\]

Notice that, if $d(s,x)\leq 2D$, then $\ell(P^*)\leq (1+2\eps)d(s,x)$ as required. Let $\cset$ denote the set of all connected components of $G^H$. The total time that the algorithm spends to respond to the query $x$ in the data structure for this fixed value of $D$ is at most $O(n)+\sum_{C\in \cset}|C|\poly\log n=O(n\poly\log n)$, and the total query time is $O(n\poly\log n\log W)$.


We use two main tools. The first tool is the ES-trees. Given a connected graph $\hat G$, a designated source vertex $s(\hat G)$, and a length bound $ D(\hat G)$, we denote by $\EST(\hat G,s(\hat G), D(\hat G))$  the ES-tree data structure of $\hat G$ with respect to the source $s(\hat G)$, with the distance restriction $D(\hat G)$. We denote by $\ESIN(\hat G,e)$ and by $\ESDEL(\hat G,e')$ the procedures for inserting edge $e$ into the data structure $\EST(\hat G,s(\hat G), D(\hat G))$, and the procedure for deleting edge $e'$ from the data structure $\EST(\hat G,s(\hat G), D(\hat G))$, respectively. Both procedures include the necessary updates of the data structure.

In addition to ES-trees, we also need a data structure for connectivity. We will use the results of~\cite{dynamic-connectivity}, that provide a data structure, that we denote by $\CONN(\hat G)$, that, given an $n$-vertex graph $\hat G$ subject to edge deletions and edge insertions, responds to each connectivity query in $O(\log n/\log\log n)$ time, and has amortized running time of $O(\log^2n)$ per edge deletion or insertion. The data structure and the algorithm are deterministic.  In a connectivity query, we are given a pair $u,v$ of vertices of $\hat G$, and need to determine whether they are connected in $G$.
We denote by $\CONNIN(\hat G,e)$ and by $\CONNDEL(\hat G,e')$ the procedures for inserting an edge $e$ into and deleting an edge $e'$ from the data structure, respectively. We also denote by $\conn(\hat G,u,u')$ the connectivity query between $u$ and $u'$ in the data structure.


Before we define our data structure, we need a few additional definitions.
 For $1\leq j\leq \log n$, let $L_j$ contain the set of all vertices  $v$ of $G$ whose effective degree is: $2^j\leq \Delta(v)<2^{j+1}$.  We refer to vertices of $L_j$ as \emph{level-$j$ vertices}. For a vertex $v\in L_j$, we denote $\level(v)=j$.
 We let $1\leq\rho\leq\log n$ be the largest integer, for which $L_{\rho}\neq \emptyset$.
 We now define graphs $G_1,\ldots,G_{\rho}$ inductively, starting from graph $G_{\rho}$. For each graph $G_j$, we will also define an extended graph $G'_j$, that will allow us to handle super-node splitting. 
We then let $\cset_j$ be the set of all connected components of graph $G'_j$ that are not isolated vertices, and for each such component $C\in \cset_j$, we let $R(C)$ denote the set of all {\bf regular} vertices of $C$.

In order to define the graph $G_{\rho}$, we let the set of its vertices be $V(G)$. For every vertex $v\in L_{\log n}$, we add all edges that $v$ owns in $G_{\rho}$. The weight of each such edge is set to $1$, and they are called type-1 edges. The extended graph $G'_{\rho}=G_{\rho}$.

We now define graph $G_j$, for some integer $1\leq j<\rho$, assuming that graphs $G_{j+1}$ and $G'_{j+1}$ were defined. Recall that $\cset_{j+1}$ is the set of all connected components of graph $G'_{j+1}$ that are not isolated vertices, and for each such component $C\in \cset_{j+1}$, $R(C)$ is the set of all regular vertices lying in $C$. The set of vertices of $G_j$ consists of two subsets: set $V_1^j=V(G)$ of regular vertices, and set $V_2^j=\set{v_C\mid C\in \cset_{j+1}}$ of super-nodes. The set of edges consists of two subsets: set $E_1^j$ of type-$1$ edges contains, for every vertex $v\in L_j$, all edges owned by $v$. All edges of $E_1^j$ have weight $1$. Set $E_2$ of type-$2$ edges is defined as follows. For every component $C\in \cset_{j+1}$, for every regular vertex $u\in R(C)$, we add an edge $(u,v_C)$ of weight $1/2$ to $E_2$. (Note that $C$ may contain super-nodes $v_{C'}$, where $C'$ is a connected component of $G'_{j+2}$, and $v_{C'}$ does not belong to $G_j$; we only add edges connecting $v_C$ to regular vertices).

In order to define the extended graph $G'_j$, we start with $G'_j=G_j$. For every super-node $v_C\in V_2^j$, we add a set $X(v_C)$ of $\ceil{4|C|\log |C|}$ \emph{extra-vertices}, that all connect to $v_C$ with an edge of weight $1$ -- these edges are called type-3 edges. We say that super-node $v_C$ \emph{owns} all vertices of $X(v_C)$. Let $V_3^j$ denote the set of all extra-vertices of $G'_j$, and let $E_3^j$ be the set of all edges incident to them. Note that each extra-vertex has degree exactly $1$. 

As the algorithm progresses, the underlying graph $G$ changes, and the graphs $G_j$ and $G'_j$ evolve. When we refer to graph $G_j$ or $G'_j$, we refer to these graphs defined with respect to the current graph $G$. Similarly, for a vertex $x\in V(G)$, the values of $\cutoff(x)$, $\Delta(x)$, $\level(x)$ evolve as the algorithm progresses.
  Recall that $\cset_j$ is the set of all connected components of $G'_j$ that are not isolated vertices, and for each component $C\in \cset_j$, $R(C)$ is the set of all regular vertices of $C$. We then have the following simple observation and its corollary

\begin{observation}\label{obs: containment of CC's}
Let $1<j\leq \rho$ be an index, and let $C\in \cset_j$ be a non-singleton connected component of $G'_j$. Then there is some connected component $C'\in \cset_{j+1}$, such that $R(C)\subseteq C'$.
\end{observation}

\begin{corollary}\label{cor: containment of CC's}
For all $1\leq j'<j\leq \rho$, for every component $C\in \cset_j$, there is a component $C'\in \cset_{j'}$, such that $R(C)\subseteq C'$.
\end{corollary}


\subsubsection{Data Structures}
We now describe the data structures that we maintain.

\begin{itemize}
\item For each $1\leq j\leq \rho$, we maintain a list $\lset_j$ of all connected components of $G_j'$ that are not isolated vertices, so $\lset_j$ contains a list of all components of $\cset_j$. Every vertex of $G_j'$ that is not an isolated vertex, has a pointer to the connected component in $\lset_j$ to which it belongs. Additionally, for every component $C\in \lset_j$, there are bi-directional pointers between $C$ and the corresponding super-node $v_C$ in $G'_{j-1}$.

\item For every vertex $v\in V(G)$, we maintain a pointer from $v$ to its copies in each graph $G_j'$.

\item For each edge $e$, we maintain the information of which endpoints of $e$ own it, and pointers from its owners to $e$ and back. We also maintain pointers to the graphs $G'_j$ to which $e$ belongs (either one or two of them, depending on whether one or both endpoints of $e$ own it, and whether both endpoints belong to the same class), and to the corresponding copies of its endpoints.

\item For every regular vertex $v$, we maintain a list of all edges it owns, sorted into buckets, where bucket $B_i(v)$ contains all edges of class $i$ that $v$ owns. We also maintain the effective degree of $v$, $\Delta(v)$, and $\level(v)$.

\item For each $1\leq j\leq \log n$, we maintain the connectivity data structure $\CONN(G'_j)$.

\item For each $1\leq j\leq \log n$, for every connected component $C\in \cset'_j$, we select some vertex $s(C)$ to be a source, and we let $D(C)=12|C|/2^j$ be the distance bound for $C$. We later show that, as long as $C$ remains connected, the depth of the shortest-path tree from $s(C)$ is always at most $D(C)$. Finally, we maintain the data structure $\EST(C,s(C),D(C))$ for all $C\in \cset'_j$.
\end{itemize}





\begin{observation}\label{obs: size of cc's}
Throughout the algorithm, for all $1\leq j\leq \rho$, every connected component $C\in\cset_j$ contains at least $2^j$  regular vertices.
\end{observation}
\begin{proof}
The proof is by induction on $j$, starting from $j=\rho$. Graph $G'_{\rho}$ contains no super-nodes. If $C\in \cset_{\rho}$ is a connected component that is an isolated vertex, then it contains at least one edge. Since $G'_{\rho}$ has no super-nodes, every edge of $G'_{\rho}$ is a type-1 edge, that is, it is an edge of $G$ that is owned by some vertex $v\in L_{\rho}$. Let $e$ be any such edge that lies in $C$, and let $v\in L_{\rho}$ be the endpoint that owns it. Then $v\in L_{\rho}$, $\Delta(v)\geq 2^{\rho}$, and so $C$ contains at least $2^{\rho}$ vertices of $V(G)$.

We now assume that the claim is true for some $1<j\leq \rho$, and prove it for $j-1$. Let $C\in \cset_{j-1}$ be a connected component of $G'_{j-1}$, that is not an isolated vertex. Then some edge $e$ belongs to $C$. If one of the endpoints of $e$ is a super-node $v_{C'}$, for some $C'\in \cset_j$, then, from the induction hypothesis, $C'$ contains at least $2^{j}$ vertices of $V(G)$. Each such vertex connects to $v_{C'}$ with an edge in $G'_{j-1}$, and so $C$ contains at least $2^j$ regular vertices. Therefore, we assume that both endpoints of $e$ are regular vertices. Denote $e=(x,y)$. Since $e\in G_j'$ and its endpoints are regular vertices, $e\in E(G)$, and at least one of its endpoints (say $x$) owns it and belongs to $L_j$. Then the effective degree of $x$ is at least $2^j$, and all edges that $x$ owns belong to $C$. Therefore, $C$ contains at least $2^j$ regular vertices -- the endpoints of these edges.
\end{proof}

\begin{corollary}\label{cor: depth of tree bound}
Throughout the algorithm, for all $1\leq j\leq \log n$, for every connected component $C\in \cset_j$, for every vertex $x\in C$, the distance from $x$ to the source vertex $s(C)$ in $G'_j$ is at most $12|C|/2^j$.
\end{corollary}

\begin{proof}
Fix some $1\leq j\leq \log n$.
Recall that for every edge $e\in G'_j$, one of12dpoints of $e$ is either a super-node, or a vertex of $L_j$. In either case, the degree of this vertex in $G'_j$ is at least $2^j$. Consider now some connected component $C\in \cset_j$ and some vertex $x\in V(C)$. Let $P$ be the shortest path from $x$ to $s(C)$, and let $U\subseteq V(P)$ contain all super-nodes and all vertices of $L_j$ on this path. Then the length of the path $P$ is at most $2|U|$. Let $U'$ be obtained from $U$ by taking one vertex out of every $6$ consecutive vertices, so that $|U'|\geq |U|/6$. Then for every pair $v,v'\in U$ of vertices, $N_C(v)\cap N_C(v')=\emptyset$ (or we could shortcut the path $P$; notice that some edges have length $1/2$, and some edges have length $1$, which is why we take one vertex in $6$). Therefore, $|U'|\leq |C|/2^j$, and $\ell(P)\leq 12|C|/2^j$.
\end{proof}



Next, we describe how path queries are answered, and then how the data structure is updated.

\subsubsection{Path Queries}
Let $C$ be a connected component of $G^H$, and let $u,u'$ be any two vertices of $C$. 
We next describe an algorithm that answers the query $(u,u')$. Recall that the algorithm must return, in time $O(|C|\poly\log n)$, a path $Q\subseteq C$ connecting $u$ to $u'$, such that for each $1\leq i\leq \log n$, path $Q$ contains at most \fbox{$\frac{24|C|\log n}{2^i\tau}$} edges of class $i$.

Notice that $u,u'$ must lie in the same connected component of $G_1'$, that we denote by $C^*$. Let $s^*$ be the source vertex that we have selected for $C^*$. Consider the shortest-path tree $T(C^*)$ from $s^*$, that is maintained by the data structure $\EST(C^*,s(C^*),D(C^*))$. Let $x$ be the lowest common ancestor of $u$ and $u'$ in the tree, and let $P_1$ be the path obtained by concatenating the path from $u$ to $x$ and the path from $u'$ to $x$ in the tree $T(C^*)$. In order to compute $P_1$, we let $P$ be the path from $u$ to $s^*$, and $P'$ we let $P'$ be defined similarly for $u'$. We then traverse both paths in the reversed order, in order to identify the vertex $x$, and truncate them suitably.
 Note that $P_1$ does not contain any extra-vertices, since all extra-vertices have degree $1$, but it may contain super-nodes. We call $P_1$ a \emph{level-1 path}. Let $v_{C_1},\ldots,v_{C_r}$ be the super-nodes appearing on this path. For each $1\leq k\leq r$, let $u_k$ and $u'_k$ be the regular vertices appearing immediately before and immediately after $v_{C_k}$ on $P_1$. We then recursively find, for each $1\leq k\leq r$, a simple level-$2$ path $P^2_k$, connecting $u_k$ to $u'_k$ in $C_k$, by exploiting the paths connecting these two vertices to the source $s(C_k)$ in the tree $T(C_k)$ stored in the data structure $\EST(C_k,s(C_k),D(C_k))$ (as before, we truncate the two paths to the lowest common ancestor of $u_k$ and $u'_k$, so that $P^2_k$ is a simple path). We continue this process recursively, until we obtain a final path $P^*$, that only contains regular vertices. Notice that over the course of this process, for each $1\leq j\leq \rho$, we have computed a set $\pset_j$ of level-$j$ paths, that we denote by $\pset_j=\set{P_1^j,\ldots,P_{r_j}^j}$. Each such path $P_k^j$ lies in a distinct connected component $C^j_k$ of $\cset_j$ (because paths from previous levels were simple, and so each super-node could appear at most once, on at most one such path), and it was obtained by concatenating two paths of the ES-tree $T(C^j_k)$: a path from some vertex $u^j_k$ to the source $s^j_k$ of $C^j_k$, and a path from some vertex $\hat u^j_k$ to $s^j_k$ (after possibly deleting recurring vertices). In order to bound the approximation ratio, we prove the following claim.

\begin{claim}\label{claim: approx ratio full}
For each $1\leq i\leq \log n$, the number of class-$i$ edges that appear on the final path $P^*$ is at most $24|C^*|\log n/(2^i\tau)$.
\end{claim}

\begin{proof}
Let $E_i$ be the set of all level-$i$ edges that appear on $P^*$.
For each $1\leq j\leq \rho$, let $E_i^j\subseteq E_i$ be the set of all edges of $E_i$ that lie on the paths of $\pset_j$. 
It is enough show that for all $1\leq j\leq \log n$, $|E_i^j|\leq 24|C^*|/(2^i\tau)$.
We now fix some index $1\leq j\leq \log n$, and some path $P_k\in \pset_j$. Let $C_k\in \cset_j$ be the connected component to which $C_k$ belongs, and let $n_k=|R(C_k)|$. Recall that $P_k$ is a concatenation of two paths: a path  $Q$ from some vertex $u_k$ to the source $s_k$ of $C_k$, and a path $Q'$ from some vertex $\hat u_k$ to $s_k$, after we discard all vertices that appear on both paths, except for the lowest common ancestor of $u_k$ and $\hat u_k$ in $T(C_k)$. %Note that $Q$ may not contain extra-vertices, since each such vertex has degree $1$. 
Consider some edge $e\in E_i$ that lies on $Q$, and denote $e=(x,y)$. Since $e\in G'_j$, at least one of its endpoints (say $x$) owns $e$ and belongs to $L_j$. Therefore, if we denote $i'=\cutoff(x)$, then $i'\geq i$, and $|I_{i'}(x)|=\Delta(x)\geq 2^i\tau$, while, since $x\in L_j$, $2^j\leq \Delta(x)<2^{j+1}$. We conclude that $2^{j+1}>2^i\tau$. Consider the path $Q$, and let $U$ be the set of all vertices of $Q$ that belong to $L_j$. Let $U'\subseteq U$ be obtained by taking one out of every three consecutive vertices of $U$, so $|U'|\geq |U|/3$. Then each vertex of $U'$ has  effective degree at least $2^j\geq 2^i\tau/2$, and so it has at least $2^i\tau/2$ neighbors in $R(C_k)$. Moreover, for every pair $a\neq b$ of vertices in $U'$, $N_{C_k}(a)\cap N_{C_k}(b)=\emptyset$  (or we could decrease the length of $Q$ by connecting $a$ to $b$ through their common neighbor). Therefore, $|U'|\leq \frac{2|R(C_k)|}{2^i\tau}$, and $|U|\leq \frac{6|R(C_k)|}{2^i\tau}$. Therefore, the number of level-$i$ edges that lie on path $Q$ is bounded by $\frac{12|R(C_k)|}{2^i\tau}$ (as a vertex may be responsible for up to two such edges). We can use the same argument for path $Q'$. Overall, the number of level-$i$ edges that lie on $P_k$ is bounded by $\frac{24|R(C_k)|}{2^i\tau}$, and the total number of level-$i$ edges lying on paths of $\pset_j$ is at most $\frac{24}{2^i\tau}\sum_{C_k\in \cset_j}|R(C_k)|\leq \frac{24|C^*|}{2^i\tau}$.
\end{proof}


We now bound the running time of this algorithm.
For every level $1\leq j\leq \rho$, for every connected component $C\in \cset_j$, the algorithm spends up to $O(|C|)$ time to find the required path in the corresponding tree $T(C)$. We need to relate this bound to the number of regular vertices of $C$. Recall that each super-node $v_{C'}\in V(C)$ corresponds to a subset $C'\subseteq R(C)$ of regular vertices of $C$, and moreover, if $v_{C'}\neq v_{C''}$, then $C'\cap C''=\emptyset$. Therefore, there are at most $|R(C)|$ super-nodes in $C$. Each such super-node $v_{C'}\in C$ owns $O(|C'|\log |C'|)$ extra-vertices, so the total number of extra-vertices in $C$ is bounded by $\sum_{\stackrel{C'\in \cset_{j+1}:}{v_{C'}\in C}}O(|C'|\log |C'|)=O(|R(C)|\log |R(C)|)$. Overall, $|V(C)|=O(|R(C)|\log |R(C)|)$. The total time the algorithm spends on each layer $1\leq j\leq \rho$ is then at most $\sum_{C\in \cset_j}O(|R(C)|\log |R(C)|)=O(|C^*|\log |C^*|)$, and the total time for computing the answer to the query is $O(|C^*|\log^2n)$.



%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
\subsubsection{Maintaining the Data Structures}
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------

\paragraph{Initialization}

For every vertex $v$ in the original graph $G$, we compute $\cutoff(v)$, create the list of edges it owns partitioned into buckets by their level,  compute the effective degree of $v$ and $\level(v)$, in time $O(d_G(v))$. During this process we identify heavy edges. For each heavy edge $e$, we store pointers to its owner(s). All this takes $O(m)$ time.

Starting from $j=\log m$, we construct the graph $G_j$, the extended graph $G'_j$, and the set $\cset_j$ of connected components of $G'_j$. 
In order to do so, we construct the graph $G_j$, by adding one copy of every vertex in $V(G)$, and all edges owned by vertices on $L_j$. We then add, for every connected component $C\in \cset_{j+1}$, that is not a singleton vertex, a super-node $v_C$, that connects to every regular vertex of $C$, and a set $X(v_C)$ of $4|C|\log |C|$ extra-vertices, that connect to $v_C$ with edges. Since $\sum_{C\in \cset_{j+1}}|C|\leq n$, this can be done in time $O(m\log n)$ altogether. For every connected component $C$ of $G'_j$, we select an arbitrary vertex that is not an extra vertex to be its source $s(C)$ and set $D(C)=12|C|/2^j$. We then initialize $\EST(C,s(C),D(C))$. All this can also be done in total time $O(m\log n)$. %For every connected component $C\in \cset_j$, we set the bound $D(C)$ on the depth of the ES tree to be $12|C|/2^j$. From Corollary~\ref{cor: depth of tree bound}, the tree depth will always be bounded by this value.
We also initialize, for each $1\leq j\leq  \rho$, the data structure $\CONN(G'_j)$. This is done by starting from an empty data structure, and then adding the edges of $G'_j$ one-by-one.

%For accounting purposes, we also define potentials of the edges and the vertices of $G'_j$. Consider some connected component $C\in \cset_j$. For every edge $e=(u,v)$ of $C$, we let $\delta(e)$ denote $\min\set{d(s,u),d(s,v)}$. Throughout the algorithm, for every connected component $C\in \cset_j$, for every edge $e$ of $C$, the potential of $e$ is $4(D(C)-\delta(e))\tau$, where $\tau=O(\log n)$ is the time for a constant number of  heap operations. The potential of a vertex $v$ is $4(D(C)-d(s,v))\tau$.  We note that as the algorithm progresses and the clusters of $\cset_j$ are split into smaller clusters, we will define new bounds $D(C)$ on the cluster depth for the new clusters differently, to ensure that the potentials of the edges and the vertices do not increase.


\paragraph{Update Step.}

Suppose we need to delete an edge $e^*=(x,y)$. If $e^*$ is not a heavy edge, then the algorithm of Bernstein handles it. So we assume from now on that $e^*$ is a heavy edge. Assume first that $e^*$ is owned by exactly one of its endpoints - say $x$, and that $x\in L_j$. Then we need to delete the edge $e^*$ from the graph $G'_j$. As the result of this deletion, it is possible that the degree of $x$ will decrease below $2^j$, and so $x$ no longer belongs to $L_j$. Moreover, it is possible that $\cutoff(x)$ decreases, and so some of the edges that $x$ owned before the current iteration are no longer owned by $x$. In either case, we need to delete every type-$1$ edge $e'$ incident to $x$ from $G'_j$, unless $e'$ is owned by its other endpoint that belongs to $L_j$. We need to recompute the new effective degree and the new level $j'<j$ of $x$, and insert all edges that it still owns to the corresponding graph $G'_{j'}$. Moreover, as the result of all these edge-deletion operations, it is possible that some connected components of $G'_j$ split, and we will need
to split the corresponding super-nodes of $G'_{j-1}$ accordingly. This, in turn, can trigger more node-splitting in lower-level graphs. If the original edge $e^*$ is owned by both its endpoints, then it is possible that 
we need to delete it from two graphs, and repeat this whole process twice.


Therefore, over the course of the algorithm, we may need to delete edges from several graphs $G'_j$, where the deleted edge is either $e^*$, or it is an edge incident to a vertex whose effective degree decreases, or an edge may be deleted as a result of a vertex-splitting operation. Each one of these edge-deletion procedures may, in turn, trigger a vertex-splitting operation in the subsequent graph $G'_{j-1}$. Since vertex-splitting in $G'_{j-1}$ includes edge-deletion operations, this can in turn trigger vertex-splitting in $G'_{j-2}$, and so on. We now describe a procedure that deletes a given edge $e$ from a given graph $G'_j$.

\program{Delete-Edge($G'_j$,$e=(u,v)$)}{
\begin{enumerate}
\item Let $C$ be the connected component of $\cset_j$ that contains $e$ -- we can find it since $e$ points to it, and let $T(C)$ be the tree maintained by $\EST(C,s(C),D(C))$. If $e$ is not an edge of $T(C)$, delete $e$ from $G'_{j}$, and terminate the procedure. From now on, we assume that $e\in T(C)$.

\item Execute $\CONNDEL(G'_j,e)$. Check whether $u$ and $v$ are still connected in the new graph $G'_j$, by calling procedure $\conn(G'_j,u,v)$. 

\item If $u,v$ are still connected in the new graph $G'_j$:
execute $\ESDEL(C,e)$ and terminate the algorithm.

From now on we assume that $u,v$ are no longer connected in $G'_j$. We assume that $u$ is the parent of $v$ in the tree $T(C)$. Let $T_v$ be the sub-tree of $T$ rooted at $v$, and let $T'=T\setminus T_v$. Note that $C$ now decomposes into two connected components: one spanned by $V(T_v)$, and one spanned by $V(T')$. Next, we establish which of the two components contains fewer vertices.


\item Perform a BFS of $T_v$ from $v$ and a BFS of $T'$ from $s(C)$ in parallel, so both algorithms discover the same number of vertices at each step. Terminate the algorithm once all vertices in one of the two trees are explored. We assume w.l.o.g. that it is $T_v$; the other case is dealt with symmetrically.
\label{step: BFS}

\item 
We denote the connected component of $G'_{j+1}$ containing all vertices of $T_v$ by $C'$, and the connected component containing all vertices of $T'$ by $C''$. Set $s(C')=v$ and $D(C')=12|C'|/2^j$. Similarly, set $s(C'')=s(C)$ and $D(C'')=12|C''|/2^j$.
 Notice that $T_v$ is a shortest-path tree for $C'$ and $s(C')$, and $T'$ is a shortest-path tree of $C''$ and $s(C'')$. Initialize two new data structures: $\EST(C',s(C'),D(C'))$ using the tree $T_v$ and $\EST(C'',s(C''),D(C''))$ using tree $T'$, and the original data structure $\EST(C,s(C),D(C))$. Notice that the labels $\delta(x)$ for $x\in T_v$ have changed, and need to be set to $d(x,v)$ instead of $d(x,s)$. However, we know that $d(x,v)=d(x,s)-\delta(v)$, where $\delta(v)$ is the label of $v$ before the current update. Instead of updating the labels $\delta(x)$, we simply remember the value $\offset(C')=\delta(v)$ and treat each label $\delta(x)$ as $d(v,x)+\offset(C')$. We follow this pattern as the labels $\delta(x)$ get updated over the course of the algorithm. (We may not be able to afford to update all labels $\delta(x)$ for $x\in V(T_v)$, if $T_v$ contains more than half the vertices of $C$). \label{step: split ES-trees}

\item If $C'$ consists of a single vertex $v$:  \label{step: if one vertex}


\begin{enumerate}
\item update $v$ so that it no longer points to any connected component of $\lset_j$ and execute $\DE(G'_{j-1},e'=(v,v_C))$.
\item if $C''$ consists of a single vertex $u$: delete $C$ from the list $\lset_j$ of connected components of $G'_j$; update $u$ so that it no longer points to any component of $\lset_j$; execute $\DE(G'_{j-1},e'=(u,v_C))$.
\end{enumerate}

\item Otherwise: $C'$ and $C''$ contain more than one vertex each. \label{step: of more than one vertex}

\begin{enumerate}
 \item Add $C'$ to the list $\lset_j$ of connected components of $G'_j$ and add pointers from every vertex of $C'$ to $C'$; rename $C$ by $C''$ in $\lset_j$.
 
 \item Execute $\VS(G'_{j-1},v_C,C')$. \label{step: execute split cluster}
\end{enumerate}.
\end{enumerate}
}


\program{Vertex-Split($G'_j$,$v_C$, $C'$)}{
The procedure receives as input index $j$ of graph $G'_j$, and a super-node $v_C$ in this graph, such that cluster $C\in G'_{j+1}$ was split into $C'$ and $C''$, with $1<|C'|\leq |C''|$. The procedure is also given the list of vertices of $C'$, and a pointer to $C'$ and $C''=C\setminus C'$ in the list $\lset_j$ of components of $G'_{j+1}$. Let $\hat C\in \cset_j$ be the connected component of $G'_j$ containing $v_C$.

\begin{enumerate}
%\item If $C'$ contains a single vertex, that we denote by $u$, then execute $\DE(G'_j,(v_C,u))$ and terminate the algorithm. We now assume that $|C'|>1$.

\item Select disjoint subsets $X(v_{C'})$ of $\ceil{4|C'|\log |C'|}$ vertices of $C$ and $X(v_{C''})$ of $\ceil{4|C''|\log |C''|}$ vertices of $C$, and an additional vertex of $X(C)$ denoted by $v_{C'}$. Add a pointer from $v_{C'}$ to the component $C'$ on list $\lset_{j+1}$.

\item For each $x\in C'$, execute $\ESIN(\hat C, (v_{C'},x))$, and $\CONNIN(G'_j,(v_{c'},x))$.

\item For each $y\in X(v_{C'})$, execute $\ESIN(\hat C,(v_{C'},y))$, $\CONNIN(G'_j,(v_C',y))$, $\ESDEL(\hat C,(v_{C'},y))$, and $\CONNDEL(G_{j}',(v_{C'},y)$  (Notice that vertex $x$ has  degree $1$ in the original and in the new graph $G'_j$, so there is no need to run the full Procedure $\DE(G'_j,(v_C,y))$.)

\item For each $x\in C'$, and for each $x\in X(C)\setminus X(C'')$, execute $\DE(G'_j,(v_C,x))$ (notice that this includes $x=v_{C'}$).

%\item Execute $\DE(G'_j(v_C,v_{C'}))$.

\item Rename $v_C$ as $v_{C''}$ and add a pointer from it to $C''$ in the list $\lset_{j+1}$ of connected components of $G'_{j+1}$.
\end{enumerate}
}


We need to argue that operations $\ESIN$ that we perform do not decrease distances of vertices from $s(\hat C)$.
Notice that we only insert edges that connect $x_{C'}$ to the regular vertices of $C'$ and to the vertices of $X(C')$. At the moment of the insertion of these edges, all these vertices are connected to $v_C$ with an edge of length $1$, and the neighbors of $v_{C'}$ are a subset of the neighbors of $x_C$. \mynote{Need to fix this. Distance from $s(\hat C)$ to $v_{C'}$ may shorten.}

 Let $e^*=(x,y)$ be the edge that we need to delete from $G^H$. Let $z\in \set{x,y}$ be an endpoint of $e^*$ that owns it, and assume that $\level(z)=j$. We execute $\DE(G'_j,e^*)$. We then inspect both endpoints of $e^*$. We say that endpoint $z'$ of $e^*$ is bad if all of the following hold:
 
 \begin{itemize}
 \item $z'$ owned $e^*$ at the beginning of the update;
 \item $z'\in L_j$ at the beginning of the update; and
 \item $\Delta(z')<2^j$ after $e^*$ is deleted.
 \end{itemize}
 
For each bad endpoint $z'$ of $e^*$ we do the following:

\begin{itemize}
\item Recompute $\cutoff(z')$. If $\cutoff(z')$ decreased, then for every edge $e$ that $z'$ originally owned, but does not own anymore, update this information in edge $e$ and in $z'$.

\item Recompute the new effective degree of $z'$. If there is some index $1\leq j'\leq \rho$, such that $2^{j'}\leq \Delta(z')<2^{j'+1}$, add $z'$ to $L_{j'}$; for every edge $e$ that $z'$ still owns: execute $\ESIN(G'_{j'},e)$ and $\CONNIN(G'_{j'},e)$.

\item Inspect every edge $e\neq e^*$ that $z'$ owned before the update. 
Let $y_e$ be the other endpoint of this edge. If $y_e\not \in L_j$, or if $y_e$ does not own $e$, execute $\DE(G'_j,e)$.
\end{itemize}

Notice that, if $e^*$ is owned by both its endpoints, and these endpoints have different levels, we may need to execute the above procedure twice.

We need to verify that, when an edge is inserted into an $\EST$ data structure, the distances from the source do not increase. We only insert an edge $e=(a,b)$ into $G'_{j'}$ if both endpoints $a,b$ of $e$ belong to the same connected component of $G'_j$ for some $j>j'$. From Corollary~\ref{cor: containment of CC's}, $a$ and $b$ belong to the same connected component of $G'_{j'+1}$, that we denote by $\hat C$. Therefore, graph $G'_{j'+1}$ contains a vertex $v_{\hat C}$, to which both $a$ and $b$ are connected with edges of weight $1/2$. The insertion of the edge $(a,b)$ of length $1$ does not decrease any distances in $G'_{j'+1}$.



\paragraph{Time Analysis}
Fix some $1\leq j\leq \rho$. We first bound the total number of vertices of $G'_j$, and the total number of edges that ever belong to $G'_j$. To bound $|V(G'_j)|$, recall that it contains $n$ regular vertices, up to $n$ super-nodes, and up to $O(n\log n)$ extra-vertices, so $|V(G'_j)|=O(n\log n)$.

We now bound the total number of edges that either belong to $G'_j$ from the beginning, or are added to it over the course of the algorithm. Notice that every regular vertex $v$ may belong to $L_j$ at the start of the algorithm (time $0$), or it may start belonging to $L_j$ over the course of the algorithm. Whenever vertex $v$ is first added to $L_j$, either at the beginning of the algorithm, or later, it owns at most $2^{j+1}$ edges, that are added to $G'_j$ as type-$1$ edges. Therefore, the total number of type-$1$ edges that ever belong to $G'_j$ is bounded by $2^{j+1}\cdot n$.

We now bound the number of type-$2$ and type-$3$ edges. At the beginning of the algorithm, we are given some set $\cset_{j+1}$ of connected components of $G_{j+1}$, that are not isolated vertices. Denote these components by $C_1,\ldots,C_r$. Each component $C_i$ has $|C_i|$ type-$2$ edges incident to $v_{C_i}$, and $O(|C_i|\log |C_i|)$ type-$3$ edges incident to it. We charge the vertices of $C_i$ for these edges, so each vertex of $C_i$ is charged for one type-$2$ edge -- the edge that is incident to it, and $O(\log n)$ type-$3$ edges.

Consider now an iteration when $C_i$ is split into $C'_i$ and $C''_i$, with $|C'_i|\leq |C''_i|$. We then insert $|C'_i|$ new type-2 edges, and $O(|C'_i|\log |C'_i|)$ new type-$3$ edges. As before, we charge every vertex of $C'_i$ for one new type-$2$ edge, and for $O(\log n)$ new type-$3$ edge. Notice however that $|C'_i|\leq |C_i|/2$, so every vertex of $G$ can be charged at most $\log n$ times. Overall, the total number of type-$2$ edges that are ever added to $G'_j$ is bounded by $O(n\log n)$, and the bound for type-$3$ edges is $O(\log^3n)$.

Since the amortized update time for $\CONN(G_j')$ is $O(\log^2n)$, the total amount of time spent on $\CONNIN$ and $\CONNDEL$ operations is bounded by $O(n\poly\log n)$. Moreover, we only call query $\conn(G'_j,u,u')$ when the edge $(u,u')$ is deleted from $G'_j$. So the number of such queries over the course of the algorithm is $O(n\poly\log n)$, and the total time spent handling them is $O(n\poly\log n)$. From now on we can ignore all calls to the data structures $\CONN(G_j')$ over the course of our algorithm.



In order to analyze the remainder of the algorithm, we define potentials. Throughout the algorithm, for every vertex $v\in G_j'$, if $v$ is an isolated vertex then its potential $\phi(v)=0$. Otherwise, if $v$ belongs to a connected component $C\in \cset_j$, then $\phi(v)=(D(C)-d(v,s(C)))d(v)\eta$, where $d(v)$ is the degree of $v$ in $G_j'$, and $\eta=O(\log n)$ is time needed to perform a constant number of standard heap operations.
We then let $\phi(G_j')=\sum_{v\in V(G_j')}\phi(v)$.

At the beginning of the algorithm, for every connected component $C\in \cset_j$, $D(C)\leq n/2^j$. The total potential is then bounded by:

\[\phi(G_j')=\sum_{v\in V(G_j')}\phi(v)\leq \sum_{v\in V(G_j')}\frac{n}{2^j}\eta |E(G_j')|\leq \frac{n}{2^j}\eta n\cdot 2^j\leq O(n^2\poly\log n).\]


Whenever an edge is inserted into $G'_j$, the potential may increase by up to $2\cdot\frac{n}{2^j}\cdot \eta$, and the total number of edges every inserted into $G'_j$ is bounded by $O(n\log n\cdot 2^j)$, so the total increase in the potential is bounded by $O(n^2\poly\log n)$.

Consider now an execution of procedure $\DE(G'_j,e=(u,v))$, and assume that $u$ and $v$ lie in the connected component $C\in \cset_j$ before the current iteration. If the deletion of $e$ does not cause the split of $C$, then, ignoring the calls to $\CONN$ data structure, we execute one call to $\ESDEL$ data structure. As discussed before, the time spend on executing such a call is bounded by the decrease in the total potential.

Assume now that after $e=(u,v)$ is removed, component $C$ is split into $C'$ and $C''$, with $|C'|\leq |C''|$. Step~\ref{step: BFS} of Procedure $\DE$ takes $O(|C'|)$ time; we charge it to the $\VS$ procedure that is executed in Step~\ref{step: execute split cluster}. The remaining steps of the procedure take $O(1)$ time. However, once we split $C$ into $C'$ and $C''$, we set the new bounds $D(C')$ and $D(C'')$ on the cluster depths, and the potentials of the edges change. We assume w.l.o.g. that $C'$ is the cluster corresponding to the tree $T_v$. Notice that now, for every vertex $x\in T_v$, we need to take into account the distance of $x$ from the new source $v$, instead of $s$, in the potential $\phi(x)$. First, for every vertex $x\in C''$, $d(x,s(C''))=d(x,s(C))$ does not change, while $D(C'')<D(C)$ holds, so $\phi(x)$ may only decrease. We now consider some vertex $x\in V(C')$, and show that its potential also can only decrease. The original potential is:

\[\phi'(x)=(D(C)-d(x,s(C)))d(x)\eta=\left (\frac{12|C|}{2^j}-d(x,s(C))\right )d(x)\eta.\]

The new potential is:

\[\phi(x)=(D(C')-d(x,v))d(x)\eta=\left (\frac{12|C'|}{2^j}-d(x,v)\right )d(x)\eta.\]

Notice that $d(x,v)=d(x,s(C))-d(v,s(C))$, where all these distances are taken before the deletion of the edge $(u,v)$; this is since $v$ is on the shortest path from $x$ to $s(C)$. Therefore, in order to prove that the potential of $x$ does not increase, it is enough to show that:

\[\frac{12|C'|}{2^j}-d(x,s(C))+d(s(C),v)\leq \frac{12|C|}{2^j}-d(x,s(C)),\]

or, equivalently that:

\[d(s(C),v)\leq \frac{12(|C|-|C'|}{2^j}).\]

This is done in a way similar to the proof of Corollary~\ref{cor: depth of tree bound}. We let $U$ be the set of all vertices on the path $P$ from $s(C)$ to $v$ (before the deletion of the edge), that either lie in $L_j$ or are super-node. At least half of the vertices of $P$ belong to $U$, and each such vertex must have at least $2^j$ neighbors, each of which lies in $|C|-|C'|$. We then let $U'$ contain one vertex out of every $6$ consecutive vertices of $P$, and observe that for all $a,b\in U'$, $N(a)\cap N(b)=\emptyset$. Therefore, $|U'|\leq (|C|-|C'|)/2^j$... \mynote{need to switch 12 to 24}.

Finally, we analyze Procedure \VS. The running time of this procedure, excluding the calls to $\ESDEL$, $\ESIN$, $\CONNIN$ and $\CONNDEL$ is $O(|C'|)$

